Computing f-Divergences and Distances of High-Dimensional Probability Density Functions -- Low-Rank Tensor Approximations

Very often, in the course of uncertainty quantification tasks or data analysis, one has to deal with high-dimensional random variables (RVs). A high-dimensional RV can be described by its probability density (pdf) and/or by the corresponding probability characteristic functions (pcf), or by a polynomial chaos (PCE) or similar expansion. Here the interest is mainly to compute characterisations like the entropy, or relations between two distributions, like their Kullback-Leibler divergence. These are all computed from the pdf, which is often not available directly, and it is a computational challenge to even represent it in a numerically feasible fashion in case the dimension $d$ is even moderately large. In this regard, we propose to represent the density by a high order tensor product, and approximate this in a low-rank format. We show how to go from the pcf or functional representation to the pdf. This allows us to reduce the computational complexity and storage cost from an exponential to a linear. The characterisations such as entropy or the $f$-divergences need the possibility to compute point-wise functions of the pdf. This normally rather trivial task becomes more difficult when the pdf is approximated in a low-rank tensor format, as the point values are not directly accessible any more. The data is considered as an element of a high order tensor space. The considered algorithms are independent of the representation of the data as a tensor. All that we require is that the data can be considered as an element of an associative, commutative algebra with an inner product. Such an algebra is isomorphic to a commutative sub-algebra of the usual matrix algebra, allowing the use of matrix algorithms to accomplish the mentioned tasks.

==> ALmacrosV2.tex <==
% !TEX root = Rev2_13May2022.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: ALmacros.tex,v 2.2 2022/05/16 23:29:29 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 2.2 $",
%%  DATE      = "$Date: 2022/05/16 23:29:29 $",
%%  FILENAME  = "$RCSfile: ALmacros.tex,v $"}



\newcommand{\KL}{Karhunen-Lo\`eve}
\newcommand{\ip}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\bkt}[2]{\left\langle #1 \mid #2 \right\rangle}
\newcommand{\ipj}[1]{\left\langle #1 \right\rangle}
\newcommand{\ipd}[2]{\left\langle\negthinspace\ip{#1}{#2}\negthinspace\right\rangle}
\newcommand{\bkd}[2]{\left\langle\negthinspace\bkt{#1}{#2}\negthinspace\right\rangle}
\newcommand{\ns}[1]{\left| #1 \right|}
\newcommand{\nd}[1]{\left\Vert #1 \right\Vert}
\newcommand{\nt}[1]{\left\Vert\negthinspace\left| #1 \right|\negthinspace\right\Vert}
\newcommand{\trpos}{{\ops{T}}}

\newcommand{\cntrct}[2]{\tensor*[_#1]{\times}{_#2}}

\newcommand{\bbbone}{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}
{\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}

%%%%Needed for tensor section
\newcommand    {\ve}[1]
                {\underline{#1}}

\newcommand    {\dist}[2]
                {\mrm{dist}\, \left ( #1, #2 \right ) }

\newcommand    {\Mul}[2]
                {\C{M}ul(#1, #2)}

%\newcommand    {\tr}[1]
%                {\C{T}_#1}

\newcommand{\R}{\D{R}}
\newcommand{\N}{\D{N}}
\newcommand{\bbC}{\D{C}}
\newcommand{\Tp}{\C{T}}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\var}{var}
\newcommand{\Nset}{\D{N}}

%
%\newcommand    {\E}
%                {\mathds{E}}

\newcommand    {\RR}
                {\D{R}}
\newcommand    {\Rp}
                {\C{R}}

\newcommand    {\kts}[5]
                {\sum_{#1=1}^{#2} \ten_{#3=1}^{#4} #5_{#1 #3}}

\newcommand    {\ktsS}[4]
                {\sum_{#1=1}^{#2} \ten_{\mu=1}^{#3} #4_{#1 \mu}}

\newcommand    {\Kts}[5]
                {\sum_{#1=1}^{#2} \Ten_{#3=1}^{#4} #5_{#1 #3}}

\newcommand    {\KtsS}[4]
                {\sum_{#1=1}^{#2} \Ten_{\mu=1}^{#3} #4_{#1 \mu}}

\newcommand    {\ten}    { \otimes }
\newcommand    {\Ten}    { \bigotimes }
   \newcommand    {\Rd}    { \D{R}^d }
   \newcommand    {\Rn}    { \D{R}^n }
   \newcommand    {\RN}    { \D{R}^N }
    \newcommand    {\Rnn}   { \D{R}^{n \times n}}
    \newcommand    {\Rm}    { \D{R}^m }
    \newcommand    {\Rmm}   { \D{R}^{m \times m}}
    
\newcommand    {\BbbC}{\D{C}}                                %%  complex C
\newcommand    {\BbbN}{\D{N}}                                %%  integer N
\newcommand    {\BbbK}{\D{K}}                                %%  field K
\newcommand    {\BbbQ}{\D{Q}}                                %%  rational Q
\newcommand    {\BbbR}{\D{R}}                                %%  real    IR
\newcommand    {\BbbE}{\D{E}}                                %%  euclidian IE
\newcommand    {\BbbZ}{\D{Z}}                                %%  integer Z

%\newcommand\dblone{\hbox{$1\hskip -1.2pt\vrule depth 0pt height 1.6ex width 0.7pt \vrule depth 0pt height 0.3pt width 0.12em$}}
%\newcommand{\jmath}{j}
%\newcommand{\supp}{\mathop{\mrm{supp}}\nolimits}
%\newcommand{\div}{\mathop{\mrm{div}}\nolimits}
%\newcommand{\cov}{\mathop{\mrm{cov}}\nolimits}
\newcommand{\diam}{\mrm{diam}}
%\newcommand{\dist}{\mrm{dist}}
\newcommand{\sons}{\mrm{sons}}
%\newcommand{\const}{\mrm{const}}
%\newcommand{\rank}{\mrm{rank}}
\newcommand{\trace}{\mrm{trace}}
%\newcommand{\KLD{\mbox{KLD}}
\newcommand{\alphab}{\vek{\alpha}}
\newcommand{\betab}{\vek{\beta}}

\newcommand    {\dotprod}[2] { \left \langle #1, #2 \right \rangle }

\newcommand{\frkt}[2]{{{\raise0.6ex\hbox{{\leavevmode$\textstyle #1$}}}{\raise0.25ex\hbox{\kern-0.35ex\hbox{/}}}{\raise-0.3ex\hbox{\kern-0.4ex\hbox{{\leavevmode$\textstyle  #2$}}}}}}
\newcommand{\frkc}[2]{{{\raise0.7ex\hbox{{\leavevmode$\scriptstyle #1$}}}{\raise0.2ex\hbox{\kern-0.4ex\hbox{\footnotesize /}}}{\raise-0.2ex\hbox{\kern-0.4ex\hbox{{\leavevmode$\scriptstyle #2$}}}}}}
\newcommand{\frkx}[2]{{{\raise0.75ex\hbox{{\leavevmode$\scriptscriptstyle #1$}}}{\raise0.17ex\hbox{\kern-0.45ex\hbox{\scriptsize /}}}{\raise-0.15ex\hbox{\kern-0.4ex\hbox{{\leavevmode$\scriptscriptstyle #2$}}}}}}
\newcommand{\frkz}[2]{{{\raise0.75ex\hbox{{\leavevmode$\scriptscriptstyle #1$}}}{\raise0.17ex\hbox{\kern-0.45ex\hbox{\tiny /}}}{\raise-0.15ex\hbox{\kern-0.4ex\hbox{{\leavevmode$\scriptscriptstyle #2$}}}}}}

%\newcommand{\frk}[2]{{\mathchoice{{\frkt{#1}{#2}}}{{\frkc{#1}{#2}}}{{\frkx{#1}{#2}}}{{\frkz{#1}{#2}}}}}
\newcommand{\frk}[2]{{\mathchoice{{\frac{#1}{#2}}}{{\frac{#1}{#2}}}{{\frac{#1}{#2}}}{{\frac{#1}{#2}}}}}


\newcommand{\erf}{\mbox{erf}}
%\newcommand{\EXP}[1]{\mathbb{E}\left(#1\right)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dblone}{\hbox{$1\hskip -1.2pt\vrule depth 0pt height 1.6ex width 0.7pt \vrule depth 0pt height 0.3pt width 0.12em$}}

\newcommand{\pb}{\vek{p}}
\newcommand{\U}{\vek{U}}
\newcommand{\bSigma}{\vek{\Sigma}}

\newcommand{\eps}{\varepsilon}
%\def\diag{\mathop{\rm diag}\nolimits}
%\def\supp{\mathop{\rm supp}\nolimits}
\newcommand{\Ip}{\C{I}}
%\def\nin{\hspace{0.22em}/ \hspace{-0.88em} \in}       %%  not in
\newcommand{\nin}{\notin}
\newcommand{\Js}{\C{J}}


% Some my aliases
\newcommand{\mybold}[1]{\vek{#1}}
%\newcommand{\u}{\mybold{u}}
\newcommand{\bi}{\mybold{i}}
\newcommand{\bk}{\mybold{k}}
\newcommand{\bp}{\mybold{p}}
\newcommand{\bx}{\mybold{x}}
\newcommand{\by}{\mybold{y}}
\newcommand{\bX}{\mybold{X}}
%\newcommand{\b0}{\mybold{0}}
\newcommand{\bt}{\mybold{t}}
\newcommand{\bT}{\mybold{T}}
\newcommand{\bw}{\mybold{w}}
\newcommand{\bA}{\mybold{A}}
\newcommand{\bB}{\mybold{B}}
\newcommand{\f}{\mybold{f}}
\newcommand{\bC}{\mybold{C}}
\newcommand{\bI}{\mybold{I}}
\newcommand{\K}{\mybold{K}}
\newcommand{\BDelta}{\vek{\Delta}}
\newcommand{\J}{\C{J}}
\newcommand{\param}{\kappa}
\newcommand{\ttp}{\mathtt{p}}
\newcommand{\uh}{\mybold{u}}
\newcommand\myeq{\stackrel{\mathclap{\normalfont\mbox{def}}}{?}}

\newcommand{\bv}{\vek{v}}
\newcommand{\vd}{\vec{d}}
\newcommand{\vX}{\vek{\xi}}
\newcommand{\vY}{\vek{y}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vxi}{\vek{\xi}}
\newcommand{\bTheta}{\vek{\Theta}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vj}{\vec{j}}
\newcommand{\mT}{\mtt{T}}
\newcommand{\Rset}{\C{J}}

\newcommand{\thetab}{\vek{\theta}}
\newcommand{\Fd}{\C{F}_d}
\newcommand{\iFd}{\C{F}_{d}^{-1}}
\newcommand{\zetab}{\vek{\zeta}}
\newcommand{\etab}{\vek{\eta}}
\newcommand{\varphib}{\vek{\varphi}}
\newcommand{\phib}{\vek{\phi}}
\newcommand{\omegab}{\vek{\omega}}

\newcommand{\cdf}{\texttt{cdf}\xspace} % cumulative probability function
\newcommand{\pdf}{\texttt{pdf}\xspace} % probability density function
\newcommand{\cdfs}{\texttt{cdfs}\xspace} % cumulative probability function
\newcommand{\pdfs}{\texttt{pdfs}\xspace} % probability density function
\newcommand{\pcfs}{\texttt{pcfs}\xspace} % probability characteristic function
\newcommand{\pcf}{\texttt{pcf}\xspace} % probability characteristic function
\newcommand{\StochDim}{J} % Stochastic dimension
\newcommand{\nus}{\nu} % Index for stochastic variable
\newcommand{\rhs}{\mybold{b}} % The right hand side
\newcommand{\solu}{\mybold{v}} % The right hand side

\newcommand    {\normTp}[1] { \|  #1  \|_\Tp }
\newcommand    {\minset}[2]
                {\F{M}(#1,#2)}

\newcommand{\BIGOP}[1]{\mathop{\mathchoice%
{\raise-0.22em\hbox{\huge $#1$}} {\raise-0.05em\hbox{\Large $#1$}}
{\hbox{\large $#1$}}{#1}}}
% nur fuer Bigboxplus andere Korrekturen
\newcommand{\BIGboxplus}{\mathop{\mathchoice%
{\raise-0.35em\hbox{\huge $\boxplus$}}%
{\raise-0.15em\hbox{\Large $\boxplus$}}{\hbox{\large
$\boxplus$}}{\boxplus}}}
%\newcommand{\bigtimes}{\BIGOP{\times}}

\newcommand    {\Vp}{\C{V}}
\newcommand    {\Pp}{\C{P}}
\newcommand    {\Np}{\C{N}}

%\newcommand    {\Lp}
%                {\mathcal{L}}
% \Lp already defined in macros

\newcommand    {\Mp}{\C{M}}
\newcommand    {\Span}  { \mbox{\rm span} }

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{defn}[theorem]{Definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{notation}[theorem]{Notation}
%\newtheorem{problem}[theorem]{Problem}
%\newtheorem{task}[theorem]{Definition and Notation}
%\newenvironment{defn}{\textbf{Definition
%\refstepcounter{theorem}{\thetheorem}} }
\newtheorem{example}[theorem]{Example}
%\newenvironment{example}{\textbf{Beispiel
%\refstepcounter{theorem}{\thetheorem}} }


%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{lemmaDef}[theorem]{Lemma and Definition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{korollar}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}

%\newcommand{\bv}{\mathbf{v}}
\newcommand{\br}{\mybold{r}}
\newcommand{\bz}{\mybold{z}}
\newcommand{\bs}{\mybold{s}}
\newcommand{\bu}{\mybold{u}}
%\newcommand{\trace}{\mbox{trace}}
%\newcommand{\A}{\mat{A}}
%\newcommand{\bA}{\mybold{A}}
%\newcommand{\B}{\mat{B}}
%\newcommand{\bB}{\mybold{B}}

\newcommand{\todo}[1]{{\Large\textcolor{red}{#1}}}

%\renewcommand\theparagraph{\textbf{paragraph}}

\definecolor{light-blue}{rgb}{0.1,0.75,0.9} 
\definecolor{myred}{rgb}{0.8, 0.1, 0.2}


\newcommand{\note}[1]{\textcolor{red}{ #1 }}

\newcommand{\ALc}[1]{\textcolor{magenta}{[AL: #1]}}
\newcommand{\AL}[1]{\textcolor{myred}{#1}}
\newcommand{\ALs}[2]{\textcolor{orange}{#1 / }\textcolor{myred}{#2}}

\newcommand{\HGMc}[1]{\textcolor{magenta}{[HGM: #1]}}
\newcommand{\HGM}[1]{\textcolor{blue}{#1}}
\newcommand{\HGMs}[2]{\textcolor{light-blue}{#1 / }\textcolor{blue}{#2}}




%  $Log: ALmacros.tex,v $
%  Revision 2.2  2022/05/16 23:29:29  hgm
%  to make it run with ALmacros
%
%  Revision 2.1  2022/05/16 21:07:38  hgm
%  headers and footers
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Rev2_13May2022"
%%% End: 



==> chaptersV2/TT-cross.tex <==






% % !TEX root = ../19_low-rank_tensor_prob_den_char.tex
% % !TEX encoding = UTF-8 Unicode

% % RCSID:       $Id: TT_approx.tex,v 1.4 2021/08/03 08:23:29 hgm Exp $
% % Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
% %              Marco Scavino, and Alessio Spantini
% % Contact:     wire@tu-bs.de
% % =================================
% %% texfile{
% %%  AUTHOR    = "$Author: hgm $",
% %%  VERSION   = "$Revision: 1.4 $",
% %%  DATE      = "$Date: 2021/08/03 08:23:29 $",
% %%  FILENAME  = "$RCSfile: TT_approx.tex,v $"}
% %
% \subsection{Direct approximation of $\tnb{v}:=g(\tnb{u})$}
% \label{sec:TT-cross-apr}

% In this section, we discuss the so-called cross algorithms \cite{oseledetsTyrt2010,BallaniGrasedyck2015,ds-alscross-2017pre,DolgovLitvLiu19}. 
% Some extensions of the TT-Cross and ALS-Cross algorithms (e.g., AMEn algorithm) were suggested by S. Dolgov and co-authors and can be found here \url{https://people.bath.ac.uk/sd901/als-cross-algorithm/}.

% These algorithms building an alternative to iterations and series expansions, to compute a low-rank approximation of $g(\tnb{u})$ for a given function $g(\cdot)$ and a tensor $\tnb{u}$ directly, ``on the fly''.
% We assume here that the full tensor $\tnb{v}:=g(\tnb{u})$ is not given explicitly, but rather as a function which can return any element $\tnb{v}_{\tnb{i}}$ of $\tnb{v}$.

% For example, amen$\_$cross$\_$s() algorithm can compute the representation~\eqref{eq:tt} using only $\mathcal{O}(dnr^2)$ entries of $\tnb{v}$ and $\mathcal{O}(dnr^3)$ additional arithmetic operations. 
% The pseudocode is listed in \cite{DolgovLitvLiu19}.
% It is based on the skeleton decomposition (another name is adaptive cross approximation) of a matrix~\cite{TyrtyshACA,ACA,bebe-aca-2011} and the \emph{maxvol} algorithms \cite{gostz-maxvol-2010}. The idea of \emph{maxvol} is to find a rank-$r$ matrix approximation $A_r$ of a $n\times m$ matrix $A$, rank of which is $r$. The \emph{maxvol} suggests to select among all $r\times r$ submatrices the one that has the largest volume (determinant). The computational complexity is $\mathcal{O}(r(n+m))$, and the approximation error $\Vert A-A_r \Vert_{\infty}\leq (r+1) \sigma_{r+1}$, where $\sigma_{r+1}$ is the $(r+1)$-th singular value of $A$.

% A general cross algorithm
% computes the following representation:
% \begin{equation}\label{eq:tt}
% %  \begin{split}
%   \tnb{v}(\alpha_1,\ldots,\alpha_M)  = 
%   \sum_{s_1=1}^{r_1} \sum_{s_2=1}^{r_2}  \cdots \sum_{s_{M-1}=1}^{r_{M-1}}
%       \tns{v}^{(1)}_{s_0,s_1}(\alpha_1) \tns{v}^{(2)}_{s_1,s_2}(\alpha_2) 
%       \cdots \tns{v}^{(M)}_{s_{M-1},s_M}(\alpha_M).
% %  \end{split}
% \end{equation}
% %and is listed in Algorithm \ref{alg:cross}.
% % where we let $\mathcal{I}_{<1} = \mathcal{I}_{>d} = \emptyset$ for uniformity.

% %Note, that after applying IFFT, we obtain a similar %representation for $p_{\vX}(\by)$.}
% % \textcolor{red}{We are thinking  to replace the TT cross by standard ACA...}

% % \begin{algorithm}[t]
% % \caption{TT cross algorithm with rank adaptation.\textcolor{red}{Notation below is not defined}}
% % \label{alg:cross}
% % \begin{algorithmic}[1]
% %  \Require Initial index sets $\mathcal{I}_{>k}$, rank increasing parameter $\rho\ge 0$, stopping tolerance $\delta>0$ and/or maximum number of iterations $\mathrm{iter}_{\max}$.
% %  \Ensure TT blocks of an approximation \eqref{eq:tt} to $\tnb{v}$.
% %  \While{$\mathrm{iter}<\mathrm{iter}_{\max}$ and $\|\tilde{\tnb{v}}_{\mbox{iter}}-\tilde{\tnb{v}}_{\mbox{iter}-1}\|>\delta \|\tilde{\tnb{v}}_{\mbox{iter}}\|$}
% %     \For{$k=1,2,\ldots,d$} \Comment{Forward iteration}
% %       \State (Optionally) prepare an auxiliary enrichment set $\mathcal{I}_{>k}^{aux}$.
% %       \State Compute the $r_{k-1}n \times r_k$ unfolding matrix $\tnb{v}(\mathcal{I}_{<k},i_k;~\mathcal{I}_{>k})$.
% %       \State Compute $\mathcal{I}_{<k+1}$ by the \emph{maxvol} algorithm and (optionally) truncate.
% %     \EndFor
% %     \For{$k=d,d-1,\ldots,1$} \Comment{Backward iteration}
% %       \State (Optionally) prepare an auxiliary enrichment set $\mathcal{I}_{<k}^{aux}$.
% %       \State Compute the $r_{k-1} \times nr_k$ unfolding matrix $\tnb{v}(\mathcal{I}_{<k}~;i_k,\mathcal{I}_{>k})$.
% %     \State Compute $\mathcal{I}_{>k-1}$ by the \emph{maxvol} algorithm and (optionally) truncate.
% %     \EndFor
% %  \EndWhile
% % \end{algorithmic} 
% % \end{algorithm} 


% If $g(\cdot)$ is analytic, the TT ranks often depend logarithmically on the accuracy \cite{khor-rstruct-2006,uschmajew-approx-rate-2013}.
% %Interpolation or integration using the TT format with collocation on the Chebyshev grid costs $\mathcal{O}(d|\log\varepsilon|^{3})$, which
% %is smaller than $\mathcal{O}(\varepsilon^{-2})$ -- the cost of the Monte Carlo method.
% %For proper definitions and properties we refer to the Appendix~\ref{sec:TT-cross-apr}.


% % \subsection{Adaptive Cross Approximation (ACA) \textcolor{red}{Notation below is old!}}
% % \label{sec:ACA}
% % Suppose that $R\in \mathbb{R}^{n\times m}$ is a given rank-$k$ matrix. The ACA Algorithm~\ref{algo:ACA} is a heuristic algorithm, which computes factor matrises $A$ and $B$, such that $R=A\cdot B^\top$,  $A\in \mathbb{R}^{n\times k}$ and $B\in \mathbb{R}^{m\times k}$. The standard SVD is exact, but costs $\mathcal{O}(n^2m)$, so a cheaper technique is desired.
% % One of the possible ways to do it is the Adaptive Cross Approximation (ACA) algorithm \cite{TyrtyshACA, ACA, ACA2, Winter}. 

 
% % Suppose we have a function, which allows us to compute any element of $\R$. The ACA algorithm computes vectors $a_{\ell}$ and $b_{\ell}$ which form $\tilde{R}$ such that $\Vert R-\tilde{R}\Vert \leq \varepsilon $, where $\tilde{R}=\sum_{\ell=1}^{k}a_{\ell}b_{\ell}^T$ and $ \varepsilon $ is a desired accuracy.


% % \begin{algorithm}[t]
% % \caption{ACA algorithm}
% % \label{algo:ACA}   
% %     \begin{algorithmic}
% %       \State \textbf{begin}
% %       \State{\quad $/*$ input is a function which computes $R_{ij}$ and required accuracy $\varepsilon$ $*/$;} 
% %       \State{\quad $/*$ output is matrix $\tilde{R}$ $*/$;} 
% %       \State{\quad $k=0$; $\tilde{R}=0$;} 
% %       \State{\quad $S=\emptyset$; $/*$ set of row indices $*/$}
% %       \State{\quad $T=\emptyset$; $/*$ set of column indices $*/$}
% %       \State{\quad \textbf{do}}
% %       \State{\quad\quad Take a row $i^*\notin S$;}
% %       \State{\quad\quad Subtract $R_{i^*j}:=R_{i^*j}-\tilde{R}_{i^*j}$, $j=1..m$;}
% %       \State{\quad\quad Find $\max_j |a_{i^*j}|\neq 0$, $j<m$. Suppose it lies in column $j^*$;}
% %       \State{\quad\quad Compute all elements $b_{ij^*}$ in column $j^*$, $i<n$;}
% %       \State{\quad\quad Subtract $R_{ij^*}:=R_{ij^*}-\tilde{R}_{ij^*}$, $i=1..n$;}
% %       \State{\quad\quad $k:=k+1$; $S:=S\cup \{i^*\}$; $T:=T\cup \{j^*\}$;}
% %       \State{\quad\quad Compute $\tilde{R}=\tilde{R}+a_{i^*}\cdot b_{j^*}^T$; $/*$ it is rank $k$ approximation$*/$}
% %       \State{\quad\quad if$(\Vert a_{i^*}\cdot b_{j^*}^T \Vert_2 \leq \varepsilon \cdot \Vert a_{1}\cdot b_{1}^T \Vert_2)$ return $\tilde{R}$};
% %       \State{\quad\quad Find $\max_i |b_{ij^*}|$, $i<n$, $i\neq i^*$. The row where it lies is a new row $i^*$}; 
% %       \State{\quad \textbf{until}($k<k_{\max}$)}
% %       \State{\quad return $\tilde{R}$;}
% %       \State \textbf{end}; 
% %     \end{algorithmic}
% %  \end{algorithm}
% % Note that the algorithm does not compute the whole matrix $R$. The subtraction is done only from the elements under consideration, i.e. rows $a_{\ell}$ and column $b_{\ell}$, $\ell=1,...,k$. Note also that only $k$ rows and $k$ columns of $R$ are computed and stored. 
 

% %In \cite{Grased_Interpol} the authors assume that for smooth $\chi\vert_{B_{\tau}\times B_{\sigma}}$ the matrix $\tilde{\R}$ of rank $k$ can be constructed %by interpolation of the kernel $\chi$ in such a way that the approximation error behaves like 
% %\begin{equation}
% %\Vert \R-\tilde{\R}\Vert=\mathcal{O}(\mu^{-k})
% %\end{equation}
% %for a constant $\mu<1$, i.e., exponential convergence with respect to the order $k$.\\
% %``''
% % \begin{rem}
% %  Another useful application of the ACA algorithm is preprocessing for computing SVD. Suppose that factorisation of matrix $\R=\A\B^T$, $\A\in \RR^{n\times K}$, $\B\in \RR^{m\times K}$, is found by ACA. Suppose also that rank of $\R$ is $k$, $k<K$. Then one can apply the following algorithm to compute a reduced SVD $\R=\U\Sigma\V^T$ efficiently \cite{Winter}.
% % \end{rem}
% % \begin{algo}
% % \label{algo:tSVD}   
% %     \begin{algorithmic}
% %       \State{Truncated SVD algorithm}
% %       \State \textbf{begin}
% %       \State{\quad $/*$ input is the matrices $\A\in \RR^{n\times K}$ and $\B\in \RR^{m\times K}$;} 
% %       \State{\quad $/*$ output is the SVD of $\R=\A\B^T$ $*/$;} 
% %       \State{\quad $/*$ Compute QR-factorisation of $\A$ and $\B$ $*/$} 
% %       \State{\quad $\A=\Q_{A}\R_{A}$; $/*$ $\Q_{A}\in \RR^{n\times k}$, $\R_{A} \in \RR^{k\times k}$, with $k<K$ $*/$} 
% %       \State{\quad $\B=\Q_{B}\R_{B}$; $/*$ $\Q_{B}\in \RR^{m\times k}$, $\R_{B} \in \RR^{k\times k}$ $*/$} 
% %       \State{\quad $/*$ Compute a reduced SVD of $\R_A \R_B^T$ $*/$}
% %       \State{\quad $\R_A \R_B^T=\U^{'}\Sigma(\V^{'})^T$;}
% %       \State{\quad $/*$ Compute matrix-matrix products $*/$}
% %       \State{\quad $\U:=\Q_A\U^{'}$;}
% %       \State{\quad $\V:=\Q_B\V^{'}$;}
% %       \State \textbf{end}
% %     \end{algorithmic}
% % \end{algo}
% % The computational cost of all three steps is $\mathcal{O}((n+m)k^2+k^3+(n+m)k^2)$ \cite{Winter}.
% %







==> chaptersV2/TuckerFormat.tex <==
% !TEX root = 19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: TuckerFormat.tex,v 1.2 2021/11/07 22:17:44 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.2 $",
%%  DATE      = "$Date: 2021/11/07 22:17:44 $",
%%  FILENAME  = "$RCSfile: TuckerFormat.tex,v $"}


\subsection{The Tucker tensor format}
\label{ssec:Tucker}
%
The Tucker tensor format was introduced in \citep{Tuck:66}.
\begin{figure}[htb]
\centering
\includegraphics[width=0.55\textwidth]{figs/Tucker1.png}
\caption{Schema of the Tucker decomposition of a 3D tensor.}
\label{fig:Tucker}
\end{figure}
A schema for the Tucker tensor format for $d=3$ is shown in 
Figure~\ref{fig:Tucker}.  The full tensor 
$\tnb{w}\in \D{R}^{n_1\times n_2\times n_3}$ is shown on the left side of the equality 
sign, and its decomposition on the right.  The small cube on the right side in the 
Tucker format denotes a core-tensor $\That{w}$ of size 
$r_1\times r_2 \times r_3$, and the rectangles denote matrices of column vectors
$\vek{U}_1:=[\vek{w}_{1}^{(1)},\dots,\vek{w}_{r_1}^{(1)}]\in \D{R}^{n_1\times r_1}$,
$\vek{U}_2:=[\vek{w}_{1}^{(2)},\dots,\vek{w}_{r_2}^{(2)}]\in \D{R}^{n_2\times r_2}$,
$\vek{U}_3:=[\vek{w}_{1}^{(3)},\dots,\vek{w}_{r_3}^{(3)}]\in \D{R}^{n_3\times r_3}$,
In this way one has
\[ 
\tnb{w} =  \That{w} \times_1 \vek{U}_1^\trpos \times_2 \vek{U}_2^\trpos \times_3 \vek{U}_3^\trpos,
\]
where the symbol $\times_k$ denotes the contraction of the $k$-th tensor index 
of $\That{w}$ with the first index of the matrix $\vek{U}_k^\trpos$ in Figure~\ref{fig:Tucker}.


\begin{definition}[Tucker Tensor Format]\label{D:TuckerFormat}
The Tucker tensor format in $\C{T}$ with rank parameter $\vek{r}=(r_1,\dots,r_d)$ is
defined by the multilinear mapping
\begin{align} \nonumber
\tns{U}_{\Tuck,\vek{r}} : \C{P}_{\Tuck,\vek{r}}&:=\bigtimes_{\nu=1}^d \C{P}^{r_\nu}_\nu 
  \times \C{P}_c  \rightarrow \C{T}, \quad \C{P}_\nu = \D{R}^{M_\nu}\; (\nu=1,\dots,d), 
  \quad \C{P}_c = \D{R}^{r_1} \otimes \dots \otimes \D{R}^{r_d},\\ \label{eq:TuckerFormat}
   \C{P}_{\Tuck,\vek{r}}\ni \tnb{P} &:= \left(\vek{w}^{(i)}_{\nu_i}, \That{w}=
    (\Shat{w}_{\nu_1, \ldots ,\nu_d})\in\C{P}_c: 1\le \nu_i \le r_i, 1\le i\le d\right) \\
    &\qquad \mapsto \quad\tns{U}_{\Tuck,\vek{r}}(\tnb{P}) := \tnb{w}=
    \sum_{\vek{\nu}}^{\vek{r}} \Shat{w}_{\nu_1, \ldots ,\nu_d}\bigotimes_{i=1}^d
     \,  {\vek{w}}^{(i)}_{\nu_i}\; \in\C{T},
    \nonumber
\end{align}
where $\{{\vek{w}}^{(i)}_{\nu_i}\}_{\nu_i=1}^{r_i}\subset \D{R}^{M_i}$ 
represents a set of orthonormal vectors for $i=1,\dots,d$ and $\That{w}=
 (\Shat{w}_{\nu_1, \ldots ,\nu_d} ) = (\Shat{w}_{\vek{\nu}})\in\C{P}_c$ 
is the so-called Tucker core tensor.  We call the sum of elementary tensors 
$\tnb{w}=\tns{U}_{\Tuck,\vek{r}}(\tnb{P})$ a tensor represented in the Tucker tensor format with
$\prod_{i=1}^d r_i$ terms. 
%The system of vectors $\left(\tns{p}_{i \nu} : 1\leq i \leq r,
%\mbox{ } 1\leq \nu \leq d\right)$ is a \emph{representation system}
%of $\tnb{v}$ with \emph{representation rank} $r$.
\end{definition}
Originally, it was applied for tensor decompositions of
multidimensional arrays in chemometrics.
The Tucker tensor format provides a
stable algorithm for decomposition of full-size tensors. 
The higher order singular value decomposition (HOSVD) and the Tucker
ALS algorithm for orthogonal Tucker approximation of higher 
order tensors were introduced in \citep{DMV-SIAM2:00}. 
%We say that the tensor $\tnb{w} $ is represented in the rank-$\vek{ r}$ orthogonal Tucker format 
%with the rank parameter ${\vek{ r}}=(r_1,\ldots,r_d)$ if 
%\begin{equation}\label{eqn:Tucker_form}
%  {\tnb{w}}  =\sum\limits_{\nu_1 =1}^{r_1}\ldots
%\sum\limits^{r_d}_{{\nu_d}=1} \Shat{w}_{\nu_1, \ldots ,\nu_d}
%\,  {\tns{ w}}^{(1)}_{\nu_1} \otimes \ldots \otimes {\tns{ w}}^{(\ell)}_{\nu_{\ell}} 
%\ldots \otimes {\tns{ w}}^{(d)}_{\nu_d},\quad \ell=1,\ldots,d, 
%\end{equation}
%where $\{{\tns{ w}}^{(\ell)}_{\nu_\ell}\}_{\nu_\ell=1}^{r_\ell}\in \D{R}^{n_\ell}$ 
%represents a set of orthonormal vectors for $\ell=1,\ldots,d$, 
%and 
%%$\bB=[\bB_{\nu_1,\ldots,\nu_d}] \in \D{R}^{r_1\times \cdots \times r_d}$ 
%$\That{w}=(\Shat{w}_{\nu_1, \ldots ,\nu_d})\in \D{R}^{r_1\times \cdots \times r_d}$
%is 
%the Tucker core tensor. 
The storage cost for the Tucker tensor is bounded by 
$\C{O}(d\,r\,n +r^d)$, with $r:=\max_\ell r_\ell$.
% Using the orthogonal side matrices $V^{(\ell)}=[v^{(\ell)}_1 \ldots v^{(\ell)}_{r_\ell}]$ 
% and contracted products, the Tucker tensor decomposition may be presented in the alternative notation,
% \[
%   { {\bf A}_{({\bf r})}=\bB \times_1 V^{(1)}\times_2 V^{(2)} \times_3 \ldots 
%   \times_d V^{(d)}.} 
% \]  
% In the case $d=2$, the orthogonal Tucker decomposition is equivalent to the singular 
% value decomposition (SVD) of a rectangular matrix. 
% %
%
\subsubsection{Basic operations with the Tucker format}
Let us assume $\tnb{w}=\tns{U}_{\Tuck,\vek{r}}(\tnb{P})$
in Tucker format as in \refeq{eq:TuckerFormat}. 

\paragraph{Multiplication by a scalar} $\alpha$
can simply be done by multiplying the core tensor $\That{w}$:
\begin{equation*}
\alpha\cdot {\tnb{w}}  = \sum_{\vek{\nu}}^{\vek{r}} (\alpha\Shat{w}_{\nu_1, \ldots ,\nu_d})
    \bigotimes_{i=1}^d \, \vek{w}^{(i)}_{\nu_i}. 
\end{equation*}
The computational cost is $\C{O}( \prod_{i=1}^d r_i)$ (or simpler $\C{O}(r^d)$) 
operations, and no change in rank and storage.
%
\paragraph{Addition of two Tucker tensors} is computed as follows:
\begin{align*}
\tnb{w}  &= \tnb{u}+\tnb{v}= 
  \sum_{\vek{\mu}}^{\vek{\rho}} \Shat{u}_{\vek{\mu}} \bigotimes_{i=1}^d \vek{u}^{(i)}_{\mu_i}
  + \sum_{\vek{\nu}}^{\vek{r}} \Shat{v}_{\vek{\nu}} \bigotimes_{i=1}^d \vek{v}^{(i)}_{\nu_i}  \\
  \nonumber
  &= \sum_{\vek{\mu}}^{\vek{\rho}+\vek{r}} \Shat{w}_{\vek{\mu}}
     \bigotimes_{i=1}^d \vek{w}^{(i)}_{\mu_i}, \quad
     \text{--- with }  \vek{\mu} = (\mu_1,\dots,\mu_d), \text{ and similarly } 
     \vek{\nu}, \vek{\rho}, \vek{r} \text{ ---}
\end{align*}
and where the core tensor $\That{w}=(\Shat{w}_{\mu_1,\ldots,\mu_d})\in  
\D{R}^{(\rho_1+r_1)} \otimes\ldots \otimes \D{R}^{(\rho_d+r_d)}$
of order $d$ consists of the two blocks of core tensors $\That{u}$ and $\That{v}$, i.e.\ 
$(\Shat{u}_{\mu_1,\ldots,\mu_d}), (\Shat{v}_{\mu_1,\ldots,\mu_d})$ on the main diagonal.
In more detail
\begin{equation*}
\Shat{w}_{\mu_1,\ldots,\mu_d} = \begin{cases} 
      \Shat{u}_{\mu_1,\ldots,\mu_d} &\text{if }   \mu_1\le\rho_1,\ldots,\mu_d\le\rho_d \\
      \Shat{v}_{\mu_1-\rho_1,\ldots,\mu_d-\rho_d} &\text{if }
      0< \mu_1-\rho_1\le r_1,\ldots,0<\mu_d-\rho_d\le r_d       \\
      0 &\text{otherwise}. 
   \end{cases}
\end{equation*}

Similarly, the vectors $\vek{w}^{(i)}_{\mu_i} \in \D{R}^{M_i}$ are constructed from 
$\vek{u}^{(i)}_{\mu_i}\in \D{R}^{M_i}$ and $\vek{v}^{(i)}_{\nu_i} \in \D{R}^{M_i}$
as follows for $i=1,\dots,d$ and $\mu_i = 1,\dots,\rho_i+r_i$:
\begin{equation*}
\vek{w}^{(i)}_{\mu_i} = \begin{cases} 
      \vek{u}^{(i)}_{\mu_i}        &\text{ if } \mu_i\le\rho_i \\
      \vek{v}^{(i)}_{\mu_i-\rho_i} &\text{if } 0<\mu_i-\rho_i\le r_i . 
   \end{cases}
\end{equation*}
For details see \citep{HA12, khorBook18}.
The computational cost is again $\C{O}(1)$ since only more memory needs to be allocated,
but the rank generally increases to the sum of the individual ranks of $\tnb{u}$ and $\tnb{v}$.



\paragraph{The Hadamard product} of two tensors given in Tucker format is computed
 as follows:
\begin{equation*}
 \tnb{u}\odot\tnb{v}:=\sum_{\nu}^{\vek{r}_u}
 \sum\limits_{\mu }^{\vek{r}_v}
 \Shat{u}_{\nu_1, \ldots ,\nu_d}
 \Shat{v}_{\mu_1, \ldots ,\mu_d}\, \bigotimes_{i=1}^d
\left({\vek{u}}^{(i)}_{\nu_i}\odot {\vek{v}}^{(i)}_{\mu_i}\right).
\end{equation*}
Note \citep{khoromskaia2018tensor} that the new Tucker core has size $r^{2d}$,
i.e.\ the ranks get multiplied.
The storage cost of the Hadamard product is $\C{O}(d\,r^2\,n+r^{2d})$.
%\textbf{Matrix-by-vector product.}\\


\paragraph{The Euclidean inner product} is computed as follows:
\begin{equation*}
\bkt{\tnb{u}}{\tnb{v}}_{\C{T}}:=\sum_{\nu}^{\vek{r}_u}  \sum_{\mu }^{\vek{r}_v}
 \Shat{u}_{\nu_1, \ldots ,\nu_d}  \Shat{v}_{\mu_1, \ldots ,\mu_d}\,
\prod_{i=1}^d    \bkt{\vek{u}^{(i)}_{\mu_i}}{\vek{v}^{(i)}_{\nu_i}}_{\C{P}_i}.
\end{equation*}
The overall computational complexity of the inner product is $\C{O}(d\,n\,r^2+r^{2d})$.\\


\subsubsection{Rank truncation in the Tucker format}
%
To truncate the Tucker tensor rank from $2r$ or $r^2$ back to $r$ the high order SVD 
(HOSVD) algorithm together with ALS iterations are applied \citep{DMV-SIAM2:00}.
As the set of Tucker tensors of fixed rank is closed, the best approximation exist, 
and there is an algorithm with quadratic convergence in the energy norm.
One may compare this to the matrix case, where the SVD yields a best low-rank 
approximation. %[R.A.Horn and C.R. Johnson, Sec. 7.4.9]
The truncated tensor $\tnb{w}^*$ resulting from the HOSVD could be sub-optimal, 
but nevertheless the following inequality holds
\begin{equation}
\label{eq:minim_prob}
\Vert \tnb{w} - \tnb{w}^*\Vert \leq \sqrt{d}\cdot \min_{\tnb{v}\in 
%  U_{T,\vek{r}}(k_1,...,k_d)} \Vert \tnb{w} -\tnb{v}\Vert. 
\tns{U}_{\Tuck,\vek{r}}(\tnb{P})} \Vert \tnb{w} -\tnb{v}\Vert. 
\end{equation}
For some improved estimates see \citep{Tucker_trunk12}.

The most time-consuming part of the Tucker algorithm is the HOSVD procedure. 
Namely, the computation of the initial guess using
the SVD of the matrix unfolding of the original tensor \citep{DMV-SIAM2:00}. 
The numerical cost of Tucker decomposition for full size tensors is 
$\C{O}(n^{d+1})$. 
%
%

%\textcolor{red}{Add pictures about CP, Tucker and TT formats.}\\
%\textcolor{red}{Addition in Tucker format to add}\\
%\textcolor{red}{PUT THE SAME ORDER OF SECTIONS}\\

%
%
%  $Log: TuckerFormat.tex,v $
%  Revision 1.2  2021/11/07 22:17:44  hgm
%  as obtained 7-11-2021
%
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 





==> chaptersV2/abstractV2.tex <==
% !TEX root = ../Rev2_13May2022.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: abstract.tex,v 2.3 2022/05/19 23:42:04 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 2.3 $",
%%  DATE      = "$Date: 2022/05/19 23:42:04 $",
%%  FILENAME  = "$RCSfile: abstract.tex,v $"}



\abstract[Abstract]{
Very often, in the course of uncertainty quantification tasks or 
data analysis, one has to deal with high-dimensional random variables.
Here the interest is mainly to compute characterisations like the entropy, 
the Kullback-Leibler divergence, more general $f$-divergences, or other such characteristics based on
the probability density.  The density is often not available directly, 
and it is a computational challenge to just represent it in a numerically
feasible fashion in case the dimension  is even moderately large.   It
is an even stronger numerical challenge to then actually compute said characteristics
in the high-dimensional case.  
In this regard it is proposed
to approximate the discretised density in a compressed form, in 
particular by a low-rank tensor.
This can alternatively be obtained from the corresponding 
probability characteristic function,
or more general representations of the underlying random variable.

The mentioned characterisations need
point-wise functions like the logarithm.  
This normally rather trivial task becomes computationally difficult
when the density is approximated in a compressed resp.\ low-rank tensor 
format, as the point values are not directly accessible.
The computations become possible by considering the compressed data 
as an element of an associative, commutative algebra with an inner product,
and using matrix algorithms to accomplish the mentioned tasks.
The representation as a low-rank element of a high
order tensor space allows to reduce the computational complexity and storage cost from 
exponential in the dimension to almost linear.  
}



%\vspace{1em}
%{\noindent\textbf{Keywords:} \thekeywords}
%\keywords{high-dimensional probability density, Kullback-Leibler divergence, f-divergence, tensor representation, computational algorithms, low-rank approximation}
\keywords{\thekeywords}

%\vspace{1em}
%{\noindent\textbf{MSC Classification:} \thesubject}





%  $Log: abstract.tex,v $
%  Revision 2.3  2022/05/19 23:42:04  hgm
%  shortening for V2
%
%  Revision 2.2  2022/05/17 06:53:22  hgm
%  shortened
%
%  Revision 2.1  2022/05/16 21:08:05  hgm
%  to be made shorter
%
%  Revision 1.15  2021/11/12 21:50:21  hgm
%  small changes
%
%  Revision 1.14  2021/11/07 22:21:06  hgm
%  added header and footer
%
%  Revision 1.13  2021/11/07 21:50:36  hgm
%  as obtained 7-11-2021
%
%  Revision 1.12  2021/08/03 18:29:57  hgm
%  small changes
%
%  Revision 1.11  2021/04/01 08:56:02  hgm
%  small changes
%
%  Revision 1.10  2019/06/10 01:21:48  hgm
%  runs
%
%  Revision 1.9  2019/06/09 10:27:59  hgm
%  for new article
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Rev2_13May2022"
%%% End: 


==> chaptersV2/algorithms_21_12_2020.tex <==
% !TEX root = ../19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: algorithms.tex,v 1.1 2019/07/07 10:40:09 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.1 $",
%%  DATE      = "$Date: 2019/07/07 10:40:09 $",
%%  FILENAME  = "$RCSfile: algorithms.tex,v $"}

%
%
\section{Algorithms} \label{S:algs}
%
This section gives the algorithms to actually compute functions from Table~\ref{table:f-divergence}.
\HGMc{This is what it is about already now, but it has to be expanded,
and the notation has to be adjusted.  Iteration and series was already
touched on in sect. 2, but now this should cover all the functions needed,
and also explain TT-cross.}

Very often not only the density $p_{\vX}(\by)$ is of interest, but functions of density, e.g., the $f$-divergence or the entropy. 
Below we will list algorithms, which approximate $f(p_{\vX}(\by))$ by $f(\tnb{P})$, where 
\begin{equation*}
f(\cdot)=\{\sign(\cdot), (\cdot)^{-1}, \sqrt{\cdot}, \sqrt[p]{\cdot}, (\cdot)^k, \log{(\cdot)},\exp{(\cdot)},(\cdot)^2, \vert \cdot \vert\},
\end{equation*}
$k>0$, and
$\tnb{P}$ a tensor which represents the samples of $p_{\vX}(\by)$, i.e.\
$\tnb{P} = p_{\vX}(\That{Y})=
\sum_{j=1}^{r_p} \Ten_{\nu=1}^d 
\vek{p}_{j}^{(\nu)}$.
We will also need the characteristic function of a set, and the level 
set function. \HGMc{Should be explained after where the $\sign$ function is, together with absolute value.  
And the $p$-th root we need for scaling!}

% We remind iterative algorithms to compute pointwise tensors
% $\sign(\tnb{P})$, ${\tnb{P}}^{-1}$, $\sqrt{\tnb{P}},\log(\tnb{P}),\exp{(\tnb{P})}$, and $\tnb{P}^2$.
These algorithms are non-trivial and their detailed consideration is out of scope of
this work. Possible difficulties, which may appear are:
the intermediate tensor ranks of iterates may become very large, the stable rank truncation procedure is neither not available or very computationally intensive, problem to chose the starting value $\tnb{X}_0$.


\subsection{Discretisation}  \label{SS:discret}
%
\ALc{!!!See please Section 2.3.1 on page 15. We have already partially described discretisation!!!}
\HGM{Discretisation for the \pdf and the \pcf should go here.  Considerations for the Fourier transform also}.
In this section we explain how we discretise the \pdf and the \pcf 
from \refeq{eq:p} and \refeq{eq:pcf2}. We introduce $d$-dimensional tensor grids for $\bt$ and $\bx$.
Let there is a following regular discretization in $\ell$-th dimension
$\tau_{\ell}=\{t_1^{(\ell)},..., t_{n_{\ell}}^{(\ell)}\}$, $\ell=1,\dots,d$. We do not require these 1d grids to be equidistant. Then the whole grid can be defined as the following product
\begin{equation}  \label{eq:T}
%\bigotimes\mT=\left[ \mT_{\beta}\right]=
\mT:=\tau_1\times\tau_2\times...\times \tau_d=
\bigotimes_{\ell=1}^d \tau_{\ell}\in \mathbb{R}^{n_1\times n_2 ... \times n_d},\,\quad \tau_{\ell}\in \mathbb{R}^{n_{\ell}},  
%\bigotimes_{\ell=1}^dt_{\beta_{\ell}},\quad t_{\beta_{\ell}}\in \mathbb{R}^{n_{\ell}},  
\end{equation}
The grid $\mT$ contains $N:=n_1\times... \times n_{d}$ nodes.
%each node has $d$ coordinates
Each nodal point $\vek{t}\in  \mT$ is indexed by a $d$-tuple $i_1,...,i_d$ with $1\leq i_{\ell} \leq n_{\ell}$: $\vek{t}(i_1,...,i_d)=(t_{i_1}^{1},...,t_{i_d}^{d})$.
% A grid function $u$ defined on $\mT$ is characterized by the nodal values $u[i_1,...,i_d]\in \mathbb{R}^N$. There is an isomorphysm 
% \begin{equation}
% \mathbb{R}^N\simeq \mathbb{R}^{n_1}\otimes...\otimes \mathbb{R}^{n_d}.
% \end{equation}

% Another Notation: $\tau_{\ell}=[t_{1,\ell},...,t_{\beta_{\ell},\ell},...,t_{n_{\ell},\ell}]^T\in \mathbb{R}^{n_{\ell}}$.
% Each node has $d$ coordinates and can be described by the multi-index $\beta=(\beta_1,...,\beta_d)$, $\beta_{\ell}=1..n_{\ell}$.
% Let us say that $\beta \in \mathcal{I}_{\beta}$, where $\mathcal{I}_{\beta}:=\{(\beta_1,...,\beta_d),\quad \vert \beta_{\ell}\in{1,...,n_{\ell}}\}$.
% \\ 




\subsection{Consistency of data}  \label{SS:consistency}
%
Making sure the data one works with is consistent is of great importance, and
should be checked before any other computations.  This was already touched upon at the
end of \refSSS{conv-Hada-tens} and in \refSSS{func-of-tens}.  We recall that
for the continuous case, the \pdf has to be in the set $\F{D}$ (\refeq{eq:set-prob-dens-fct}),
and the \pcf has to be in the set $\F{C}$ (\refeq{eq:set-char-fct}).

The \pdf is real valued, and the Fourier transform (FT) translates this into the
\pcf being Hermitean \refeq{eq:FT-real-hermite}.  The discrete FT preserves these
properties.  And as the FT is applied to the low-rank approximation without any
approximation in \refeq{eq:FT-grid-char-LR}, these properties are preserved also
in the low-rank representation.  Now checking that the \pcf is Hermitean is
directly not easy in the low-rank representation.  On the other hand, for the \pdf
one only has to make sure that the imaginary part is zero --- it does not even
have to be represented.  So this condition is most easily checked on the \pdf.

The next condition is that the \pdf is non-negative, and the Fourier transform (FT)
translates this into the \pcf being positive definite, see the relation in
\refeq{eq:FT-pos-posdef} which is preserved also by the discrete FT.  
It was already stated that for the \pcf tensor $\tnb{\Phi}$, resulting from the 
\pdf tensor $\tnb{P}$, being positive definite means that the convolution
operator $\tnb{K}_{\tnb{\Phi}}$ 
mentioned earlier in \refSSS{conv-Hada-tens} is positive definite.  
In \refSSS{func-of-tens} it was concluded that its spectrum are the values of the
\pdf tensor $\tnb{P}$.  Hence, to check positive definiteness is easiest by checking
that $\tnb{P}\ge 0$.  It will be shown in \refS{algs} that it is possible to
compute the functions $\max(\tnb{P})$ and $\min(\tnb{P})$.  The linear maps
$\tnb{K}_{\tnb{\Phi}}$ and $\tnb{L}_{\tnb{P}}$ are positive definite iff $\min(\tnb{P})\ge 0$.
In case this condition is not satisfied, a possible remedy was already indicated in
\refSSS{func-of-tens}: compute the level set function $\Lambda_U$ from \refSSS{func-of-tens}
for the level set $U=]-\infty, 0]$, and for a corrected \pdf tensor $\tnb{P}_c$ set 
\begin{equation}  \label{eq:corr-P-tens-neg}
   \tnb{P}_c := \tnb{P} - \Lambda_U(\tnb{P}).
\end{equation}
This new approximation has all the faulty negative values removed, so that
$\tnb{P}_c \ge 0$.  This change will not affect the Hermitean or self-adjoint
character discussed earlier.  Having satisfied this condition we turn to the next,
which can be affected by \refeq{eq:corr-P-tens-neg}.

This condition is the requirement that the \pdf integrate to unity, or equivalently
(see \refeq{eq:FT-unitint-unit}), that the \pcf takes the value one at the origin.
This condition should be preserved by the discrete approximation.  It was already
formulated at the very end of \refSSS{conv-Hada-tens}, namely the requirement
that $\tnb{\Phi}_{\vek{j}^0} = \tns{\Phi}_{j_1^0,\dots,j_d^0} = 1$.  Completely equivalents
is the condition that the discrete integral \refeq{eq:discr-int} of the \pdf tensor is unity,
i.e.\ $\C{S}(\tnb{P})=1$.  In case this is not satisfied, say $\tnb{\Phi}_{\vek{j}^0} =
\C{S}(\tnb{P})=\beta \ne 1$, for a re-scaled $\tnb{P}_s$ one may set
\begin{equation}  \label{eq:corr-P-tens-one}
   \tnb{P}^{(s)} := \tnb{P} / \beta.
\end{equation}
If one recomputes then the \pcf tensor $\tnb{\Phi}^{(s)} = \Fd(\tnb{P}^{(s)})$, it will
also satisfy $\tnb{\Phi}^{(s)}_{\vek{j}^0} =1$.



\subsection{Overview of methods to compute tensor functions}  \label{SS:comp-tens}
%
There are many methods to compute $f(\tnb{v})$. The exponential sums to
compute ${\tnb{v}}^{-1}$ in $[1,R]$, $1 \leq R \leq \infty$, are implemented
in \cite{BraessHack05,Beylkin05}. Some other methods and estimates are developed in \citep{Grasedyck2004, Hack06_Kron_nonlocal, Khor06_StruckRank}.
The function ${\tnb{v}}^{-1/2}$ was
computed in \cite{khorBook18,Khor06_StruckRank} and
 ${\tnb{v}}^{-\mu}$ in \cite{KhorTensors07,Khor06_StruckRank}.
The quadrature rules for computing the Dunford-Cauchy contour integral 
%\begin{equation}
%    f(\tnb{A})=\frac{1}{2\pi i}\int_\Gamma f(z)(z\tnb{I}-\tnb{A})^{-1}dz
%\end{equation}
is presented in \citep{GAHAKH03,GAHAKH05,HKTP,LowKroneker,litv17Tensor, khorBook18}.
The Newton and Newton-Schultz iterative methods are used in
\citep{EspigDiss, Espig2012VarCal, TensorCalEspig, Espig:2013, ESHAROSCH09_1,
  ESHALIMA11_1, ESHA10_3}. The inversion in the Tucker format is done by the
Newton–Schultz approximate iterations in \citep{Oseledets2009}.
The Tucker cross algorithm to approximate $\tnb{v}^{-1}$
was used in \citep{OselSavoTyrt08}.  In \citep{Savo08}, the multigrid Cross 3D
algorithm is used to calculate the Gauss polynomial. In \citep{Osel10_Cross}
iterative methods in the Tucker format are used to compute $ \tnb{v}^{1/3}$.
In \citep{BallaniGrasedyck2015, EspigGrasedyckHackbusch2009}, the authors are using the cross method for the Hierarchical
Tucker format to estimate various functionals of the solution in the UQ context.
In \citep{HeidelKhor18, litv17Tensor} the sinc quadrature is used to compute fractional
derivatives of the $d$-dimensional Laplace operator.
The TT approximation of the sign function was computed in
\citep{dolgov2015polynomial, dolgov2014computation}, but the TT ranks were large.
The pointwise inverse, level sets, sign functions are defined and computed in \citep{ESHALIMA11_1}.
The pointwise inverse is required for computing pointwise functions
$\sign(\tnb{v})$ and $\sqrt{\tnb{v}}$, \citep{ESHALIMA11_1}. The Newton algorithm for computing $\sign(\tnb{v})$ and $\exp(-\tnb{v})$, its convergence and error analysis for hierarchical matrices were considered in \citep{Grasedyck03_Riccati}.

%

Below we adapted and listed the classical matrix algorithms, described in \citep{NHigham}, for computing tensor-functions listed above.
%

%
%In this section we discuss how, having \pdfs and \pcfs in a low-rank tensor format, to calculate various statistics and QoIs.
%


%
\subsection{Iterative methods} \label{SS:itrunc}
%
{We want to compute $f(\tnb{w})$ for some function $f:\C{T}\to\C{T}$ from the list at the beginning of this section. We describe how to do it through iteration (see also \cite{Matthies2020}).  Thus we have an iteration function $\tns{\Psi}_f$, 
which only uses operations from the Hadamard algebra on $\C{T}$, and which is iterated, 
$\tnb{v}_{i+1}=\tns{\Psi}_f(\tnb{v}_i)$, and converges to a fixed point $\tns{\Psi}_f(\tnb{v}_*)=\tnb{v}_*$. 
When started with a $\tnb{v}_0$ depending on $\tnb{w}$, the fixed point is $\lim_{i\to\infty} \tnb{v}_i = \tnb{v}_* =\tns{\Psi}_f(\tnb{v}_*)= f(\tnb{w})$.}
A Newton-type family of high-order iterative methods for some matrix functions
was discussed in \cite{Newton18}.

%\paragraph{Iteration with Truncation} 
\ALc{Took from recent JCP paper \citep{Matthies2020}. It will be modified and reduced.}\\
While performing algebraic operations on tensors in some compressed format, the tensor ranks are increasing. To keep computational cost low a tensor compression 
after each or after a number of algebraic operations
may be necessary. 
We perform the \emph{truncation}
$\tns{T}_\epsilon$ to \emph{low rank} $r$ with error $\epsilon$
\citep{HA12, Espig:2013}.
We thus allow that the algebraic operations are possibly
only executed approximately.
%\HGMs{The theoretical convergence rate of iterative methods may become smaller.}{}



\subsubsection{Perturbed iteration} \label{SSS:pert_iter}
%
Thus, we speak about \emph{perturbed iteration} \citep{whBKhEET:2008,
Zander10}, where the standard iteration map
$\tns{\Psi}_f$ is replaced by $\tns{T}_\epsilon \circ \tns{\Psi}_f$.

The general structure of the iterative
algorithms for a post-processing task $f$ 
or for an auxiliary function is shown in Algorithm~\ref{alg:basic}.
  Here we want to collect
some results for this kind of iteration.
\begin{algorithm}
  \caption{Iteration with truncation}
       \label{alg:basic}
   \begin{algorithmic}[1]    
    \State Start with some initial \emph{compressed} guess  $\tnb{v}_0=\tnb{w}$.
    \State $i\gets 0$
    \While  {\emph{no convergence}} 
       \State $\tnb{z}_{i} \gets \tns{\Psi}_f(\tnb{v}_i)$ \Comment{See Remark below}
       \Statex\Comment{ the iterator $\tns{\Psi}_f$ may \emph{deteriorate} the
                     compression level } 
       \If {compression level of $\tnb{z}_i$ is too bad} 
          \State $\tnb{v}_{i+1} \gets \tns{T}_\epsilon(\tnb{z}_i)$
          \Statex\Comment{ use \emph{truncation} $\tns{T}_\epsilon$ to
                                  compress $\tnb{z}_i$ with error $\epsilon$ }
       \Else
          \State $\tnb{v}_{i+1} \gets \tnb{z}_i$  
       \EndIf
       \State $i\gets i+1$
    \EndWhile 
  \end{algorithmic}
\end{algorithm}
For such a truncated or perturbed iteration as in  Algorithm~\ref{alg:basic},
it is known that
\begin{enumerate}
\item if the iteration by $\tns{\Psi}_f$ is \emph{super-linearly}
   convergent, the \emph{truncated iteration}  $\tns{T}_\epsilon \circ \tns{\Psi}_f$ will
   still \emph{converge} super-linearly, but finally \emph{stagnate} in an 
   $\epsilon$-neighbourhood of the fixed point $\tnb{v}_*$ \citep{whBKhEET:2008}.
   One could loosely say that the super-linear convergence of $\tns{\Psi}_f$ is
   stronger than the truncation by $\tns{T}_\epsilon$. 
\item if the iteration by $\tns{\Psi}_f$ is \emph{linearly} convergent with \emph{contraction}
   factor $q$, the \emph{truncated iteration}  $\tns{T}_\epsilon \circ \tns{\Psi}_f$ will
   still \emph{converge} linearly, but finally
   \emph{stagnate} in an $\epsilon/(1-q)$-neighbourhood
   of $\tnb{v}_*$ \citep{Zander10}.  Again, one could loosely say that
   iteration by $\tns{\Psi}_f$ and truncation by $\tns{T}_\epsilon$ balance each other,
   thus resulting in a larger neighbourhood of stagnation. 
\end{enumerate}

We shall assume that the truncation level has thus been chosen according to the
desired re-construction accuracy and taking into account the possible influence
due to the convergence behaviour of the iterator $\tns{\Psi}_f$.
\begin{remark}   \label{rem:too-big-rank}
In Algorithm~\ref{alg:basic} we assume that the tensor rank of $\tnb{z}_{i}$ is not increasing too much after applying 
the mapping $\tns{\Psi}_f$ to the tensor $\tnb{v}_i$. This could be a strong assumption. Additionally, we assume that there is a 
mapping $\tns{T}_\epsilon$, which is able to truncate the rank of $\tnb{z}_i$.
\end{remark}
{
\begin{remark}  \label{rem:starting-value}
In some of the iterations to follow, one fixed point $\tnb{v}_a = \tns{\Psi}_f(\tnb{v}_a)$ is often 
known a priori, often this is the identity $\tnb{v}_a = \tnb{1}$.
Since most iterative methods, e.g.\ Newton's method, do not converge unless the starting point is close to 
the fixed point, it is beneficial to artificially change the task at hand so that the desired fixed point
$\tnb{v}_*$ is close to an a priori known one $\tnb{v}_a$.  If $\tnb{v}_a = \tnb{1}$ this is particularly easy 
and can be achieved through scaling, i.e.\ $\tnb{v}_0 = \alpha\cdot\tnb{w}$ with a properly chosen $\alpha$.
\end{remark}
}


\subsubsection{Iteration functions} \label{SSS:iter-fcts}
%
{
The first function to consider is an auxiliary function which is needed for a different kind of ``scaling'', 
namely iterated squaring or iterated inverse squaring.  It will be used in subsequent algorithms.
In some of the algorithms the scaling factor involves e.g.\ $\nd{\tnb{w}}_\infty$, we shall show at the end of this section how to compute that.
}
%
%
%
\paragraph{Computing $\tnb{w}^{\odot m}$ for $m\in\D{Z}$.}
{This is a really simple and well know way to compute any \emph{integer power}, and at the same 
time make sure that no unnecessary multiplications are performed. 
The Algorithm~\ref{alg:pow-m} computes $\tnb{w}^{\odot m} = \tns{\Psi}_{\text{pow}}(m,\tnb{w})$ 
for positive and negative powers $m$ and takes note of possibilities to use squaring.}
\begin{algorithm}
  \caption{Computing $\tns{\Psi}_{\text{pow}}(m,\tnb{w})$}
       \label{alg:pow-m}
  \begin{algorithmic}[1]
     \Require $(m \ge 0)\; \vee \; (\tnb{w}^{\odot -1} \text{exists}$).
     \Ensure Output $\tnb{v} = \tnb{w}^{\odot m}$
     \State $\tnb{v} \gets \tnb{1}$
     \If {$m < 0$}
       \State $\tnb{x} \gets \tnb{w}^{\odot -1}$;
       \State $n \gets -m $
     \Else
       \State $\tnb{x} \gets \tnb{w}$
       \State $n \gets m$
     \EndIf
     \While {$n > 0$} 
       \If{$n$ is even}
          \State $\tnb{x} \gets \tnb{x} \odot \tnb{x}$
          \State $n \gets n/2$
       \Else   
          \Statex\Comment{ $n$ is odd } 
          \State $\tnb{v} \gets \tnb{x} \odot \tnb{v}$
          \State $n \gets n-1$
       \EndIf
     \EndWhile
  \end{algorithmic}
\end{algorithm}
{
This is not really an iteration function to be used in Algorithm~\ref{alg:basic}, but it is iterative
in nature, and is an auxiliary function which is used in a few other algorithms and iteration functions.  For negative powers it 
needs $\tnb{w}^{\odot -1}$.  It is really only meaningfully used for $m>2$ or $m< -1$.
}
%
%
%
\ignore{
\paragraph{Computing $\tnb{w}^{\odot 2^k}$ or $\tnb{w}^{\odot -2^k}$ for $k\in\D{N}$}
{The basic function is really simple, but it will be reused several times:
\begin{equation}  \label{eq:square}
  \tns{\Psi}_2(\tnb{v}) = \tnb{v} \odot \tnb{v} .
\end{equation}
}
{
Then, to compute $\tns{\Psi}_{2^k}$, one executes the Algorithm~\ref{alg:2-exp-k-times}:}
\begin{algorithm}
  \caption{Computing $\tns{\Psi}_{2^k}$}
       \label{alg:2-exp-k-times}
  \begin{algorithmic}[1]
     \State Start with some input point $\tnb{v}_0$ and a $k\in\D{Z}$.
     \Require $k \ge 0$
     \Ensure Output $\tnb{v} = \tnb{v}_0^{\odot 2^k}$
     \If {$k = 0$}
       \State $\tnb{v} \gets \tnb{w}$;
       \Statex\Comment{ Only for completeness, no one should use this part. } 
     \ElsIf {$k>0$}
       \State $\tnb{v} \gets \tnb{w}^{\odot 2}$;
     \Else
       \State $\tnb{v} \gets \tnb{w}^{\odot -1}$;
     \EndIf
     \For{$i\gets 2$ to $k$} 
       \State $\tnb{v} \gets \tns{\Psi}_2(\tnb{v})$;
     \EndFor 
  \end{algorithmic}
\end{algorithm}
{This is not really an iterative algorithm, the ``iteration'' is executed exactly $k$ times. It is needed
for scaling in the computation of $\log$ and $\exp$.  The starting point is $\tnb{v}_0 = \tnb{w}$ for 
the computation of $\tnb{w}^{\odot 2^k}$ for $k\ge 0$, and
in case $\tnb{w}^{\odot -2^k}$ is wanted, one takes $\tnb{v}_0 = \tnb{w}^{\odot -1}$.
}
}
%
%
%
\paragraph{Computing $\tnb{w}^{\odot -1}$.}
Let $\tns{F}(\tnb{x}):=\tnb{w}-\tnb{x}^{\odot -1}$.  
{It is clear that for $\tnb{w}=\tnb{1}$ the solution is $\tns{F}(\tnb{1})=\tnb{0}$.  This means 
that  $\tnb{v}_a=\tnb{1}$ is one of the a priori known fixed points, see Remark~\ref{rem:starting-value}}
Applying Newton's method to $\tns{F}(\tnb{x})$ for approximating the inverse of a given tensor
$\tnb{w}$, one obtains \citep{Oseledets2009} the 
{following iteration function $\tns{\Psi}_{\odot-1}$ --- 
to be used with Algorithm~\ref{alg:basic} with the initial iterate $\tnb{v}_0=\alpha \cdot\tnb{w}$ 
to bring $\tnb{v}_0$ close to $\tnb{v}_a=\tnb{1}$}:
\begin{equation}  \label{eq:Newton-inverse}
    \tns{\Psi}_{\odot-1}(\tnb{v})= \tnb{v}\odot (2\cdot\tnb{1} − \tnb{v}_0 \odot \tnb{v}) .
\end{equation}
% \HGMs{
% In both, the exact and approximate (tensor) arithmetic this iteration has quadratic convergence rate. The requirement is that
% the initial residual
% }
{
The iteration converges if the initial iterate $\tnb{v}_0$ 
}
 satisfies $\nd{\tnb{1}−\tnb{w}\odot\tnb{v}_0}_\infty <1$.
\AL{A possible candidate for the starting value is $\tnb{v}_0=\alpha \tnb{w}$ with
% \HGMs{$\alpha$ a small number ($\alpha < (1 /\max(\tnb{v}))^{\odot 2}$)}
{$\alpha < (1 /\nd{\tnb{w}}_\infty)^2$}. 
For such a $\tnb{v}_0$, the convergence initial
condition  $\nd{\tnb{1} - \alpha \tnb{w}^{\odot 2}}_\infty <1$ is always satisfied.}
{As the initial iterate was scaled, the fixed point of the iteration is $\tnb{v}_* = (1/\alpha) \cdot \tnb{w}^{\odot -1}$, and
thus the final result is $\tnb{w}^{\odot -1} = \alpha \cdot \tnb{v}_*$.}

% \HGMs{To keep tensor ranks of $\tnb{v}_k$ under control we introduce a projection operator (or a rank truncation procedure)
% $\mathcal{P}$.  Then the Newton iteration looks like:
% \begin{equation}
% \tnb{Y}_{k+1}=2\tnb{X}_k − \tnb{X}_k \tnb{A} \tnb{X}_k,\quad \tnb{X}_{k+1}=\mathcal{P}(\tnb{Y}_{k+1}).
% \end{equation}
% }
{
We did not assume that $\tnb{w}$ is invertible, as the iteration actually computes the pseudo-inverse
(i.e.\ only the non-zero entries are inverted).  It is easily seen from \refeq{eq:Newton-inverse} that
with $\tnb{v}_0=\alpha \tnb{w}$ zero entries in $\tnb{w}$ stay zero during the iteration.
}
%
%
%
\paragraph{Computing $\sqrt{\tnb{w}}$ or $(\tnb{w})^{\odot -1/2}$.}
Let $\tns{F}(\tnb{x}):=\tnb{x}^{\odot  2} - \tnb{w} = 0$.
% \HGMs{
%  and $\tnb{\Delta}_k:=\tnb{x}_k - \tnb{x}_{k-1}$.
% }
{
We assume that $\tnb{w}\ge\tnb{0}$, and again 
it is clear that for $\tnb{w}=\tnb{1}$ the solution is $\tns{F}(\tnb{1})=\tnb{0}$,
so that $\tnb{v}_a=\tnb{1}$ is one of the a priori known fixed points, see Remark~\ref{rem:starting-value}.
The Newton iteration for the above function uses the iteration function \refeq{eq:Newton-sqrt-1} 
together with Algorithm~\ref{alg:basic}.
}
% \HGMs{
% \begin{equation}
% \tnb{x}_{k-1}\tnb{\Delta}_{k}+\tnb{\Delta}_{k}\tnb{x}_{k-1}=\tnb{A}-\tnb{x}_{k-1}^2,\quad k=1,2,\ldots    
% \end{equation}
% or more stable iteration
% }
{
% Newton iteration:
\begin{equation} \label{eq:Newton-sqrt-1}
  \tns{\Psi}_{\sqrt{}}(\tnb{v}) = \frac{1}{2} \cdot (\tnb{v} + \tnb{v}^{\odot -1}\tnb{w}) .
\end{equation}
The starting value can be $\tnb{v}_0 = (\tnb{w}+\tnb{1})/2$, other stating values
obtained through scaling are described later.
}
{
Unfortunately, \refeq{eq:Newton-sqrt-1} contains an inverse power $\tnb{v}^{\odot -1}$ and can thus
not be computed directly only with operations from the algebra.  Of course, one could use the just described
algorithm for the inverse, but this would involve a nested iteration, which is mostly not so advantageous.
The well known stable inversion free Newton-Schulz iteration \citep{NHigham} computes $\tnb{v}_*^+=\sqrt{\tnb{w}}=\tnb{w}^{\odot 1/2}$ 
and $\tnb{v}_*^-=(\sqrt{\tnb{w}})^{\odot -1}=\tnb{w}^{\odot -1/2}$ at the same time.
Hence we set $\tnb{V}_0 = [\tnb{y}_0, \tnb{z}_0] = [\alpha \cdot\tnb{w}, \tnb{1}] \in \C{T}^2$, and the iteration function is 
}
% \HGMs{
% \begin{equation}
% \tnb{Y}_{0}=\tnb{A}, \quad \tnb{Z}_0=\tnb{I},\\
% \tnb{Y}_{k+1}=\frac{1}{2}\tnb{Y}_k(3\tnb{I}-\tnb{Z}_k\tnb{Y}_k),\quad 
% \tnb{Z}_{k+1}=\frac{1}{2}(3\tnb{I}-\tnb{Z}_k\tnb{Y}_k)\tnb{Z}_k, \quad k=0,1,\ldots
% \end{equation}
% It is known that, for certain normalisation of $\tnb{A}$, we have quadratic convergence $\tnb{Y}_k\rightarrow \tnb{A}^{1/2},\quad \tnb{Z}_k\rightarrow \tnb{A}^{-1/2}$.
% }
{
best written using the auxiliary function $\tns{A}(\tnb{y},\tnb{z}) = 3\cdot\tnb{1} - \tnb{z}\odot\tnb{y}$:
\begin{equation}  \label{eq:Newton-sqrt}
    \tns{\Psi}_{\sqrt{}}\left(\begin{bmatrix}
       \tnb{y} \\ \tnb{z}
    \end{bmatrix}\right) = \frac{1}{2}\begin{bmatrix}
     \tnb{y}\odot\tns{A}(\tnb{y},\tnb{z}) \\  \tns{A}(\tnb{y},\tnb{z})\odot\tnb{z}
    \end{bmatrix} .
\end{equation}
}
{
The iteration converges to $\tnb{V}_* = [\tnb{v}_*^+, \tnb{v}_*^-] = [ \sqrt{\tnb{y}_0}, (\sqrt{\tnb{y}_0})^{\odot -1}] $
if $\nd{\tnb{1}-\tnb{y}_0}_\infty < 1$, which can be achieved with a scaling factor $\alpha < 1/\nd{\tnb{w}}_\infty$.  
As the initial iterate was scaled, the fixed point of the iteration is $\tnb{v}_*^+ = \sqrt{\alpha} \cdot \sqrt{\tnb{w}}$ and 
$\tnb{v}_*^- = (1/\sqrt{\alpha}) \cdot (\sqrt{\tnb{w}})^{\odot -1}$.  Thus the final result is
$\sqrt{\tnb{w}} = (1/\sqrt{\alpha}) \cdot \tnb{v}_*^+$ and
$(\sqrt{\tnb{w}})^{\odot -1} = \sqrt{\alpha} \cdot \tnb{v}_*^-$.
}
%
%
\paragraph{Computing \HGM{$\tnb{w}^{\odot 1/m}$ when $m\in\D{N}$}.}
{This function may be needed for logarithmic scaling purposes, see \refSS{series}.}
For the theory and required definitions see Section 7 in \citep{NHigham}.
A new family of high-order iterative methods for the matrix $m$-th root was suggested in \citep{pthroot15}. 

To compute the principal $m$-th root of $\tnb{w}$,
{where it is assumed that $\tnb{w}\ge\tnb{0}$, one considers}
Newton's method for $\tns{F}(\tnb{x}) = \tnb{x}^{\odot m}-\tnb{w}=0$.
{Again it is clear that for $\tnb{w}=\tnb{1}$ the solution is $\tns{F}(\tnb{1})=\tnb{0}$,
so that $\tnb{v}_a=\tnb{1}$ is one of the a priori known fixed points, see Remark~\ref{rem:starting-value}.  The iteration function with $\tnb{v}=\tnb{w}$}
{corresponding to \refeq{eq:Newton-sqrt-1}} looks like
% \HGMs{
% \begin{equation}
%     \tnb{X}_{k+1} = \frac{1}{p} \left [ (p-1)\tnb{X}_k + \tnb{X}_k^{1-p}\tnb{A} \right], \quad \tnb{X}_0\tnb{A}=\tnb{A}\tnb{X}_0.
% \end{equation}
% }
{
\begin{equation}  \label{eq:Newton-p-root}
    \tns{\Psi}_{m-\text{root}}(\tnb{v}) = \frac{1}{m} \left( (m-1)\cdot\tnb{v} + \tns{\Psi}_{\text{pow}}(1-m,\tnb{v})\odot\tnb{v}_0 \right) .
\end{equation}
}
{If $m\ge2$, this involves a negative power $\tnb{v}^{\odot(1-m)}$.}
The convergence analysis is rather complicated, see more in Section 7.3, \citep{NHigham}{, but the algorithm converges for all $\tnb{w}\ge\tnb{0}$}.

%\HGM
{
Just as there is a more stable version \refeq{eq:Newton-sqrt} for $m=2$ avoiding inverses, so one has a ``double iteration'' \citep{NHigham} here as well.
It is best written using the auxiliary function $\tns{A}(\tnb{y},\tnb{z}) = (1/m)\cdot ((m+1)\cdot\tnb{1} - \tnb{z})$:
\begin{equation}  \label{eq:Newton-sqrt-p}
    \tns{\Psi}_{m-\text{root}}=\left(\begin{bmatrix}       \tnb{y} \\ \tnb{z}
    \end{bmatrix}\right) = \begin{bmatrix}
     \tnb{y}\odot\tns{A}(\tnb{y},\tnb{z}) \\  \tns{\Psi}_{\text{pow}}(m,\tns{A}(\tnb{y},\tnb{z}))\odot\tnb{z}
    \end{bmatrix} ,
\end{equation}
where $\tnb{y}_i \to \tnb{w}^{\odot -1/m}$.  The starting values are $\tnb{V}_0 = [\tnb{y}_0, \tnb{z}_0] = [\alpha \cdot\tnb{1}, (\alpha)^m \tnb{w}] \in \C{T}^2$, with $\alpha < (\nd{\tnb{w}}_\infty/\sqrt{2})^{-1/m}$.
For scaling purposes it is best used with $m=2^k$.
}
%
%
%
\paragraph{Computing $\sign(\tnb{w})$.}
% \HGMs{Let $f:\tnb{X}\mapsto \sign(\tnb{X})$. Applying the scaling Newton iteration to the equation}
{
The equation to be used for the Newton iteration is
}
$\tns{F}(\tnb{x}):=\tnb{x}\odot \tnb{x}-\tnb{1}$.  With starting value $\tnb{v}_0=\tnb{w}$ we obtain the following iteration function:
% \HGMs{
% \begin{equation}
% \tnb{X}_{k+1}=  \Phi(\tnb{X}_k),\quad  \Phi(\tnb{X}):=\frac{1}{2}(\mu\tnb{X}+\frac{1}{\mu}\tnb{X}^{\odot-1}),
% \end{equation}
% }
{
\begin{equation}  \label{eq:Newton-sign}
 \tns{\Psi}_{\sign}(\tnb{v})=\frac{1}{2}(\mu\cdot\tnb{v}+\frac{1}{\mu}\cdot\tnb{v}^{\odot-1}),
\end{equation}
}
with $\mu = \nd{\tnb{v}^{\odot-1}}_\infty / \nd{\tnb{v}}_\infty$ (see Section 8.6 in \citep{NHigham}).  This method converges to $\sign(\tnb{w})$.

Alternatively, one can rewrite this iteration function without computing $\tnb{v}^{\odot -1}$, namely
\begin{equation} \label{eq:Newton-Schulz-sign}
    \tns{\Psi}_{NS}(\tnb{v})=\frac{1}{2}\cdot\tnb{v} \odot ( 3\cdot \tnb{1}-\tnb{v}\odot \tnb{v} ) ,
\end{equation}
{with starting value $\tnb{v}_0 = \alpha\cdot \tnb{w}$,
where $\alpha = \nd{\tnb{w}^{\odot -1}}_\infty / \nd{\tnb{w}}_\infty$.}
The last formula is called the Newton-Schulz iteration, it has quadratic (local) convergence to 
$\sign(\tnb{w})$ \citep{EspigDiss,ESHALIMA11_1,ESHAHARS11_2,NHigham}.
%
%
%
\paragraph{Computing the absolute value $\ns{\tnb{w}}$}is simple if $\sign(\tnb{w})$ is available:
\[
\ns{\tnb{w}} = \tnb{w}\odot \sign{(\tnb{w})}.
\]
%
%
%

\paragraph{Computing the characteristic function of a set}  
is done as described in \refeq{eq:char-def-level} by using the shifted $\sign$-function \cite{ESHA09_1,ESHAHARS11_2,Matthies2020}.

%
%
%

\paragraph{Computing the level set function of a set}
is done by using the characteristic function \cite{ESHA09_1,ESHAHARS11_2,Matthies2020}:
\[
\Lambda_{U}(\tnb{w}) = \chi_{U}(\tnb{w}) \odot \tnb{w} .
\]
%
%
%
\paragraph{Computing $\nd{\tnb{w}}_\infty = \vrho(\tnb{w})$, $\max \tnb{w}$,
$\min \tnb{w}$.}
We need these values in all the algorithms, and also for checking the consistency. Particularly,
$\min \tnb{w}$ is needed for consistency.  Once one has achieved $\min \tnb{w} \ge \tnb{0}$, i.e.\ $\tnb{w}\ge \tnb{0}$, it follows that 
$\nd{\tnb{w}}_\infty = \vrho(\tnb{w})=\max \tnb{w}$. \HGM{This means we have to describe the eigenvalue algorithms,
preferably only the one with squaring which has exponential convergence.
Here we assume that $\tnb{w}\ge \tnb{0}$.  In that case one has $\nd{\tnb{w}}_\infty = \vrho(\tnb{w}) = \max \tnb{w}$.}

\HGMc{This is all from the JCP paper and need to be reformulated:}
\paragraph{``Exponentiating'' the power iteration.}  This can be easily achieved
via the clever idea of \citep{Grasedyck-gamm}. Recall that with the starting
vector $\tnb{v}_0:=\tnb{1}/\sqrt{N}$, power iteration would compute 
$\tnb{v}_1 \propto \tnb{w}^{\odot 1}=\tnb{w}^{\odot 1}\odot \tnb{1}$,
a scaled version of $\tnb{w}$,
corresponding to the action of $\tnb{w}^{\odot 1}$ on $\tnb{1}$.  
Starting actually with $\tnb{v}_0\propto\tnb{w}$ and 
changing line 2 in Algorithm~\ref{alg:power-it} or Algorithm~\ref{alg:power-RQ}
to $\tnb{u} := \tnb{v}_i^{\odot 2}$, one has $\tnb{v}_1 \propto \tnb{w}^{\odot 2}=
\tnb{w}^{\odot 2}\odot\tnb{1}$, i.e.\ the action of $\tnb{w}^{\odot 2}$ on $\tnb{1}$.
In the next iteration
one has $\tnb{v}_2 \propto \tnb{w}^{\odot 4}$, and in iteration $i$
one has $\tnb{v}_i \propto \tnb{w}^{\odot 2^i}$.
Reformulating Algorithm~\ref{alg:power-RQ} for this new task of
``exponentiated'' power iteration ($P\gets\text{exp-pow}$)
for the new iteration function $\tns{\Phi}_{\text{exp-pow}}$ results 
in Algorithm~\ref{alg:exp-pow}, to be used in Algorithm~\ref{alg:basic}
with starting vector $\tnb{v}_0 := \tnb{w}/\nd{\tnb{w}}_{\C{T}}$.
We also need to keep the auxiliary vector $\tnb{y}=\tnb{w}^{\odot 2}$.

\begin{algorithm}
  \caption{One step ``exponentiated'' power iteration with RQ: $\tns{\Phi}_{\text{exp-pow}}$}
       \label{alg:exp-pow}
   \begin{algorithmic}[1]     
    \State Input iterate $\tnb{v}_i$;
    \Comment{ assume $\tnb{v}_i \propto \tnb{w}^{\odot 2^{i}}$ of unit length. }
    \State $\tnb{u} \gets \tnb{v}_i \odot \tnb{v}_i$;
    \Comment{ $\tnb{u} \propto \tnb{L}_{\tnb{w}}^{\odot 2^{i+1}} \tnb{1}=\tnb{w}^{\odot 2^{i+1}}$.}
    \State $\vrho_1 \gets \bkt{\tnb{w}}{\tnb{u}}_{\C{T}}$; 
    \Comment{ Rayleigh quotient (RQ) $\lambda_1 \approx \vrho_1$ }
    \State $\vrho_2 \gets \bkt{\tnb{y}}{\tnb{u}}_{\C{T}}$; 
    \Comment{ RQ of $\tnb{w}^{\odot 2}$. }
    \State $\vepsilon_\lambda \gets (\vrho_2-\vrho_1^2)^{1/2}$; 
    \Comment{ error bound \refeq{eq:kryl-bogo-2} of $\lambda_1$. }
    \State $\gamma \gets \bkt{\tnb{u}}{\tnb{u}}_{\C{T}}^{-1/2}$; 
    \Comment{ inverse length of $\tnb{u}$. }
    \State $\tnb{z} \gets \gamma\;\cdot \tnb{u}$;
    \Comment{ normalise output $\tnb{z}$ to unit length. }
    \State Output $\tnb{z}$;
  \end{algorithmic}
\end{algorithm}

Thus the eigenvalue approximation is through the Rayleigh quotient
$\vrho_1 = \bkt{\tnb{w}}{\tnb{u}}_{\C{T}} = \bkt{\tnb{w}}{\tnb{v}_i^{\odot 2}}_{\C{T}}
= \bkt{\tnb{w}\odot\tnb{v}_i}{\tnb{v}_i}_{\C{T}}$ in line 3
of Algorithm~\ref{alg:exp-pow}.
As $\tnb{y}=\tnb{w}^{\odot 2}$, on line 4 the quantity
$\vrho_2= \bkt{\tnb{y}}{\tnb{u}}_{\C{T}} = 
\bkt{\tnb{w}^{\odot 2}}{\tnb{v}_i^{\odot 2}}_{\C{T}} = 
\bkt{\tnb{w}^{\odot 2}\odot\tnb{v}_i}{\tnb{v}_i}_{\C{T}}$ computes the RQ of 
$\tnb{w}^{\odot 2}$.  The ``eigenvector'' $\tnb{v}_i\propto\tnb{w}^{\odot 2^{i}}$
converges with the rate $|\lambda_2/\lambda_1|^{2^i}$, and hence one achieves
\emph{exponential} convergence.  This acceleration technique can be used in all
eigenvalue computations described here.


\paragraph{Transformed eigenvalue computations} are a well-known device
to find e.g.\ the maximum of the function $\tnb{y}=f(\tnb{w})$.  After
computing $f(\tnb{w})$, one proceeds as before, but with $\tnb{y}$
instead of $\tnb{w}$.  Some functions $f(t)$ are simple
enough so that the computation of $f(\tnb{w})$ is combined with the iteration.
Recall that this transforms all eigenvalues $\lambda_{\tnb{w}}$ to
$\lambda_{\tnb{y}}=f(\lambda_{\tnb{w}})$ according to spectral calculus,
leaving the eigenvectors unchanged.


\paragraph{Shifting and inverse shifting} are functions needed to access other than the
point of largest modulus in the spectrum of
$\tnb{L}_{\tnb{w}}$ resp.\ $\tnb{w}$.  These functions are the shift $f: t\mapsto t + \beta$
and the inverse shift $f:t \mapsto (t-\rho)^{-1}$.

The simple function of shifting $f(t) = t + \beta$ is needed
if the actual element of maximum modulus is a minimum of $\tnb{w}$;
then this is a maximum of $-\tnb{w}$.  In the iteration this will be picked up
by the Rayleigh-quotient being negative: $\vrho_{\tnb{w}} < 0$.
Also note that for this case --- where the maximum has smaller absolute
value than the minimum --- one may \emph{shift} the tensor by
a value of $\beta = - \vrho_{\tnb{w}} \approx -\lambda_1$ to
$\That{w}:=\tnb{w}+ \beta\cdot\tnb{1}$ so that the
maximum of $\That{w}$ has larger absolute value than the minimum of
$\That{w}$.  One then iterates with $\That{w}$.
After determining the maximum of $\That{w}$,
we may subtract the number $\beta>0$ again to obtain the maximum of $\tnb{w}$.
The index of the maximum of $\That{w}$ is of course the same as the
one for the maximum of $\tnb{w}$.  Completely analogous manipulations can
be performed to find a minimum which is not of maximum modulus. 
These and similar techniques are well known from eigenvalue
calculations of large / sparse symmetric matrices  
\citep{golubVanloan, parlett98, saad92, ds-watk-07}.

The  inverse shift $f(t)=(t-\rho)^{-1}$ is needed to access intermediate points
in the spectrum $\sigma(\tnb{w})$.  Here one finds the data in $\tnb{w}$
closest to $\rho$, as they have the maximum modulus under the transformation.
Thus one computes first $\tnb{y}:=(\tnb{w} - \rho\cdot\tnb{1})^{\odot-1}$
approximately through Algorithm~\ref{alg:basic} with the iteration
function \refeq{eq:iter-Had-inv} --- with $\Tcek{w} := \tnb{w} - \rho\cdot\tnb{1}$
instead of $\tnb{w}$ --- followed by the eigenvector computation
with iteration function as in Algorithm~\ref{alg:exp-pow}, but with
starting vector $\tnb{v}_0 := \tnb{y}/\nd{\tnb{y}}_{\C{T}}$. 



%
\subsection{Series expansions} \label{SS:series}
%
\paragraph{Computing $\log(\tnb{w})$.}



{We assume that $\tnb{w} > 0$.}
Various algorithms, improvement ideas, stability issues and tricks to compute $\log(\tnb{w})$  are discussed in \citep{HighamMLog01}.
Improved inverse scaling and squaring algorithms for the matrix logarithm were suggested later in \citep{Higham12}. We suggest to follow these works for the case when $\tnb{w}$ is a tensor. 
Stability of the matrix arithmetic-geometric mean iterations for computing the matrix logarithm is investigated in \citep{CompLog16}.
For the algorithms to work well, $\tnb{w}$ has to be close to the identity $\tnb{1}$, which can be achieved by taking roots:
for $\lambda \in [-1,1]$ one has $\log\left(\tnb{w}^\lambda\right) = \lambda \log \tnb{w}$.

From matrix calculus it is known \citep{HighamMLog01,Higham12} that one of the ways (for $\tnb{w}$ close to the identity) to compute $\log(\tnb{w})$ 
is to truncate the Taylor series {(radius of convergence  $\nd{\tnb{x}}_\infty < 1$)}:
\[
\log(\tnb{1}-\tnb{x})= - \sum_{n=1}^\infty \frac{1}{n} \cdot \tnb{x}^{\odot n}
%\tnb{x}-\tnb{x}^{\odot 2}/2-\tnb{x}^{\odot 3}/3-\ldots,
\]
where $\tnb{x}:=\tnb{1}-\tnb{w}$. If $\tnb{w}$ is not near to the identity, then $\log(\tnb{w})=2^k\log(\tnb{w}^{\odot 1/2^k})$, where $\tnb{w}^{\odot 1/2^k}\to \tnb{1}$ as $k$ increases \cite{kenney1989condition}.

Another way to compute the logarithm of a positive 
$\tnb{w}$ is Gregory's series  \citep{NHigham} {which converges for all $\tnb{w} > 0$:}
\[
   \log \tnb{w} = -2 \sum_{k=0}^\infty \frac{1}{2k+1} 
   \left((\tnb{1}-\tnb{w})\odot(\tnb{1}+\tnb{w})^{\odot -1}\right)^{\odot (2k+1)} .
\]
This involves $(\tnb{1}+\tnb{w})^{\odot -1}$, which should be computed only once.
% In \cite{Hack05_HKT}, the Kronecker ranks and error estimates of the Green's function $\log(x-y)$ of the 2D-Laplace operator are investigated. In \cite{Hack06_Kron_nonlocal}, the boundary elements method (BEM) kernel $\log(x+y)$ is approximated with a low-rank.
%
%
%
\paragraph{Computing $\exp(\tnb{w})$.}
The structured rank-$ (r_1,...,r_d) $ decompositions of function-related tensors,
particularly, $\exp(\tnb{w})$, and $\exp(-\tnb{w}^{\lambda})$, $\lambda \in \mathbb{R}_{>0}$,
are listed in \citep{Khor06_StruckRank}.
The one of the standard algorithms using the Taylor expansion
\[
  \exp{(\tnb{w})} = \sum_{k=0}^\infty \frac{1}{k!} \tnb{w}^k ,
\]
is explained in \cite{NHigham}.

{
Power series plus scaling and squaring.  Set
\[
  \tnb{u}_{r,s} = \left(\sum_{k=0}^r \frac{1}{k! s^k} \tnb{w}^{\odot k}\right)^{\odot s},
\]
then $\lim_{r\to\infty} \tnb{u}_{r,s}=\lim_{s\to\infty} \tnb{u}_{r,s}=\exp\tnb{w}$.  
It is of advantage to use $s$ from the series of powers of $2$, $s=1,2,4,\dots,2^k$, then the $s$-th power can be computed by squaring.  Best pick $s > \nd{\tnb{w}}_\infty$ for the scaling.
}
%
%

\input{\thetext/TT_approx.tex}

% \subsection{Algorithms from Prof. Matthies from Higham's book}

% %


% \[
%   \exp \vek{A} =  \lim_{k\to\infty} (\vek{I}+\vek{A}/k)^k ,
% \]
% \[
%   \exp \vek{A} =  \lim_{k\to\infty} \exp(\vek{A}/(2^k))^{2^k} ,
% \]
% \[
%   \exp \vek{A} = \int_\Gamma \ee^z (z\vek{I} - \vek{A})^{-1}\di z .
% \]

% Power series plus scaling and squaring.  Set
% \[
%  \vek{T}_{r,s} = \left(\sum_{k=0}^r \frac{1}{k!} (\vek{A}/s)^k\right)^s,
% \]
% then $\lim_{r\to\infty} \vek{T}_{r,s}=\lim_{s\to\infty} \vek{T}_{r,s}=\exp\vek{A}$.


% Algorithm 10.20 N.~Higham


% \paragraph{Matrix logarithm:}
% \[
%   \log \vek{A} = \int_0^1 (\vek{A}-\vek{I})[t(\vek{A}-\vek{I})+\vek{I}]^{-1}\di t
% \]
% For $\alpha\in [-1,1]$ one has $\log\left(\vek{A}^\alpha\right) = \alpha \log \vek{A}$

% Not so good (small radius of convergence) for $\vrho(\vek{A})<1$:
% \[
%   \log (\vek{I}+\vek{A}) =  \sum_{n=1}^\infty \frac{(-1)^{n+1}}{n} \vek{A}^n
% \]
% Gregory's series converges for all pos.def.\ matrices
% \[
%   \log \vek{A} = -2 \sum_{k=0}^\infty \frac{1}{2k+1} 
%   \left((\vek{I}-\vek{A})(\vek{I}+\vek{A})^{-1}\right)^{2k+1}
% \]

% Algorithm 11.10 N.~Higham


% \paragraph{Matrix square root:} first with inversion\\
% %

% Newton iteration:
% \[
%  \vek{X}_0 = \frac{1}{2} (\vek{A}+\vek{I}); \quad  
%  \vek{X}_{k+1}\gets \frac{1}{2} (\vek{X}_k + \vek{X}_k^{-1}\vek{A})
% \]

% %DB-Iteration: $\vek{X}_0 = \vek{A}$; $\vek{Y}_0 = \vek{I}$;
% %\begin{align*}
% %   \vek{X}_{k+1}&\gets  \frac{1}{2} (\vek{X}_k + \vek{Y}_k^{-1}), \\
% %   \vek{Y}_{k+1}&\gets  \frac{1}{2} (\vek{Y}_k + \vek{X}_k^{-1}), \\
% %   \lim_{k\to\infty} \vek{X}_k &= \vek{A}^{1/2}, \quad \lim_{k\to\infty} \vek{Y}_k=\vek{A}^{-1/2}.
% %\end{align*}

% Inversion free Newton-Schulz iteration: for  $\vrho(\vek{I}-\vek{A})<1$ and
% $\vek{Y}_0 = \vek{A}$; $\vek{Z}_0 = \vek{I}$;
% \begin{align*}
%   \vek{Y}_{k+1}&\gets  \frac{1}{2} \vek{Y}_k(3\vek{I}-\vek{Z}_k \vek{Y}_k), \\
%   \vek{X}_{k+1}&\gets  \frac{1}{2} (3\vek{I}-\vek{Z}_k \vek{Y}_k)\vek{Z}_k, \\
%   \lim_{k\to\infty} \vek{Y}_k &= \vek{A}^{1/2}, \quad\lim_{k\to\infty} \vek{Z}_k=\vek{A}^{-1/2}.
% \end{align*}

% Visser iteration:  let $0<\alpha<\vrho(\vek{A})^{-1/2}$, 
% \[
%  \vek{X}_0 = \frac{1}{2\alpha}\vek{I},\quad
%  \vek{X}_{k+1}\gets \vek{X}_k+\alpha(\vek{A} - \vek{X}_k^{2}).
% \]



% \paragraph{Matrix $p$-th root:} first with inversion\\
% %

% Newton iteration:  $\vek{X}_0 = \vek{A}$; $\lim_{k\to\infty} \vek{X}_k=\vek{A}^{1/p}$
% \[  
%  \vek{X}_{k+1}\gets \frac{1}{p} ((p-1)\vek{X}_k + \vek{X}_k^{1-p}\vek{A})
% \]

% Iteration: for $\vek{0}\le \vek{A} \le \vek{I}$, $\vek{X}_0 = \vek{A}$;
%  $\lim_{k\to\infty} \vek{X}_k = \vek{A}^{1/p}$
% \[
%   \vek{X}_{k+1}\gets  \vek{X}_k + \frac{1}{p} (\vek{A} - \vek{X}_k^{p}),
% \]

% Inverse $p$-th root Newton-Schulz iteration:
% $\vek{X}_0 = \vek{A}$;  $\lim_{k\to\infty} \vek{X}_k=\vek{A}^{-1/p}$.
% \[
%   \vek{X}_{k+1}\gets  \frac{1}{p} ((p+1)\vek{X}_k-\vek{X}_k^{p+1} \vek{A}) .
% \]





%  $Log: algorithms.tex,v $
%  Revision 1.1  2019/07/07 10:40:09  hgm
%  initial from AL
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 



  


==> chaptersV2/characteristic.tex <==
% !TEX root = ../19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: characteristic.tex,v 1.2 2021/11/07 21:53:00 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.2 $",
%%  DATE      = "$Date: 2021/11/07 21:53:00 $",
%%  FILENAME  = "$RCSfile: characteristic.tex,v $"}




\section{Characteristic function computed from PCE} \label{S:characteristic}
%
Now, when $\vphi_{\vX}(\bt)$ is computed on the grids $\mT$ and $\bTheta$, 
we write an expression for
the \pdf of $\vX$ on $\mathbb{R}^d$ as follows 
(repeat \refeq{eq:OM-space})
\begin{equation}  \label{eq:OM-space}
p_{\vX}(\by)=\frac{1}{(2\uppi)^d}\int_{{\R}^d}\exp(-\ii\ip{\by}{\bt})
  \vphi_{\vX}(\bt) \di\bt, \quad \by \in \D{R}^d.
\end{equation}
Now the idea is to sample $p_{\vX}(\by)$ to get enough samples for 
computing different statistics. But this can be expensive and therefore, 
to reduce the computational complexity we, first, find a low-rank 
approximation of the \pdf and only then will 
sample this low-rank surrogate/approximation.

Note that the difference of $\exp(-\ii \ip{\by}{\bt})$ from 
\refeq{eq:scp} is that the variable $\by \in \D{R}^d$ is not a random variable.

%\subsection{Low-rank tensor formats}
%

%
%
% \subsection{Cross interpolation of matrices}
% If $M=2$, the left-hand side of \eqref{eq:tt} can be seen as a matrix. 
%For simplicity we consider this case first.
% The basic assumption is that any entry of a matrix (or tensor) can be evaluated.
% However, to construct a TT approximation, we do not want to compute all elements,
% but only few of them.

% The principal ingredient for this is based on the efficiency of an incomplete
% Gaussian elimination in an approximation of a low-rank matrix, also known as the
% Adaptive Cross Approximation (ACA) \cite{bebe-2000,bebe-aca-2011}.
% Given is a matrix $\U=[\U(i,j)]\in\D{R}^{p \times q}$, we select some 
% ``good'' columns and rows to approximate the whole matrix,

% \begin{equation}
% \U(i,j) \approx \bm{\tilde U}(i,j)= \U(i,\J) \cdot \widehat \U^{-1} \cdot \U(\I,j),
% \label{eq:2dcross}
% \end{equation}
% where $\widehat \U = \U(\I, \J)$, and $\I \subset \{1,\ldots,p\}$, 
%$\J \subset \{1,\ldots,q\}$ are sets of indices of cardinality $r$, so e.g. 
% $\U(i,\J) \in \mathbb{R}^{1 \times r}$.
% It is known that there exists a quasi-optimal set of interpolating indices $\I,\J$.
% \begin{lemma}[Maximum volume (\emph{maxvol}) principle \cite{gt-maxvol-2001} ]
% $\;$ If $\I$ and $\J$ are such that $\mathrm{det}~\U(\I, \J)$ is maximal among 
% all $r \times r$ submatrices of $\U$, then
%  $$
%  \|\U-\bm{\tilde U}\|_C \le (r+1) \min_{\mathrm{rank}(\bm{V}) = r} \|\U-\bm{V}\|_2,
%  $$
% where $\| \cdot \|_C$ is the Chebyshev norm, $\|\bm{X}\|_C = \max_{i,j}|\bm{X}_{i,j}|$.
% \label{lem:maxvol}
% \end{lemma}

% In practice, however, the computation of the true maximum volume submatrix 
%is infeasible, since it is an NP-hard problem.
% Instead one performs a heuristic iteration in an alternating fashion 
% \citep{gostz-maxvol-2010}:
% we start with some (e.g. random) low-rank factor $\U^{(1)} \in 
% \D{R}^{p \times r}$, determine indices $\I$ yielding a quasi-maxvol 
% $r \times r$ submatrix in $\U^{(1)}$, and compute $\U^{(2)}$ as $r$ columns
% of $\U$ of the indices $\I$.
% Vice versa, in the next step we find quasi-maxvol column indices in $\U^{(2)}$
% and calculate corresponding $pr$ elements, collecting them into the newer $\U^{(1)}$,
% which hopefully approximates the true low-rank factor better than the initial guess.
% This process continues until the convergence, which appears to be quite satisfactory in practice.


% \subsection{TT-cross interpolation of tensors}

% In higher dimensions we recurrently proceed in the same way, since the TT format constitutes a recurrent matrix low-rank factorization.
% Let us merge the first $m$ and the last $M-m$ indices from $\alphab$.
% The corresponding TT blocks will induce the following matrices:

% \begin{definition}\label{def:interface}
% Given a TT format \eqref{eq:tt} and an index $m$.
% Define the \emph{left interface matrix} $\U^{<m} \in \mathbb{R}^{(p_1+1)\cdots(p_{m-1}+1) \times r_{m-1}}$ and the \emph{right interface} matrix $\U^{>m} \in \mathbb{R}^{r_m \times (p_{m+1}+1)\cdots(p_M+1)}$ as follows,
% \begin{equation*}
%  \begin{split}
%   \U^{<m}_{s_{m-1}}(\alpha_1,\ldots,\alpha_{m-1}) & = \sum\limits_{s_1=1}^{r_1} \cdots \sum\limits_{s_{m-2}=1}^{r_{m-2}} \u^{(1)}_{s_1}(\alpha_1) \cdots \u^{(m-1)}_{s_{m-2},s_{m-1}}(\alpha_{m-1}), \\
%   \U^{>m}_{s_{m}}(\alpha_{m+1},\ldots,\alpha_M) & = \sum\limits_{s_{m+1}=1}^{r_{m+1}} \cdots \sum\limits_{s_{M-1}=1}^{r_{M-1}} \u^{(m+1)}_{s_m,s_{m+1}}(\alpha_{m+1}) \cdots \u^{(M)}_{s_{M-1}}(\alpha_M).
%  \end{split}
% \end{equation*}
% \end{definition}

% Such matrices are convenient to relate high-dimensional TT expressions with their two-dimensional analogs.
% For example, the TT format \eqref{eq:tt} can be written in the following form,
% \begin{equation}
% \uh(\alphab) \approx \U^{<m}(\alpha_1,\ldots,\alpha_{m-1}) \cdot \u^{(m)}(\alpha_m) \cdot \U^{>m}(\alpha_{m+1},\ldots,\alpha_M).
% \label{eq:tt-l-b-r}
% \end{equation}
% The \emph{TT-cross} algorithm \cite{ot-ttcross-2010} assumes that the above expansion is valid on some $r_{m-1}(p_m+1)r_m$ indices, and can thus be seen as a system of equations on elements of $u^{(m)}$.
% Let us be given $r_{m-1}$ \emph{left} indices $(\hat\alpha_1,\ldots,\hat\alpha_{m-1}) \in \I^{(m-1)}$ and $r_m$ \emph{right} indices $(\hat\alpha_{m+1},\ldots,\hat\alpha_{M}) \in \J^{(m+1)}$.
% For the single index $\alpha_m$ we allow its full range $\{\alpha_m\} = \{0,1,\ldots,p_m\}$.
% Requiring that \eqref{eq:tt-l-b-r} is valid on the combined indices
% $$
% \left(\hat\alpha_1,\ldots,\hat\alpha_{m-1},\alpha_m,\hat\alpha_{m+1},\ldots,\hat\alpha_{M}\right) \equiv \left(\I^{(m-1)}, \alpha_m, \J^{(m+1)}\right),
% $$
% we obtain the following computational rule for $\u^{(m)}$,
% \begin{equation}
% \u^{(m)}(\alpha_m) = \widehat \U_{<m}^{-1} \cdot \uh\left(\I^{(m-1)}, \alpha_m, \J^{(m+1)}\right) \cdot \widehat \U_{>m}^{-1},
% \label{eq:ttcross}
% \end{equation}
% where $\widehat \U_{<m} = \U^{<m}(\I^{(m-1)})$ and $\widehat \U_{>m} = \U^{>m}(\J^{(m+1)})$ are the submatrices of $\U^{<m}$ and $\U^{>m}$ at indices $\I^{(m-1)}$ and $\J^{(m+1)}$, respectively.


% Of course, these submatrices must be nonsingular.
% In the previous subsection we saw a good strategy: if indices $\I^{(m-1)}$ and $\J^{(m+1)}$ are chosen in accordance with the maxvol principle for $\U^{<m}$ and $\U^{>m}$, the submatrices are not only nonsingular, but also 
% provide a good approximation for \eqref{eq:tt-l-b-r}.
% However, $\U^{<m}$ and $\U^{>m}$ are too large to be treated directly.
% Instead, we use the \emph{alternating} iteration over the dimensions and build nested index sets.

% The alternating iteration means that we loop over $m=1,2,\ldots,M$ (the so-called \emph{forward} iteration) and $m=M,M-1,\ldots,1$ (\emph{backward} iteration).
% Consider first the forward transition, $m-1 \rightarrow m$.
% Given the set $\I^{(m-1)}$, the \emph{nested} indices $\I^{(m)}$ are defined as follows.
% We concatenate $\I^{(m-1)}$ and $\alpha_m$, i.e. consider $r_{m-1} (p_m+1)$ indices $(\hat \alpha_{1},\ldots,\hat\alpha_{m-1},\alpha_m) \in \{\I^{(m-1)}, \alpha_m\}$, and select $r_m$ indices $\I^{(m)}$ only from $\{\I^{(m-1)}, \alpha_m\}$, not from all $\mathcal{O}(p^m)$ possibilities.
% It can be seen that the next interface $\U^{<m+1}$, restricted to $\{\I^{(m-1)}, \alpha_m\}$, can be computed as a product of the previous submatrix $\widehat \U_{<m}$ and the current TT block $\u^{(m)}$.

% To formalize this, we need the following definition.

% \begin{definition}\label{def:folded}
% Given a three-dimensional tensor $\u^{(m)} \in \mathbb{R}^{r_{m-1} \times (p_m+1) \times r_m}$, introduce the following reshapes, both pointing to the same data stored in $\u^{(m)}$:
% \begin{itemize}
%  \item \emph{left folding}: $\u^{|m\rangle}(s_{m-1},\alpha_m;~s_m) = \u^{(m)}_{s_{m-1},s_m}(\alpha_m), \quad \u^{|m\rangle} \in \mathbb{R}^{r_{m-1}(p_m+1) \times r_m},$  and
%  \item \emph{right folding}: $\u^{\langle m |}(s_{m-1};~\alpha_m,s_m) = \u^{(m)}_{s_{m-1},s_m}(\alpha_m), \quad \u^{\langle m |} \in \mathbb{R}^{r_{m-1}\times (p_m+1) r_m}.$
% \end{itemize}
% \end{definition}

% Then the restriction of $\U^{<m+1}$ writes as follows,
% $$
% \bm{V}^{\langle m|} = \widehat \U_{<m} \u^{\langle m |}, \quad \mbox{and} \quad \U^{<m+1}\left(\I^{(m-1)}, \alpha_m\right) = \bm{V}^{| m \rangle} \in \mathbb{R}^{r_{m-1}(p_m+1) \times r_m}.
% $$
% Thus, it is enough to apply the maximum volume algorithm \cite{gostz-maxvol-2010} to the matrix $\bm{V}^{| m \rangle}$, deriving \emph{local} maxvol indices $\hat i_m \subset \{1,\ldots, r_{m-1}(p_m+1)\}$, and obtain both $\I^{(m)}$ and $\widehat \U_{<m+1}$ by the restriction
% $$
% \I^{(m)} = \{\I^{(m-1)}, \alpha_m\}(\hat i_m), \quad \widehat \U_{<m+1} = \bm{V}^{| m \rangle}(\hat i_k) \in \mathbb{R}^{r_m \times r_m}.
% $$

% The backward transition $m+1 \rightarrow m$ for $\J^{(m)}$ and $\widehat \U_{>m}$ can be written analogously.
% We show it directly in Alg.\ref{alg:cross} below.
% In total, we need only $\mathcal{O}(n_{it} M p r^2)$ entries of $\uh$ to be evaluated, where $n_{it}$ is the number of alternating iterations, typically of the order of $10$.


% we have other candidates for such auxiliary data.
% And we have reasons to consider them prior to the error.
%
% %
% \subsection{Computation of the solution function}
% Having solved the system \eqref{eq:linsystem}, we obtain the PCE coefficients of the solution in the TT format,
% \begin{equation}
% \varphi() = \sum_{s_0,\ldots,s_{M-1}} \varphi^{(0)}_{s_0}(x) \varphi^{(1)}_{s_0,s_1}(\alpha_1) \cdots \varphi^{(M)}_{s_{M-1}}(\alpha_M).
% \label{eq:tt_u}
% \end{equation}
% %
% %
%



%  $Log: characteristic.tex,v $
%  Revision 1.2  2021/11/07 21:53:00  hgm
%  as obtained 7-11-2021
%
%  Revision 1.1  2019/06/10 22:05:11  hgm
%  further down the road
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 


==> chaptersV2/common_notation.tex <==
% !TEX root = ../19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: common_notation.tex,v 1.2 2021/11/07 22:27:27 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.2 $",
%%  DATE      = "$Date: 2021/11/07 22:27:27 $",
%%  FILENAME  = "$RCSfile: common_notation.tex,v $"}


\subsection{A few tests} \label{SS:fewtests}
%
All's well that ends well.  ...

Let us see that it all works.

$a\in A$ and $A\ni a$.  $a\notin B$.

\vspace{1cm}

\paragraph{Just testing}
\[  
 \ip{\vek{a}}{\vek{U}} =  \bkt{\vek{a}}{\vek{U}} = 
 \ipd{\vek{a}}{\vek{U}} =   \bkd{\vek{a}}{\vek{U}}.
\]
\[
\ip{\Ten_{j=1}^J \vek{V}_j}{\vek{W}} = 
\bkt{\sum_{j=1}^J \vek{V}_j}{\vek{W}} = 
\ipd{\Ten_{j=1}^J \vek{V}_j}{\vek{W}} = 
\bkd{\sum_{j=1}^J \vek{V}_j}{\vek{W}}.
\]
\[
  \ipj{\sum_{n=1}^N \Ten_{j=1}^{J} \tnb{A}^{(j)}_n} =
  \ns{\sum_{n=1}^N \Ten_{j=1}^{J} \tnb{A}^{(j)}_n} =
  \nd{\sum_{n=1}^N \Ten_{j=1}^{J} \tnb{A}^{(j)}_n} =
  \nt{\sum_{n=1}^N \Ten_{j=1}^{J} \tnb{A}^{(j)}_n}.
\]


\subsection{Notation} \label{SS:notation}
%
How to write different math objects.
\vspace{1cm}

\paragraph{Variables and Constants:}
In general variables should be written in a slanted or italic font, like
\[ \alpha, \gamma, \delta, \pi, \xi, \vphi, \Delta, \Phi, \Omega, a, d, e, i, x, f, D, F, \]
and constants with an upright font, like
\[ \upgamma=0.57721\dots, \updelta_i^j, \uppi = 3.14159265\dots, \upvarphi = 1.61803\dots, 
   \ee=2.71828\dots, \ii=\sqrt{-1}.
\]

\paragraph{Operators and fixed Objects:}
Also operators should be upright like differential, derivatives, etc.   
\[
  \di \omega, \; \frac{\di f}{\di x},\; \Di F, \;\int_{\C{X}} f(x)\, \di x,\quad\upDelta = \nabla^2.
\]
Also named objects like the Kronecker-$\updelta$ --- $\updelta_{i j}$ ---
 and Dirac's $\updelta$ --- $\int_{\D{R}} \updelta_{a}(x)\,f(x)\, \di x = f(a)$
in an upright font.

\paragraph{Householder Convention:}
Additionally, when dealing with linear spaces, use the \emph{Housholder}
convention --- unless usual convention demands otherwise:
\begin{description}
\item[Scalars] with small slanted Greek letters
         \[ \alpha, \beta, \gamma, \delta, \dots \]
\item[Sets of scalars] with capital slanted Greek letters
         \[ \Gamma, \Delta, \Phi, \Xi, \Omega, \dots \]
\item[Vectors] of general spaces with small (serif) italic Latin letters
         \[ a, u, v, w, x, y, z, \dots \]       
\item[Linear Operators] of general spaces with capital (serif) italic Latin letters
         \[ A, U, V, F, X, Y, Z, \dots \]
\item[Vectors with components] as elements of $\D{R}^n$ or $\D{C}^n$ with
     \tbf{bold}  small italic (serif) Latin or Greek letters, and their components with the
     corresponding non-bold letter
  \[ \vek{\alpha} = [\alpha_1,\alpha_2,\dots,\alpha_n]^\trpos,\, 
     \vek{u} = [u_1,\dots,u_n]^\trpos,\, 
     \vek{\xi} = [\xi_1,\dots,\xi_n]^\trpos,\, 
     \vek{x} = [x_1,\dots,x_n]^\trpos,\, \dots \]  
\item[Matrices] with \tbf{bold} capital italic (serif) Latin or Greek letters,
     and their components with the
     corresponding non-bold letter
  \[ \vek{A} = [A_{11},A_{12},\dots,A_{nn}],\, \vek{\Xi} = [\Xi_{11},\Xi_{12},\dots,\Xi_{nn}],\, 
     \vek{X} = [X_{11},X_{12},\dots,X_{nn}],\, \dots \]  
\end{description}
         
\paragraph{Additional Conventions:}      
\begin{description}
\item[Multi-Indices]  as elements of $\D{N}^n$ or $\D{N}_0^n$  with
     \tbf{bold}  small italic Latin letters, and their components with the
     corresponding non-bold letter
  \[ \vek{m} = (m_1,m_2,\dots,m_n],\, \vek{\ell} = [\ell_1,\ell_2,\dots,\ell_n], \dots \] 
  or ?
\item[Multi-Indices]  as elements of $\D{N}^n$ or $\D{N}_0^n$  with
     \tbf{bold} small Fraktur letters, and their components with the
     corresponding non-bold Latin letter
  \[ \F{m} = (m_1,m_2,\dots,m_n],\, \F{k} = [k_1,k_2,\dots,k_n], \dots \] 
\item[Linear Spaces] and their subsets with capital calligraphic Latin letters
         \[ \C{A}, \C{U}, \C{V}, \C{F}, \C{X}, \C{Y}, \C{Z}, \dots \]       
\item[Spaces of Linear Operators] with capital script Latin letters
         \[ \E{L}(\C{U}),\; \E{L}(\C{X},\C{Y}), \dots \]
\item[Sets of Sets] like topologies and $\sigma$-algebras with capital Fraktur letters
        \[ \F{G}, \; \F{T}, \; \F{A}, \dots \]
\item[Tensors] as elements of e.g.\ $\D{R}^{n_1\times n_2 \times \dots \times n_d}$
   with slanted sans-serif \tbf{bold} letters, and their components with the
   corresponding slanted sans-serif non-bold letters
   \[ \tnb{w}=(\tns{w}_{i_1,\dots,i_d}),\;  \tnb{M}= (\tns{M}_{a b c d}),\;
    \tnb{y}=(\tns{y}_{{i_1}{k_1}i_2 k_2}),\; \tnb{\beta}=(\tns{\beta}_{i_1,\dots,i_\ell}),\;
    \tnb{\Theta}=(\tns{\Theta}_{\ell_1,\dots,\ell_d})
     \dots \]
       or in Penrose's \emph{symbolic} index notation
      with slanted sans-serif or serif non-bold letters
   \[ \tensor{\tns{M}}{^a_b^{cd}_e},\; \tensor[^a_b^c_d]{\tns{A}}{^a_b^c_d},\;
   \tensor{R}{_i^j_k},\; \tensor{\Gamma}{^i_j_k},\; 
   \tensor{\tns{\Omega}}{^i_\ell^k_m_n},   \dots \]
\end{description}


\subsection*{Tensor package} \label{SS:tensors}
%
\[ M\indices{^a_b^{cd}_e} = \tensor{M}{^a_b^{cd}_e}\]
\begin{verbatim}
M\indices{^a_b^{cd}_e} = \tensor{M}{^a_b^{cd}_e}
\end{verbatim}

\[ \tensor[^a_b^c_d]{M}{^a_b^c_d} \neq \tensor*[^a_b^c_d]{M}{^a_b^c_d} \]
\begin{verbatim}
 \tensor[^a_b^c_d]{M}{^a_b^c_d} \neq \tensor*[^a_b^c_d]{M}{^a_b^c_d}
\end{verbatim}

\[ \tensor*{M}{*^{i_1}_{m_1}^{i_2}_{m_2}^{i_3}_{m_3}^{i_4}_{m_4}} =
   M\indices*{*^{i_1}_{m_1}^{i_2}_{m_2}^{i_3}_{m_3}^{i_4}_{m_4}} \]
\begin{verbatim}
\tensor*{M}{*^{i_1}_{m_1}^{i_2}_{m_2}^{i_3}_{m_3}^{i_4}_{m_4}}=
  M\indices*{*^{i_1}_{m_1}^{i_2}_{m_2}^{i_3}_{m_3}^{i_4}_{m_4}}
\end{verbatim}

\renewcommand\indexmarker{\cdot}
\[ \tensor{M}{^a_b^c_d} \]
\begin{verbatim}
\renewcommand\indexmarker{\cdot}   \tensor{M}{^a_b^c_d}
\end{verbatim}

\[ \nuclide[14][6]{C} \quad \text{and} \quad \nuclide[4][2]{\upalpha} \]
\begin{verbatim}
\nuclide[14][6]{C} \quad \text{and} \quad \nuclide[4][2]{\upalpha} 
\end{verbatim}


\subsection*{Test of math fonts} \label{SS:testf}
%
\paragraph{Slanted:} --- serifs
\[ a, \alpha, A, \Phi, \phi, \vphi, \qquad 
     \vek{a}, \vek{\alpha}, \vek{A}, \vek{\Phi}, \vek{\phi}, \vek{\vphi} \]

\paragraph{Slanted:} --- sans serif
\[ \tns{a}, \tns{\alpha}, \tns{A}, \tns{\Phi}, \tns{\phi}, \tns{\vphi}, \qquad
  \tnb{a}, \tnb{\alpha}, \tnb{A}, \tnb{\Phi}, \tnb{\phi}, \tnb{\vphi} \]
   
\paragraph{Other:}  --- no small letters
\[ \C{E}, \C{Q}, \C{R}; \D{E}, \D{Q}, \D{R}; \E{E}, \E{Q}, \E{R}\]

\paragraph{Fraktur:}
\[ \F{e}, \F{q}, \F{r}; \F{E}, \F{Q}, \F{R} \]

\paragraph{Upright:} --- serifs and sans-serif, no small greek letters
\[ \mrm{a}, \mrm{A}, \mrm{\Phi},\qquad \mat{a}, \mat{A}, \mat{\Phi}, \qquad 
 \ops{a}, \ops{A}, \ops{\Phi},\qquad \opb{a}, \opb{A}, \opb{\Phi} \]

\paragraph{Small Greek upright}
\[ \upalpha, \uppi, \upgamma, \upphi, \upvarphi, \uppsi, \upxi, \upeta, \upzeta \]



%  $Log: common_notation.tex,v $
%  Revision 1.2  2021/11/07 22:27:27  hgm
%  added header and footer
%
%  Revision 1.12  2021/11/07 22:19:10  hgm
%  added header and footer
%
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 




==> chaptersV2/distances.tex <==
% !TEX root = ../19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: distances.tex,v 1.2 2021/11/07 22:27:43 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.2 $",
%%  DATE      = "$Date: 2021/11/07 22:27:43 $",
%%  FILENAME  = "$RCSfile: distances.tex,v $"}


\section{Distances}
\begin{example}
The \textbf{Wasserstein} (or Kantorovich distance) --- which arises from the idea of optimal 
transport --- is being used more and more in Statistics and Machine Learning 
\cite{Kolouri17}. 
Let $\C{J}(P,Q)$ denote all joint distributions $J$ for $(X,Y)$ 
that have marginals $P$ and $Q$. Then the Wasserstein 
distance is defined as
\begin{equation}
    W_p(P,Q)=\left( \inf_{J\in\mathcal{J}(P,Q)} \int \Vert x-y\Vert^p  J(\di x,\di y)\right)^{1/p}
\end{equation}
\end{example}
%Kolouri,  Soheil,  et  al.   Optimal  Mass  Transport:  Signal  processing  and  
%machine-learningapplications.IEEE Signal Processing Magazine 34.4 (2017):  43-59.
%Villani,  %Cedric.Topics  in  optimal  transportation.  No.  58.  American Mathematical Soc.,2003.

%\subsubsection{Hellinger distance}
\begin{example}
Let $P$ and $Q$ denote two probability measures that are absolutely continuous 
with respect to a third probability measure $\lambda$. 
The square of the 
\textbf{Hellinger distance} between $P$ and $Q$ is defined as the quantity
\begin{equation}
{\displaystyle H^{2}(P,Q)={\frac {1}{2}}\displaystyle \int 
\left({\sqrt {\frac {\di P}{\di\lambda }}}-{\sqrt {\frac {\di Q}{\di\lambda }}}
  \right)^{2}\di\lambda .}
\end{equation}
Here, $\frac{\di P}{\di\lambda}$ and $\frac{\di Q}{\di\lambda}$ are the Radon–Nikod\'ym 
derivatives of $P$ and $Q$ respectively. This definition does not depend on $\lambda$, 
so the Hellinger distance between $P$ and $Q$ does not change if $\lambda$ is replaced 
with a different probability measure with respect to which both $P$ and $Q$ are 
absolutely continuous. For compactness, the above formula is often written as
\begin{equation}
 {\displaystyle H^{2}(P,Q)={\frac {1}{2}}\int \left({\sqrt {\di P}}-
 {\sqrt {\di Q}}\right)^{2}.} 
\end{equation}
\end{example}



%  $Log: distances.tex,v $
%  Revision 1.2  2021/11/07 22:27:43  hgm
%  added header and footer
%
%  Revision 1.12  2021/11/07 22:19:10  hgm
%  added header and footer
%
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 




==> chaptersV2/extra_tensors.tex <==
% !TEX root = ../19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: extra_tensors.tex,v 1.3 2021/11/07 22:32:10 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.3 $",
%%  DATE      = "$Date: 2021/11/07 22:32:10 $",
%%  FILENAME  = "$RCSfile: extra_tensors.tex,v $"}


\subsection{CP and Tucker tensor formats}
 \label{sec:low-rank}
Canonical and Tucker tensor formats were introduced in
chemometrics and signal processing,
where they were applied for quantitative analysis of correlation in
multi-dimentional experimental data \citep{Hitch:27, Tuck:66, Cichocki:2002}. 
The Tucker algorithm is based on the higher order singular value 
decomposition (HOSVD) and the Tucker ALS algorithms \cite{DMV-SIAM2:00}. 
For dimension, $d=3$, the Tucker and CP
tensor formats are a good choice.
For higher dimensions there are other tensor formats, for example, the, 
so-called, Matrix Product States \cite{Scholl:11} and Tensor Train \citep{OseledetsTT11} format.

The fast convergence of the Tucker decomposition
for some discretized differential operators and Green's functions 
was shown in \cite{khor-rstruct-2006,KhKh:06}.
\begin{definition}
The product index set is $\C{I}:=I_1\times...\times I_d$, 
 $I_{\mu}=\{i_1,...,i_{n_{\mu}}\}$, $\# I_{\mu}=n_{\mu}$.\\
One can see tensors as vectors $(\C{A})_{j\in \C{I}} \in \D{R}^{\C{I}}$ with 
$\prod_{\mu=1}^d n_{\mu}$ entries.
\end{definition}


\begin{defi}
A tensor of order $d$ in a full format is defined as a multidimensional array
over a $d$-tuple index set,
 \begin{equation}
 \label{Tensor_def}
{\bf A}=[a_{i_1,\ldots,i_d}]\equiv [a(i_1,\ldots,i_d)] \; \in 
\mathbb{R}^{n_1 \times \ldots \times n_d}\;
\mbox{  with } \quad i_\nu\in I_\nu:=\{1,\ldots,n_{\nu}\}.
\end{equation}
Here 
$\bf A$ is an element of the linear space
%\begin{equation*}
$ \mathbb{V}_n=\bigotimes_{\nu=1}^d \mathbb{V}_{\nu},\quad \mathbb{V}_{\nu}=\mathbb{R}^{I_\nu}$,
%\end{equation*}
equipped with the Euclidean scalar product $\langle \cdot,\cdot \rangle:
\mathbb{V}_{n}\times \mathbb{V}_{n}\rightarrow \mathbb{R}$, defined as
\begin{equation*}
 \langle {\bf A},{\bf B} \rangle:=\sum_{(i_1...i_d)\in \mathcal{I}}a_{i_1...i_d}b_{i_1...i_d},
 \quad \text{for}\quad \bA,\,\bB\,\in \mathbb{V}_n.
\end{equation*}
\end{defi}
Tensors with all dimensions having equal size $n_{\nu} =n$, $\nu=1,\ldots d$,
will be called an $n^{\otimes d}$ tensor. The  required storage size 
scales exponentially in the dimension, $n^d$, which results in the 
so-called ''curse of dimensionality``. 

To reduce the exponential cost, one can apply  the 
rank-structured separable representations or approximations of multidimensional tensors.


\begin{definition}
The \textit{tensor product of vectors} $\bw^{(\nu)} \in \mathbb{R}^{n_{\nu}}$ is defined by
\begin{equation}
 \left(\bigotimes_{\nu=1}^d \bw^{(\nu)}\right)[i_1,i_2,...,i_d]:=\prod_{\nu=1}^d \bw^{(\nu)}[i_{\nu}].
\end{equation}
\end{definition}
%
\begin{definition}
The \textit{tensor product of univariate functions} $f_{\nu}$ is defined by 
\begin{equation}
 \left(\bigotimes_{\nu=1}^d f_{\nu}\right)(\xi_2,\xi_2,...,\xi_d):=
 \prod_{\nu=1}^d f_{\nu}(\xi_{\nu}).
\end{equation}
\end{definition}
%
%
\begin{defi}
A tensor in the $R$-term canonical format is defined by a finite sum of rank-$1$ tensors,
 \begin{equation}\label{eqn:CP_form}
  {\bf A} = {\sum}_{k =1}^{R} c_k
  {\bf u}_k^{(1)}  \otimes \ldots \otimes {\bf u}_k^{(d)},  \quad  c_k \in \mathbb{R},
\end{equation}
where ${\bf u}_k^{(\ell)}\in \mathbb{R}^{n_\ell}$ are normalized vectors, 
and $R$ is called the canonical rank of a tensor. 
\end{defi}
%
%
The storage cost of this
parametrization is bounded by  $d R n$.
An element  $\bA(i_1,...,i_d)$ of tensor ${\bf A}=\sum_{i=1}^R\bigotimes_{\nu=1}^d u_{i \nu}$ 
can be computed as follows
\begin{equation*}
 \bA(i_1,...,i_d)= \sum_{\alpha=1}^R u_1(i_1,\alpha)u_2(i_2,\alpha)...u_d(i_d,\alpha).
\end{equation*}

An alternative (contracted product) notation used in computer science community,
\begin{equation}
 \label{Can_Contr}
 {\bf A} = {\bf C} \times_1 U^{(1)} \times_2 U^{(2)} \times_3 \cdots \times_d U^{(d)},
 \end{equation}
where ${\bf C}=diag\{c_1,...,c_d\} \in\mathbb{R}^{R^{\otimes d}}$, and
$ U^{(\ell)}=[{\bf u}_1^{(\ell)}\ldots {\bf u}_R^{(\ell)} ]\in\mathbb{R}^{n_\ell \times R}$.
 Again, there is an analogue with a multivariate function which can be represented by a sum
of a number of separable multivariate functions (say, by a sum of Gaussians),
\[
 f(x_1,x_2,\ldots , x_d) = \sum\limits^R_{k=1} f_{1,k}(x_1) f_{2,k}(x_2)\ldots f_{d,k}(x_2).
\]
For $d\geq 3$, there are no stable algorithms for computation of the 
canonical rank of a tensor ${\bf U}$, that is
the minimal number $R$ in representation (\ref{eqn:CP_form}), and the respective
decomposition with the polynomial cost in $d$, i.e., the computation of the
canonical decomposition is an $N$-$P$ hard problem. (reference?)
\begin{figure}[htb]
\centering
\includegraphics[width=5cm]{figs/Canon.eps}\quad\quad\quad
\includegraphics[width=5cm]{figs/Tucker_AB.eps}
\caption{\small Canonical (left) and Tucker (right) decompositions of 3D tensors. We thank Venera Khoromskaja for these pictures.}
\label{fig:CP_Tucker}
\end{figure}
 

The Tucker tensor format is suitable for stable numerical decompositions with the fixed
truncation threshold.
We say that a tensor ${\bf A} $ is represented in the rank-$\bf r$ orthogonal Tucker format 
with the rank parameter ${\bf r}=(r_1,\ldots,r_d)$, if 
\begin{equation*}
 \bA(i_1,...,i_d)= \sum_{\alpha_1=1}^{r_1}\sum_{\alpha_2=1}^{r_2}...\sum_{\alpha_d=1}^{r_d} G_{\alpha_1, \ldots ,\alpha_d}u_1(i_1,\alpha_1)u_2(i_2,\alpha_2)...u_d(i_d,\alpha_d).
\end{equation*}
or, after discretisation of functions $u_1$, $u_2$,$\ldots$,$u_d$
\begin{equation}\label{eqn:Tucker_form}
  {\bf A}  =\sum\limits_{\nu_1 =1}^{r_1}\ldots
\sum\limits^{r_d}_{{\nu_d}=1} G_{\nu_1, \ldots ,\nu_d}
\,  {\bf v}^{(1)}_{\nu_1} \otimes \ldots \otimes {\bf v}^{(d)}_{\nu_d},\quad \ell=1,\ldots,d, 
\end{equation}
where $\{{\bf v}^{(\ell)}_{\nu_\ell}\}_{\nu_\ell=1}^{r_\ell}\in \mathbb{R}^{n_\ell}$,  
represents a set of orthonormal vectors for $\ell=1,\ldots,d$, 
and $\boldsymbol{G}=[G_{\nu_1,\ldots,\nu_d}] \in \mathbb{R}^{r_1\times \cdots \times r_d}$ is 
the Tucker core tensor. 
The storage cost for the Tucker tensor is bounded by $d r n +r^d$, 
with $r=|{\bf r}|:=\max_\ell r_\ell$. The term $r^d$ increases exponentially with $d$ and, therefore, is a luck of Tucker format.
Using orthogonal side matrices $V^{(\ell)}=[v^{(\ell)}_1 \ldots v^{(\ell)}_{r_\ell}]$ 
and contracted products, the Tucker tensor decomposition may be presented in an alternative notation,
\[
  { {\bf A}_{({\bf r})}=\boldsymbol{\beta} \times_1 V^{(1)}\times_2 V^{(2)} \times_3 \ldots 
  \times_d V^{(d)}.} 
\]  
In the case $d=2$, the orthogonal Tucker decomposition is equivalent to the singular 
value decomposition (SVD) of a rectangular matrix. To avoid luck of CP and Tucker tensor formats, an alternative format was developed, namely tensor train.

\subsection{Tucker decomposition of full format tensors}
\label{ssec:Tucker_decomp}
 
The algorithm for computing the Tucker decomposition of the full format tensor is
the following. First, and most time consuming part of the Tucker algorithm is computation of 
the initial guess for matrices $V^{(\ell)}$  by using
the SVD of the matrix unfolding $A_{(\ell)}$, $\ell=1,\; 2, \; 3 $, of the original tensor 
along every mode of a  tensor. 
It is called higher order singular value decomposition (HOSVD) \cite{DMV-SIAM2:00}. 
Figure \ref{fig:Unfolding} illustrates the matrix unfolding of the full format 
tensor A (\ref{Tensor_def}) along the index set $I_1=\{1,\ldots,n_1\}$. 
\begin{figure}[htb]
\centering
\includegraphics[width=10.0cm]{figs/Unfolding.eps} 
%\includegraphics[width=7.0cm]{figs/Tucker_AB.eps}
\caption{\small Unfolding of a 3D tensor along the mode $I_\ell$ with $\ell=1$.}
\label{fig:Unfolding}
\end{figure}
 
The second part of the algorithm
is the ALS procedure. For every tensor mode the so-called ''single hole`` tensor of reduced size
is constructed, by the mapping of the all modes 
of the original tensor except one into subspaces $V^{(\ell)}$. 
Then the subspace $V^{(\ell)}$ for the current mode is updated by the SVD
of the unfolding of the ''single hole`` tensor for this mode.
This alternates over all modes of the tensor, which are to be updated
at the current step of ALS. The final step is computation of the core tensor by using the
ultimate mapping matrices from the ALS.
    
 The numerical cost of the Tucker decomposition for full size tensors is dominating by
 the initial guess, which (if all $n_\ell=n$ are equal) is estimated as
 $O(n^{d+1})$, or in our case for 3D, $O(n^{4})$. This step is (a) the most computationally 
 consuming, and (b) it restricts the  available size of the tensor to be decomposed since 
 for conventional computers  for 3D case $n_\ell> 10^2$ is the limiting case for SVD.
 
  In \citep{khor-ml-2009} the Multigrid Tucker algorithm for full size tensors
was introduced which allows to reach  the computational complexity which is 
linear in the full size of the tensor, $O(n^d)$, that is $O(n^3)$ for 3D tensors. This allows to decompose 
maximum size of the input full format tensors available in computer storage.
The basic idea is to eliminate the initial guess step for tensors on large 3D grids.
The multigrid  Tucker decomposition is performed on a sequence of diadically refined grids.
It is based on implementing the HOSVD only at the coarsest grid level $n_0 \ll n$.
 The initial guess for the ALS procedure at every refined 
level is computed by the interpolation of the dominating Tucker subspaces 
obtained at the previous coarser grid. In this way, at fine 3D Cartesian grids we need 
only  $O(n^3)$ storage (to represent the initial full format tensor) 
to contract with the Tucker side matrices, obtained by 
the Tucker approximation via ALS on the previous grids.

\textcolor{red}{Can write in a simpler way},

\subsection{Actual computation }
%
%


\subsection{$d$-dimensional mesh}
%
In this section it will be explained how to compute $\varphi_{\vX}(\bt)$ 
numerically on a $d$-dimensional grid $\mT$
For instance, the element of $\mT$ 

To be able to write an expression for evaluation of the $d$-dimensional 
characteristic function on a grid $\mT$, let us introduce the following notation 
$\tau_{\beta}=(t_{\beta_1,1},t_{\beta_2,2},...,t_{\beta_d,d})\in 
\D{R}^{n_1 \times ... \times n_d}$.  Here $\tau_{\beta}$ is a node in $\mT$ coordinates 
of which are 
described by a vector $(\beta_1,...,\beta_d)$. Our aim is to evaluate the 
characteristic function in all nodes of $\mT$ an an efficient way.

After evaluation of the characteristic function 
$\vphi_{\vX}$ at the nodal point $\tau_{\beta} \in \mT$, obtain:
\begin{equation} 
\Phi_{\vX}(\tau_{\beta}):=\left[ \vphi_{\vX}(\tau_{\beta}) \right]=
\left[\varphi_{\vX}\left( t_{\beta_1,1},t_{\beta_2,2},...,t_{\beta_d,d} \right)^\trpos \right]=
\D{E}(\exp(\ii \langle \vX, \tau_{\beta}\rangle)).
\end{equation} 
%the characteristic function $\varphi_{\vX}$ evaluated at grid nodes of $\mT$.
%
Recall definition of the characteristic function:
\begin{equation}  \label{eq:T2}
%\varphi_{\vX}(\tau_{\beta})=
\D{E}\left( \exp(\ii \ip{\vX(\theta_1,...,\theta_m)}{\tau_{\beta}})\right)
 =\idotsint_{\Theta}\exp(\ii \ip{\vX(\theta_1,...,\theta_m)}{\tau_{\beta}})
 \prod_{m=1}^M p_{\theta_m}(\theta_m)\di\theta_1...\di\theta_M,
\end{equation}  
where $\thetab=(\theta_1,...,\theta_m)\in \Theta$.\\
%The scalar product is $\ip{\vX(\omega)}{\tau^{\beta}}=\sum_{\ell=1}^d 
% X_{\ell}(\thetab)t^{\beta}_{\ell}$.
%

\begin{remark}
The computational cost of $\ip{\vX(\omega)}{\tau_{\beta}}$ at 
$n_1\times...\times n_d$ points is $\C{O}(\vert \C{J} \vert (d+M\cdot C)
\sum_{\ell=1}^d n_{\ell})$,
\end{remark}
where $C$ is the highest cost to compute $\psi_{\alpha_m}(\theta_m)$. 

\begin{remark}
The computational cost of Eq.~\ref{eq:scp0} at 
$n_1\times...\times n_d$ points is $\C{O}(\vert \C{J} \vert (d+M\cdot C)
\sum_{\ell=1}^d n_{\ell})$,
\end{remark}
where $C$ is the highest cost to compute $\psi_{\alpha_m}(\theta_m)$. 



%  $Log: extra_tensors.tex,v $
%  Revision 1.3  2021/11/07 22:32:10  hgm
%  added header and footer
%
%  Revision 1.12  2021/11/07 22:19:10  hgm
%  added header and footer
%
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 




==> chaptersV2/notation_table.tex <==
% !TEX root = ../19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: notation_table.tex,v 2.1 2022/05/17 09:21:14 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 2.1 $",
%%  DATE      = "$Date: 2022/05/17 09:21:14 $",
%%  FILENAME  = "$RCSfile: notation_table.tex,v $"}


\begin{table}[h]
\caption{Notation}
\begin{tabular}{|c|l|}
\hline 
%\multicolumn{2}{|c|}{\textbf{General quantities}} \\ \hline
%${\Nset}$        &Natural numbers \\ \hline
%$(\Omega,\F{A},\D{P})$ & Probability space $\Omega$, $\sigma$-algebra $\F{A}$, and prob.\
% measure $\D{P}$ \\ \hline
$\vX$ & Random vector  $\vX=(\xi_1,...,\xi_d):\Omega\to\D{R}^d$ \\ \hline
$ \by$ & Parameter vector $ \by=(y_1,...,y_d)\in\D{R}^d$\\ \hline
\pdf & probability density function, denoted by $p_{\vX}(\by): \Rd\to\D{R}$ \\ \hline 
\pcf & probability characteristic function, denoted by $\vphi_{\vX}(\bt)$   \\ \hline 
$\bt$ & $\bt=(t_1,t_2,...,t_d) \in \D{R}^d$, the dual variable to $\by\in\Rd$ \\ \hline
\cdf & cumulative distribution function  \\ \hline RV & Random variable \\ \hline
KLD, $\widetilde{D}_{\text{KL}}$ & Kullback-Leibler divergence \\ \hline
$\EXP{\cdot}$ & expectation operator \\  \hline
$\bkt{\bt}{\by}$ & canonical Euclidean inner product on $\D{R}^d$,
   $\bkt{\bt}{\by}=\sum_{k=1}^d t_k y_k$ \\ \hline
%$\bx$ & vector $\bx=(x_1,...,x_d)$ \\ \hline
%$\bt$ & vector $\bt=(t_1,...,t_d)$ \\ \hline
$\tnb{P}$, $\tnb{Q}$ & tensors obtained after discretisation of two \pdfs \\ \hline 
% $\bar{\vX} = \EXP{\vX}\in\D{R}^d$ & mean value of random vector $\vX$  \\ \hline
% %$\tilde{\vX} = \vX - \bar{\vX}$ & mean zero part of random vector  $\vX$ \\ \hline
% $\F{B}$ & Borel $\sigma$-algebra of $\D{R}^d$ \\ \hline
% $\C{E}_{\by}\in\F{B}$ & semi-infinite interval in $\D{R}^d$, $\C{E}_{\by} = \bigtimes_{k=1}^d\;
%     ] \!-\!\infty, y_k ]$ \\ \hline
% $\mbf{1}_{\C{E}}(\by)$,  $\C{E}\in\F{B}$ & char./indicator function,  if $\by\in\C{E}$:
%   $\mbf{1}_{\C{E}}(\by) = 1$, else $\mbf{1}_{\C{E}}(\by) = 0$ \\ \hline
% $P_{\vX}(\C{E}) = \EXP{\mbf{1}_{\C{E}}(\vX)}$ & distribution (measure) of $\vX$
%      for $\C{E}\in\F{B}$, push forward $P_{\vX} = \vX_* \D{P}$ \\ \hline
% $F_{\vX}(\by) = P_{\vX}(\C{E}_{\by})$ & distribution fct.\ of $\vX$,
%      cumulative prob., $F_{\vX}(\by) = \D{P}(\vX \le \by)$ \\ \hline
% $p_{\vX}(\by)= \Di_{\by}F_{\vX}(\by)$ &  %($\Di_{\by}=\prod_{k=1}^d \dd_{y_k}$)
%   probability density fct.\ (\pdf) of $\vX$, and approximation $\tilde{p}_{\vX}(\by)$ \\ \hline
% $\vphi_{\vX}(\bt)=\EXP{\exp(\ii \ip{\bt}{\vX})}$   
%  & The characteristic fct.\ (\cdf)  of $\vX$, and approximation $\tilde{\vphi}_{\vX}(\bt)$\\ \hline
% $\chi_{\vX}(\bt)=\log(\vphi_{\vX}(\bt))$ & The 2nd characteristic or cumulant generating
%     fct.\ of $\vX$\\ \hline
% $\C{D}\subset\D{R}^d$ & Computational domain \\ \hline
% $I$, $I_N$ & Identity operator, identity matrix of size $N\times N$ \\ \hline
% %{KL}           & {Karhunen-Lo\`eve (Expansion)}\\ \hline
%(g)PCE            & (generalized) Polynomial Chaos Expansion \\ \hline
(i)(F)FT& (inverse) (Fast) Fourier transformation \\ \hline
$\iFd$, $\Fd$  & $d$-dimensional (inverse) Fourier transformation \\ \hline
%${\var}$           & Variance\\ \hline
%$H_{\alpha}$ & Multivariate Hermite polynomial with multi-index 
%  $\vek{\alpha}:=(\alpha_1,\ldots,\alpha_M)\in\D{N}_0^M$ & finite multi-index \\ \hline
%$h_{\alpha_m}(\theta_m)$ & univariate polynomial of variable $\theta_m$ \\ \hline
%$\alpha$, $\beta$, $\nu$ & multi-indices in gPCE\\ \hline
%$\J = \D{N}_0^{(\D{N})}$ & multi-index set \\ \hline
%$\vek{\alpha}$, $\vek{\beta}$, $\vek{\nu}\in\J$ & multi-indices 
%   $\vek{\beta}:=(\beta_1,\ldots,\beta_{M},...)$\\ \hline
%$\J_{M,p}\subset\D{N}_0^M\subset\J$ & $M$ components, max.\ polynomial order $p$\\ \hline
%$L$ & Number of the KLE terms after truncation \\ \hline
%$M$ & Stochastic dimension \\ \hline
%$d$ & dimension of $\vX$ \\ \hline
% $\param$ & high-dimensional parameter \\ \hline
%$p$ & polynomial order or vector of them, $\vek{p}=(p_1,\ldots,p_M)$ \\ \hline 
%\multicolumn{2}{|c|}{\textbf{Multidimensional and/or tensor product quantities}} \\ \hline
%{TT}           & Tensor train data format \\ \hline
$\otimes$  & Tensor (Kronecker) product \\ \hline
QoI & Quantity of Interest \\ \hline
%$\times$  & Cartesian product \\ \hline
%$u(\theta_1,\ldots,\theta_M)$ & $M$-variate function \\ \hline
%$ \bTheta_{\vek{\gamma}}= \bigtimes_{\ell=1}^M \theta_{\gamma_{\ell}}$ & $M$-dimensional grid 
% $\vek{\gamma}=(\gamma_1,...,\gamma_M),\,\, \theta_{\gamma_{\ell}}=(1,...,n_{\gamma_{\ell}})$ 
% \\ \hline
%$\mT$ & $d$-dim. grid, $=\bigotimes_{\ell=1}^d \tau_{\ell}\in \mathbb{R}^{n_1\times n_2 ... 
%  \times n_d},\,\quad \tau_{\ell}\in \mathbb{R}^{n_{\ell}}$ 
%\\ \hline
\end{tabular}
\label{tab:notations}
\end{table}%
%




%  $Log: notation_table.tex,v $
%  Revision 2.1  2022/05/17 09:21:14  hgm
%  in rev 2
%
%  Revision 1.2  2021/11/07 22:34:04  hgm
%  added header and footer
%
%  Revision 1.12  2021/11/07 22:19:10  hgm
%  added header and footer
%
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 



==> chaptersV2/other_tensor_formats.tex <==
% !TEX root = 19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: other_tensor_formats.tex,v 1.3 2021/11/07 22:37:56 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.3 $",
%%  DATE      = "$Date: 2021/11/07 22:37:56 $",
%%  FILENAME  = "$RCSfile: other_tensor_formats.tex,v $"}



\subsection{The Tucker tensor format}
\label{ssec:Tucker}
%
The Tucker tensor format was introduced in \citep{Tuck:66}.
\begin{figure}[htb]
\centering
\includegraphics[width=0.55\textwidth]{figs/Tucker1.png}
\caption{Schema of the Tucker decomposition of a 3D tensor.}
\label{fig:Tucker}
\end{figure}
A schema for the Tucker tensor format for $d=3$ is shown in 
Figure~\ref{fig:Tucker}.  The full tensor 
$\tnb{w}\in \D{R}^{n_1\times n_2\times n_3}$ is shown on the left side of the equality 
sign, and its decomposition on the right.  The small cube on the right side in the 
Tucker format denotes a core-tensor $\That{w}$ of size 
$r_1\times r_2 \times r_3$, and the rectangles denote matrices of column vectors
$\vek{U}_1:=[\vek{w}_{1}^{(1)},\dots,\vek{w}_{r_1}^{(1)}]\in \D{R}^{n_1\times r_1}$,
$\vek{U}_2:=[\vek{w}_{1}^{(2)},\dots,\vek{w}_{r_2}^{(2)}]\in \D{R}^{n_2\times r_2}$,
$\vek{U}_3:=[\vek{w}_{1}^{(3)},\dots,\vek{w}_{r_3}^{(3)}]\in \D{R}^{n_3\times r_3}$,
In this way one has
\[ 
\tnb{w} =  \That{w} \times_1 \vek{U}_1^\trpos \times_2 \vek{U}_2^\trpos \times_3 \vek{U}_3^\trpos,
\]
where the symbol $\times_k$ denotes the contraction of the $k$-th tensor index 
of $\That{w}$ with the first index of the matrix $\vek{U}_k^\trpos$ in Figure~\ref{fig:Tucker}.


\begin{definition}[Tucker Tensor Format]\label{D:TuckerFormat}
The Tucker tensor format in $\C{T}$ with rank parameter $\vek{r}=(r_1,\dots,r_d)$ is
defined by the multilinear mapping
\begin{align} \nonumber
\tns{U}_{\Tuck,\vek{r}} : \C{P}_{\Tuck,\vek{r}}&:=\bigtimes_{\nu=1}^d \C{P}^{r_\nu}_\nu 
  \times \C{P}_c  \rightarrow \C{T}, \quad \C{P}_\nu = \D{R}^{M_\nu}\; (\nu=1,\dots,d), 
  \quad \C{P}_c = \D{R}^{r_1} \otimes \dots \otimes \D{R}^{r_d},\\ \label{eq:TuckerFormat}
   \C{P}_{\Tuck,\vek{r}}\ni \tnb{P} &:= \left(\vek{w}^{(i)}_{\nu_i}, \That{w}=
    (\Shat{w}_{\nu_1, \ldots ,\nu_d})\in\C{P}_c: 1\le \nu_i \le r_i, 1\le i\le d\right) \\
    &\qquad \mapsto \quad\tns{U}_{\Tuck,\vek{r}}(\tnb{P}) := \tnb{w}=
    \sum_{\vek{\nu}}^{\vek{r}} \Shat{w}_{\nu_1, \ldots ,\nu_d}\bigotimes_{i=1}^d
     \,  {\vek{w}}^{(i)}_{\nu_i}\; \in\C{T},
    \nonumber
\end{align}
where $\{{\vek{w}}^{(i)}_{\nu_i}\}_{\nu_i=1}^{r_i}\subset \D{R}^{M_i}$ 
represents a set of orthonormal vectors for $i=1,\dots,d$ and $\That{w}=
 (\Shat{w}_{\nu_1, \ldots ,\nu_d} ) = (\Shat{w}_{\vek{\nu}})\in\C{P}_c$ 
is the so-called Tucker core tensor.  We call the sum of elementary tensors 
$\tnb{w}=\tns{U}_{\Tuck,\vek{r}}(\tnb{P})$ a tensor represented in the Tucker tensor format with
$\prod_{i=1}^d r_i$ terms. 
%The system of vectors $\left(\tns{p}_{i \nu} : 1\leq i \leq r,
%\mbox{ } 1\leq \nu \leq d\right)$ is a \emph{representation system}
%of $\tnb{v}$ with \emph{representation rank} $r$.
\end{definition}
Originally, it was applied for tensor decompositions of
multidimensional arrays in chemometrics.
The Tucker tensor format provides a
stable algorithm for decomposition of full-size tensors. 
The higher order singular value decomposition (HOSVD) and the Tucker
ALS algorithm for orthogonal Tucker approximation of higher 
order tensors were introduced in \citep{DMV-SIAM2:00}. 
%We say that the tensor $\tnb{w} $ is represented in the rank-$\vek{ r}$ orthogonal Tucker format 
%with the rank parameter ${\vek{ r}}=(r_1,\ldots,r_d)$ if 
%\begin{equation}\label{eqn:Tucker_form}
%  {\tnb{w}}  =\sum\limits_{\nu_1 =1}^{r_1}\ldots
%\sum\limits^{r_d}_{{\nu_d}=1} \Shat{w}_{\nu_1, \ldots ,\nu_d}
%\,  {\tns{ w}}^{(1)}_{\nu_1} \otimes \ldots \otimes {\tns{ w}}^{(\ell)}_{\nu_{\ell}} 
%\ldots \otimes {\tns{ w}}^{(d)}_{\nu_d},\quad \ell=1,\ldots,d, 
%\end{equation}
%where $\{{\tns{ w}}^{(\ell)}_{\nu_\ell}\}_{\nu_\ell=1}^{r_\ell}\in \D{R}^{n_\ell}$ 
%represents a set of orthonormal vectors for $\ell=1,\ldots,d$, 
%and 
%%$\bB=[\bB_{\nu_1,\ldots,\nu_d}] \in \D{R}^{r_1\times \cdots \times r_d}$ 
%$\That{w}=(\Shat{w}_{\nu_1, \ldots ,\nu_d})\in \D{R}^{r_1\times \cdots \times r_d}$
%is 
%the Tucker core tensor. 
The storage cost for the Tucker tensor is bounded by 
$\C{O}(d\,r\,n +r^d)$, with $r:=\max_\ell r_\ell$.
% Using the orthogonal side matrices $V^{(\ell)}=[v^{(\ell)}_1 \ldots v^{(\ell)}_{r_\ell}]$ 
% and contracted products, the Tucker tensor decomposition may be presented in the alternative notation,
% \[
%   { {\bf A}_{({\bf r})}=\bB \times_1 V^{(1)}\times_2 V^{(2)} \times_3 \ldots 
%   \times_d V^{(d)}.} 
% \]  
% In the case $d=2$, the orthogonal Tucker decomposition is equivalent to the singular 
% value decomposition (SVD) of a rectangular matrix. 
% %
%
\subsubsection{Basic operations with the Tucker format}
Let us assume $\tnb{w}=\tns{U}_{\Tuck,\vek{r}}(\tnb{P})$
in Tucker format as in \refeq{eq:TuckerFormat}. 

\paragraph{Multiplication by a scalar} $\alpha$
can simply be done by multiplying the core tensor $\That{w}$:
\begin{equation*}
\alpha\cdot {\tnb{w}}  = \sum_{\vek{\nu}}^{\vek{r}} (\alpha\Shat{w}_{\nu_1, \ldots ,\nu_d})
    \bigotimes_{i=1}^d \, \vek{w}^{(i)}_{\nu_i}. 
\end{equation*}
The computational cost is $\C{O}( \prod_{i=1}^d r_i)$ (or simpler $\C{O}(r^d)$) 
operations, and no change in rank and storage.
%
\paragraph{Addition of two Tucker tensors} is computed as follows:
\begin{align*}
\tnb{w}  &= \tnb{u}+\tnb{v}= 
  \sum_{\vek{\mu}}^{\vek{\rho}} \Shat{u}_{\vek{\mu}} \bigotimes_{i=1}^d \vek{u}^{(i)}_{\mu_i}
  + \sum_{\vek{\nu}}^{\vek{r}} \Shat{v}_{\vek{\nu}} \bigotimes_{i=1}^d \vek{v}^{(i)}_{\nu_i}  \\
  \nonumber
  &= \sum_{\vek{\mu}}^{\vek{\rho}+\vek{r}} \Shat{w}_{\vek{\mu}}
     \bigotimes_{i=1}^d \vek{w}^{(i)}_{\mu_i}, \quad
     \text{--- with }  \vek{\mu} = (\mu_1,\dots,\mu_d), \text{ and similarly } 
     \vek{\nu}, \vek{\rho}, \vek{r} \text{ ---}
\end{align*}
and where the core tensor $\That{w}=(\Shat{w}_{\mu_1,\ldots,\mu_d})\in  
\D{R}^{(\rho_1+r_1)} \otimes\ldots \otimes \D{R}^{(\rho_d+r_d)}$
of order $d$ consists of the two blocks of core tensors $\That{u}$ and $\That{v}$, i.e.\ 
$(\Shat{u}_{\mu_1,\ldots,\mu_d}), (\Shat{v}_{\mu_1,\ldots,\mu_d})$ on the main diagonal.
In more detail
\begin{equation*}
\Shat{w}_{\mu_1,\ldots,\mu_d} = \begin{cases} 
      \Shat{u}_{\mu_1,\ldots,\mu_d} &\text{if }   \mu_1\le\rho_1,\ldots,\mu_d\le\rho_d \\
      \Shat{v}_{\mu_1-\rho_1,\ldots,\mu_d-\rho_d} &\text{if }
      0< \mu_1-\rho_1\le r_1,\ldots,0<\mu_d-\rho_d\le r_d       \\
      0 &\text{otherwise}. 
   \end{cases}
\end{equation*}

Similarly, the vectors $\vek{w}^{(i)}_{\mu_i} \in \D{R}^{M_i}$ are constructed from 
$\vek{u}^{(i)}_{\mu_i}\in \D{R}^{M_i}$ and $\vek{v}^{(i)}_{\nu_i} \in \D{R}^{M_i}$
as follows for $i=1,\dots,d$ and $\mu_i = 1,\dots,\rho_i+r_i$:
\begin{equation*}
\vek{w}^{(i)}_{\mu_i} = \begin{cases} 
      \vek{u}^{(i)}_{\mu_i}        &\text{ if } \mu_i\le\rho_i \\
      \vek{v}^{(i)}_{\mu_i-\rho_i} &\text{if } 0<\mu_i-\rho_i\le r_i . 
   \end{cases}
\end{equation*}
For details see \citep{HA12, khorBook18}.
The computational cost is again $\C{O}(1)$ since only more memory needs to be allocated,
but the rank generally increases to the sum of the individual ranks of $\tnb{u}$ and $\tnb{v}$.



\paragraph{The Hadamard product} of two tensors given in Tucker format is computed
 as follows:
\begin{equation*}
 \tnb{u}\odot\tnb{v}:=\sum_{\nu}^{\vek{r}_u}
 \sum\limits_{\mu }^{\vek{r}_v}
 \Shat{u}_{\nu_1, \ldots ,\nu_d}
 \Shat{v}_{\mu_1, \ldots ,\mu_d}\, \bigotimes_{i=1}^d
\left({\vek{u}}^{(i)}_{\nu_i}\odot {\vek{v}}^{(i)}_{\mu_i}\right).
\end{equation*}
Note \citep{khoromskaia2018tensor} that the new Tucker core has size $r^{2d}$,
i.e.\ the ranks get multiplied.
The storage cost of the Hadamard product is $\C{O}(d\,r^2\,n+r^{2d})$.
%\textbf{Matrix-by-vector product.}\\


\paragraph{The Euclidean inner product} is computed as follows:
\begin{equation*}
\bkt{\tnb{u}}{\tnb{v}}_{\C{T}}:=\sum_{\nu}^{\vek{r}_u}  \sum_{\mu }^{\vek{r}_v}
 \Shat{u}_{\nu_1, \ldots ,\nu_d}  \Shat{v}_{\mu_1, \ldots ,\mu_d}\,
\prod_{i=1}^d    \bkt{\vek{u}^{(i)}_{\mu_i}}{\vek{v}^{(i)}_{\nu_i}}_{\C{P}_i}.
\end{equation*}
The overall computational complexity of the inner product is $\C{O}(d\,n\,r^2+r^{2d})$.\\


\subsubsection{Rank truncation in the Tucker format}
%
To truncate the Tucker tensor rank from $2r$ or $r^2$ back to $r$ the high order SVD 
(HOSVD) algorithm together with ALS iterations are applied \citep{DMV-SIAM2:00}.
As the set of Tucker tensors of fixed rank is closed, the best approximation exist, 
and there is an algorithm with quadratic convergence in the energy norm.
One may compare this to the matrix case, where the SVD yields a best low-rank 
approximation. %[R.A.Horn and C.R. Johnson, Sec. 7.4.9]
The truncated tensor $\tnb{w}^*$ resulting from the HOSVD could be sub-optimal, 
but nevertheless the following inequality holds
\begin{equation}
\label{eq:minim_prob}
\Vert \tnb{w} - \tnb{w}^*\Vert \leq \sqrt{d}\cdot \min_{\tnb{v}\in 
%  U_{T,\vek{r}}(k_1,...,k_d)} \Vert \tnb{w} -\tnb{v}\Vert. 
\tns{U}_{\Tuck,\vek{r}}(\tnb{P})} \Vert \tnb{w} -\tnb{v}\Vert. 
\end{equation}
For some improved estimates see \citep{Tucker_trunk12}.

The most time-consuming part of the Tucker algorithm is the HOSVD procedure. 
Namely, the computation of the initial guess using
the SVD of the matrix unfolding of the original tensor \citep{DMV-SIAM2:00}. 
The numerical cost of Tucker decomposition for full size tensors is 
$\C{O}(n^{d+1})$. 
%
%

%\textcolor{red}{Add pictures about CP, Tucker and TT formats.}\\
%\textcolor{red}{Addition in Tucker format to add}\\
%\textcolor{red}{PUT THE SAME ORDER OF SECTIONS}\\

%
%

\subsection{The Tensor Train format}
%
The tensor train (TT) format is described in \citep{OSTY09, OS11, HA12,  khorBook18}.
As already noted, it was originally developed in quantum chemistry as ``matrix product
states'' (MPS), see  \citep{VI03} and references therein, and rediscovered later
\cite{oseledetsTyrt2010, oseledets2011}.
For a motivation, let us start with a well-known example \citep{Kazeev_Laplace_TT}.
\begin{example}
Consider the $d$-dimensional Laplacian operator discretised 
with standard finite differences over a uniform 
tensor grid with $n$ degrees of freedom in each direction.
It has the Kronecker (canonical) rank-$d$ representation:
\begin{equation*}
\tnb{A} = \vek{A}\otimes 
\overbrace{\vek{I} \otimes \cdots \otimes \vek{I}}^{d-1 \text{\rm{} \; times}} + 
\vek{I} \otimes \vek{A} \otimes \vek{I} \cdots \otimes \vek{I}  
+ \cdots + \vek{I}\otimes\cdots  \otimes \vek{I}\otimes \vek{A} \in \D{R}^{n^d \times n^d}
\end{equation*}
with $\vek{A}= \text{\rm tridiag}\{-1,2,-1\}\in \D{R}^{n \times n}$, and $\vek{I}$ being the 
$n \times n$ identity.
However, the same operator in the TT format is explicitly representable with 
all TT ranks equal to 2 for any dimension \citep{Kazeev_Laplace_TT},
\begin{equation*}
\tnb{A}=  
 \begin{pmatrix}
  \vek{A}, & \vek{I}
 \end{pmatrix}
 \Join
 \overbrace{
 \begin{pmatrix}
  \vek{I} & \vek{0} \\
  \vek{A} & \vek{I}
 \end{pmatrix}\Join
\dots
 \Join
 \begin{pmatrix}
  \vek{I} & \vek{0} \\
  \vek{A} & \vek{I}
 \end{pmatrix}
 }^{d-2 \text{\rm{} \; times}}
 \Join
 \begin{pmatrix}
  \vek{I}  \\
  \vek{A}
 \end{pmatrix},
 \end{equation*}
where the ``strong Kronecker'' product operation `` $\Join $ '' is defined as a regular matrix 
product for the first level of TT cores, i.e.\ the block matrices, 
and the inner blocks  are multiplied by means of the Kronecker or tensor product \cite{Matthies2020}.
% for example 
% \[
%  \begin{pmatrix}  \vek{A}, & \vek{I} \end{pmatrix}  \Join  \begin{pmatrix}
%   \vek{I} & \vek{0} \\   \vek{A} & \vek{I} \end{pmatrix} = \begin{pmatrix}  
%   \vek{A} \otimes \vek{I}+\vek{I} \otimes \vek{A}, & \vek{I}\otimes \vek{I} \end{pmatrix} .
% \]
Every element of $\tnb{A}$ can be computed as follows:
\[
\tnb{A}[\vek{i},\vek{j}] =
\begin{pmatrix}\vek{A}[i_1,j_1] & \vek{I}[i_1,j_1]\end{pmatrix}
\begin{pmatrix}
 \vek{I}[i_2,j_2] & 0 \\
 \vek{A}[i_2,j_2] & \vek{I}[i_2,j_2]
 \end{pmatrix} \cdots
 \begin{pmatrix}
  \vek{I}[i_d,j_d]  \\
  \vek{A}[i_d,j_d]
 \end{pmatrix}.
\]
\end{example}
%
%\note{A few more words here to close the example}.
% Thus, the $d$-dimensional Laplacian operator is separable with TT ranks equal to 2,
% and each TT component (core) is defined by a one-dimensional Laplacian.


\begin{definition}[TT-Format, TT-Representation, TT-Ranks]\label{D:TTFormat}
The \emph{TT-tensor format} is for variable \emph{TT-representation
ranks} $\vek{r}=(r_0, \dots, r_{d})\in \D{N}^{d+1}$ --- with $r_0 = r_d = 1$ and
under the assumption that $d>2$ --- defined by the
following multilinear mapping
\begin{align}   \label{eq:TTRepresentation}
  \tns{U}_{\TT} : \C{P}_{\TT,\vek{r}} &:=  \bigtimes_{\nu=1}^{d} 
  \C{P}_\nu^{r_{\nu-1} \times r_{\nu}}
  \rightarrow   \C{T},\quad \C{P}_\nu = \D{R}^{M_\nu}\; (\nu=1,\dots,d),   \\ \nonumber
   \C{P}_{\TT,\vek{r}}\ni\tnb{P} &=(\tnb{W}^{(\nu)} = (\vek{w}^{(\nu)}_{j_{\nu-1} j_\nu})
   \in\C{P}_\nu^{r_{\nu-1} \times r_{\nu}} :1\le j_\nu\le r_\nu, 1\le\nu\le d) \\ \nonumber
   &\qquad\mapsto 
   \tns{U}_{\TT}(\tnb{P}):=\tnb{w}=\sum_{j_0=1}^{r_0}\dots\sum_{j_d=1}^{r_d} 
     \Ten_{\nu=1}^{d} \vek{w}_{j_{\nu-1} j_\nu}^{(\nu)} \; \in \C{T}.
\end{align}
We call  $\tnb{w}:=(\tns{w}_{i_1\dots i_d})=U_{\TT,\vek{r}}(\tnb{P})$ a tensor 
represented in the train tensor format.
Note that the TT-cores $\tnb{W}^{(\nu)}$ may be viewed as a vector 
valued $r_{\nu-1}\times r_\nu$ matrix
with the vector $\vek{w}^{(\nu)}_{j_{\nu-1} j_\nu}\in\D{R}^{M_\nu}$ with the components
$w^{(\nu)}_{j_{\nu-1} j_\nu}[i_\nu]: 1\le i_\nu \le M_\nu$
at index position $(j_{\nu-1}, j_\nu)$.    The representation in components is then
\begin{equation}   \label{eq:TTRep-comp-1}
  (\tns{w}_{i_1\dots i_d})=\sum_{j_0=1}^{r_0} \dots \sum_{j_{d}=1}^{r_{d}} 
  w_{j_0 j_1}^{(1)}[i_1] \cdots 
  w_{j_{\nu-1} j_\nu}^{(\nu)}[i_{\nu}] \cdots w_{j_{d-1} j_d}^{(d)}[i_d]
\end{equation}
Alternatively, each TT-core $\tnb{W}^{(\nu)}$ may be seen as a vector
of $r_{\nu-1}\times r_\nu$ matrices $\vek{W}^{(\nu)}_{i_\nu}$ of length $M_\nu$, i.e.\
$\tnb{W}^{(\nu)} = (\vek{W}^{(\nu)}_{i_\nu}):1\le i_\nu \le M_\nu$.  Then
the representation \refeq{eq:TTRep-comp-1} reads
\begin{equation}   \label{eq:TTRep-comp-2}
  (\tns{w}_{i_1\dots i_d})= \prod_{\nu=1}^d \vek{W}^{(\nu)}_{i_\nu},
\end{equation}
which explains the name \emph{matrix product state}.  Observe that the first matrix
is always a row vector as $r_0=1$, and the last matrix is always a column vector as $r_d=1$.
The matrix components $\vek{W}^{(\nu)}_{i_\nu}$ of the TT-cores are also called ``carriages''
or ``waggons'' with ``wheels'' $i_\nu$ at the bottom, coupled to the next ``carriage''
or ``waggon'' via the matrix product.  This explains the \emph{tensor train} name.
If one notes more carefully $\tnb{W}^{(\nu)} \in \C{P}_\nu^{r_{\nu-1} \times r_{\nu}} = 
\D{R}^{r_{\nu-1}} \otimes \D{R}^{M_\nu} \otimes \D{R}^{r_\nu}$, then \refeq{eq:TTRep-comp-2}
can be written more concisely as
\begin{equation}   \label{eq:TTRep-comp-3}
  \tnb{w} = \tns{U}_{\TT}(\tnb{P}) =  \tnb{W}^{(1)} \times_3^1 \tnb{W}^{(2)} \times_3^1 \cdots
  \times_3^1 \tnb{W}^{(d)} ,
\end{equation}
where $\tnb{U} \times_k^\ell \tnb{V}$ is a contraction of the $k$-th index of $\tnb{U}$
with the $\ell$-th index of $\tnb{V}$, where one often writes just $\times_k$ for
$\times^1_k$.  Thus in \refeq{eq:TTRep-comp-3} the contractions leave the indices from
the $\D{R}^{M_\nu}$ untouched, so that the tensor $\tnb{w}$ is formed.
\end{definition}

Each TT-core (or \emph{block}) $\tnb{W}^{(\nu)}$ is defined by 
$r_{\nu-1}\times r_{\nu} \times M_\nu$ numbers. Assuming $n=M_\nu$ for all $\nu=1,\ldots,d$,
the total number of entries scales as $\mathcal{O}(d\,n\,r^2)$, which is tractable 
as long as $r=\max\{r_k\}$ is moderate.

A pictorial representation of the schema for the TT tensor format is shown in Figure~\ref{fig:TT}.
It shows $d$ connected waggons with one wheel.  The waggons denote the TT-cores,
and each wheel denotes the index $i_\nu$.  The waggons for $\nu = 2,\dots,(d-1)$ are connected
with their neighbours by two indices $j_{\nu-1}$ and $j_{\nu}$.  The first and the last
waggons are connected by only one index, namely $j_1$ and $j_{d-1}$ respectively.  Since by 
the convention in \refD{TTFormat} above, $r_0=r_d=1$, the indices $j_0$ and $j_d$ run from 1 to 1, i.e.\ are purely formal.

%
\begin{figure}[h]
\centering
%\includegraphics[width=0.7\textwidth]{figs/TTtrain}\\
%\includegraphics[width=0.7\textwidth]{figs/TTtrain2.png}
\includegraphics[width=0.7\textwidth]{figs/TTTrain_1wheel.png}
\caption{Schema of the TT tensor decomposition.
The waggons denote the TT cores and each wheel denotes
the index $i_\nu$. Each waggon is connected with neighbours by indices $j_{\nu-1}$ and $j_{\nu}$.}
\label{fig:TT}
\end{figure}
%
\ignore{
All the TT-cores $\tnb{W}^{(\nu)}$ are tensors of degree 3 --- i.e.\
$\vek{W}^{(\nu)}_{i_\nu}[j_{\nu-1}, j_\nu]$ --- with indices
$j_{\nu-1}$, $i_\nu$, and $j_\nu$, representing the carriages or waggons.
The $i_\nu$ index is the wheel, and the $j_{\nu-1}$ and $j_\nu$ indices are the
``hitch'' to the preceding and the following waggon or carriage.

The first waggon in Figure~\ref{fig:TT} symbolises the TT-core $\vek{W}^{(1)}_{i_1}$,
and as $1 \le j_0 \le r_0=1$, it is only formally a tensor of degree 3, but rather
one of degree 2, i.e.\ a matrix, as the $j_0$ index is constant and hence does not really count.
The second waggon is the TT-core $\vek{W}^{(2)}_{i_2}$, and the last waggon is $\vek{W}^{(d)}_{i_d}$. 
The first waggon is connected with the second by the ``hitch'', the index $j_1$, the second with the 
third one by the index $j_2$, and the penultimate one to the last by the index $j_{d-1}$, 
see \refeq{eq:TTRep-comp-1} and \refeq{eq:TTRep-comp-3}.  Again, as $1 \le j_d \le r_d=1$,
the last waggon is really a matrix.  
}
The waggon or carriage 2 --- $\tnb{W}^{(2)}$ ---
is a tensor of degree 3, described by three 
indices $j_1$ (the left hitch), $i_2$ (the wheel), and $j_2$ (the right hitch).  
Multiplication of the third TT-core with the second 
and forth cores means the tensor contraction by the indices $j_1$ and $j_2$.  If we perform 
tensor contraction of all TT-cores over the indices $j_1,\ldots,j_{d-1}$,
and disregard the purely formal constant indices
$j_0$ and $j_d$, then the indices $j_0,\ldots,j_{d}$ --- the hitches --- will disappear, and 
only the indices $i_1,\ldots,i_d$ --- the wheels --- will be left.  


%Each TT representation (Equations \ref{eq:TTRep-comp-1} and \ref{eq:TTRep-comp-2}) is 
%convenient for its own purposes.
% The first one is a formal statement that a tensor $\tnb{u}$ is presented in the TT format, 
% which may be used if we change one block, for example.
% The second line is the most expanded elementwise definition, showing the polylinearity of the format.
% \textcolor{red}{NEED TO CHANGE NOTATION The third line is the seminal Matrix Product form: 
% after fixing $\alpha_k$, each block $u^{(\nu)}(\alpha_k)$ has only two indices $s_{k-1},s_k$, 
% and may be considered as a matrix.
% Thus, the TT format means that each element of $u$ is presented as a product of matrices.
% Finally, the fourth line is an analog of the \emph{Canonical Polyadic} decomposition, 
% convenient to compare the structures in both formats.
% Surely, in the same form we may write e.g. $\kappa_{\alpha} = \kappa^{(1)}(\alpha_1) 
% \cdots \kappa^{(M)}(\alpha_M)$.
% }



% As mentioned for the tensor formats above, the numerical cost for
% operation with tensors represented in the TT-format is linear in
% $d$, see for example \cite{HA12, OS11, OSTY09}.
% %


\subsubsection{Basic operations with the TT format}
%
We follow to the work of Oseledets \citep{OS11} and list the major properties of the 
TT-tensor format.

\paragraph{The multiplication with scalar} $\alpha$ could be simply
done by multiplying one of the TT-cores $\tnb{W}^{(\nu)}$ in the
representation \refeq{eq:TTRep-comp-3} for any $\nu$ in
$\tnb{w} =  \tnb{W}^{(1)} \times_3^1 \tnb{W}^{(2)} \times_3^1 \cdots
  \times_3^1 \tnb{W}^{(d)}$.
But to balance the effect better, define $\alpha_{\nu} := \sqrt[d]{|\alpha|}$ for all $\nu > 1$,
and $\alpha_{1} := \sign(\alpha)\sqrt[d]{|\alpha|}$.  Then $\Ttil{w} = \alpha\cdot\tnb{w}$
is given by
\[  \Ttil{w} =  (\alpha_1\cdot\tnb{W}^{(1)}) \times_3^1 
  (\alpha_2\cdot\tnb{W}^{(2)}) \times_3^1 \cdots  \times_3^1 (\alpha_d\cdot\tnb{W}^{(d)})
  = \Ttil{W}^{(1)}\times_3^1 \cdots \times_3^1 \Ttil{W}^{(d)}.
\]
The new cores are given by $\Ttil{W}^{(\nu)} = (\vtil{W}^{(\nu)}_{i_\nu})
= (\alpha_\nu \vek{W}^{(\nu)}_{i_\nu})$, a sequence of new ``carriage'' matrices. 
The computational complexity is $\mathcal{O}(d\,n\,r^2)$.


\paragraph{Addition of two TT-tensors}
Assume two tensors $\tnb{u}$ and $\tnb{v}$ are given in the TT-tensor format
as in \refeq{eq:TTRep-comp-2}, i.e.\
$(\tns{u}_{i_1\dots i_d})= \prod_{\nu=1}^d \vek{U}^{(\nu)}_{i_\nu}$ and 
$(\tns{v}_{i_1\dots i_d})= \prod_{\nu=1}^d \vek{V}^{(\nu)}_{i_\nu}$.  The sum
$\tnb{w}=\tnb{u}+\tnb{v}$ is given by the new cores $\vek{W}^{(\nu)}_{i_\nu}$ such that
$(\tns{w}_{i_1\dots i_d})= \prod_{\nu=1}^d \vek{W}^{(\nu)}_{i_\nu}$, where
\begin{equation*}
    \vek{W}^{(\nu)}_{i_\nu}=
\begin{pmatrix}
\vek{U}^{(\nu)}_{i_\nu} & \vek{0} \\
 \vek{0} & \vek{V}^{(\nu)}_{i_\nu} 
\end{pmatrix}, \quad 1\le i_\nu \le r_\nu, 2\le\nu\le d-1.
\end{equation*}
and the first and the last cores will be 
\[
\vek{W}^{(1)}_{i_1}=\left(\vek{U}^{(1)}_{i_1}\; \vek{V}^{(1)}_{i_1} \right)  \quad \text{ and } 
\quad
\vek{W}^{(d)}_{i_d}=\left( \begin{array}{c} \vek{U}^{(d)}_{i_d} \\ \vek{V}^{(d)}_{i_d}
\end{array} \right).
\]
As only storage may have to be concatenated, the computational cost is $\C{O}(1)$,
but as  the carriages resp.\ TT-cores grow, the final rank will generally be the
sum of the ranks.


\paragraph{The Hadamard product} $\tnb{w}=\tnb{u} \odot \tnb{v}$ in the TT format
 is computed as follows.  Assume two tensors $\tnb{u}$ and $\tnb{v}$ are given in 
 the TT tensor format as in \refeq{eq:TTRep-comp-2}, i.e.\
$(\tns{u}_{i_1\dots i_d})= \prod_{\nu=1}^d \vek{U}^{(\nu)}_{i_\nu}$ and 
$(\tns{v}_{i_1\dots i_d})= \prod_{\nu=1}^d \vek{V}^{(\nu)}_{i_\nu}$.  The Hadamard product is
\[
    (\tns{w}_{i_1\dots i_d}) = (\tns{u}_{i_1\dots i_d} \cdot \tns{v}_{i_1\dots i_d}) .
\]
The tensor $\tnb{w}$ has also the TT-tensor format, namely with the new cores
\[
   \vek{W}^{(\nu)}_{i_\nu} = \vek{U}^{(\nu)}_{i_\nu}\otimes_{\mrm{K}} \vek{V}^{(\nu)}_{i_\nu}, 
   \quad 1\le i_\nu \le r_\nu, 1\le\nu\le d ,
\]
where $\otimes_{\mrm{K}}$ is the Kronecker product of two matrices \citep{HA12}.
The rank of $\tnb{W}^{(\nu)} = (\vek{W}^{(\nu)}_{i_\nu})$ is the product
of the ranks of the TT-cores  $\tnb{U}^{(\nu)}$ and $ \tnb{V}^{(\nu)}$.


\paragraph{The Euclidean inner product} of two tensors in the TT-format
as in \refeq{eq:TTRepresentation} 
\begin{equation*}
\tnb{u} = \sum_{j_0=1}^{r^u_0}\dots\sum_{j_d=1}^{r^u_d} 
     \Ten_{\nu=1}^{d} \vek{u}_{j_{\nu-1} j_\nu}^{(\nu)} , \qquad
\tnb{v} = \sum_{j_0=1}^{r^v_0}\dots\sum_{j_d=1}^{r^v_d} 
     \Ten_{\nu=1}^{d} \vek{v}_{j_{\nu-1} j_\nu}^{(\nu)} ,
\end{equation*}
with ranks $\vek{r}^u$ and $\vek{r}^v$ can be computed as follows:
%\left ( \bA,\bB\right)
\[
\bkt{\tnb{u}}{\tnb{v}}_{\C{T}}= \sum_{j_0=1}^{r^u_0}\dots\sum_{j_d=1}^{r^u_d}
  \sum_{i_0=1}^{r^v_0}\dots\sum_{i_d=1}^{r^v_d}  \prod_{\nu=1}^d \;
       \bkt{\vek{u}_{j_{\nu-1} j_\nu}^{(\nu)}}{\vek{v}_{i_{\nu-1} i_\nu}^{(\nu)}}_{\C{P}_\nu}.
\]
%The obtained ranks in $\tnb{w}$ are again the products of corresponding ranks in $\tnb{u}$ and 
%$\tnb{v}$.  
The computational complexity is $\C{O}(d\,n\,r^4)$, and can be reduced further \citep{OselTT}. 
%Having the dot product above, we can compute the Frobenius \textbf{norm} $\Vert \tnb{w} \Vert_F =\sqrt{\dotprod{\tnb{w}}{\tnb{w}}}$.\\ 
%For truncation of ranks see \cite{OS11}.
%
%The \textbf{matrix-by-vector product} in the TT-format costs $\C{O}(dn^2r^4)$ (see more details in \cite{OS11}).
%
%

\subsubsection{Rank truncation in the TT format}
%
The rank truncation operation is based on the SVD algorithm and requires 
$\C{O}(d\,n\,r^3)$ operations \citep{GrasHack11}.  The TT-rounding algorithm (p. 2305 in \citep{oseledets2011}) is based on QR decomposition and costs $\C{O}(d\,n\,r^3)$.

Corollary 2.4 in \citep{oseledets2011} states that for a given tensor $\tnb{w}$ and
rank bounds $r_k$, the best approximation to $\tnb{w}$ in the Frobenius norm with TT-ranks 
bounded by $r_k$ always exist (denote it by $\tnb{w}^*$), and the TT-approximation 
$\tnb{u}$ computed by the TT-SVD algorithm (p. 2301 in \citep{oseledets2011}) is quasi-optimal:
\begin{equation}
    \Vert \tnb{w}-\tnb{u} \Vert_F\leq \sqrt{d-1} \Vert \tnb{w} - \tnb{w}^{*} \Vert_F.
\end{equation}
%$\C{O}(dnr^6)$ operations.
In \cite{Kressner17_Trunc} the authors suggested a new re-compression 
randomised algorithm for Tucker and TT tensor formats. Rank-adaptive DMRG-cross algorithm see in \cite{so-dmrgi-2011proc}




%  $Log: other_tensor_formats.tex,v $
%  Revision 1.3  2021/11/07 22:37:56  hgm
%  added header and footer
%
%  Revision 1.12  2021/11/07 22:19:10  hgm
%  added header and footer
%
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 






==> chaptersV2/some_extra.tex <==
% !TEX root = ../19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

\subsection{Approximation of $d$-dimensional Gaussian density function}

To test our approach (shown on the diagram in Section~\ref{S:intro}), we consider the case when both the \pdf and its characteristic functions are available analytically.

Assume that $p_{\vX}(\by)$ and  $\vphi_{\vX}(\bt)$ are given. Compute a low-rank approximation of  
  $\vphi_{\vX}(\bt)$, apply the inverse Fourier transformation, obtain a new 
  $\tilde{p}_{\vX}(\by)$, and compare $p_{\vX}(\by)$ and $\tilde{p}_{\vX}(\by)$.
%

\subsection{Approximation of multivariate elliptically contoured stable distribution}
Here we research how tensor ranks and approximation error depend on 
parameter $\alpha$ in multivariate elliptically contoured stable distributions.


\subsection{Approximation of multivariate $\alpha$-stable distribution}
Here we research how tensor ranks and approximation error depend on 
parameter $\alpha$ in multivariate $\alpha$-stable distributions.


\subsection{Approximation of multivariate geometrical $\alpha$-stable distribution}
Here we research how tensor ranks and approximation error depend on 
parameter $\alpha$ in multivariate geometrical $\alpha$-stable distributions.



\subsection{Appendix A : High-dimensional grid functions}
Assume that there is a $d$-dimensional regular grid. Let there is a following regular discretization in $j$-th dimension
$\tau_{\ell}=\{t_1^{(\ell)},..., t_{n_{\ell}}^{(\ell)}\}$. Then the whole grid can be defined as the following product
\begin{equation}  \label{eq:T}
\bigotimes\mT=\left[ \mT_{\beta}\right]=\tau_1\times\tau_2\times...\times \tau_d=
\bigotimes_{\ell=1}^d \tau_{\ell}\in \mathbb{R}^{n_1\times n_2 ... \times n_d},\,\quad \tau_{\ell}\in \mathbb{R}^{n_{\ell}},  
%\bigotimes_{\ell=1}^dt_{\beta_{\ell}},\quad t_{\beta_{\ell}}\in \mathbb{R}^{n_{\ell}},  
\end{equation}
The grid $\mT$ contains $N:=n_1\times... \times n_{d}$ nodes.
%each node has $d$ coordinates
Each nodal point $\vt\in  \mT$ is indexed by a $d$-tuple $[i_1,...,i_d]$ with $1\leq i_{\ell} \leq n_{\ell}$: $\vt[i_1,...,i_d]=(t_{i_1}^{1},...,t_{i_d}^{d})$.
A grid function $u$ defined on $\mT$ is characterized by the nodal values $u[i_1,...,i_d]\in \mathbb{R}^N$. There is an isomorphysm 
\begin{equation}
\mathbb{R}^N\simeq \mathbb{R}^{n_1}\otimes...\otimes \mathbb{R}^{n_d}.
\end{equation}

Another Notation: $\tau_{\ell}=[t_{1,\ell},...,t_{\beta_{\ell},\ell},...,t_{n_{\ell},\ell}]^T\in \mathbb{R}^{n_{\ell}}$.
Each node has $d$ coordinates and can be described by the multi-index $\beta=(\beta_1,...,\beta_d)$, $\beta_{\ell}=1..n_{\ell}$.
Let us say that $\beta \in \mathcal{I}_{\beta}$, where $\mathcal{I}_{\beta}:=\{(\beta_1,...,\beta_d),\quad \vert \beta_{\ell}\in{1,...,n_{\ell}}\}$.
\\ 


\begin{example}[Bivariate Cauchy distribution] %\label{Motiv:Cauchy}
%
If we set $d=2$ and $\alpha=1/2$ in \refeq{eq:motiv_ch2}, then we obtain the well-known bi-variate 
Cauchy distribution.
for $\bt=(t_1, t_2)\in\D{R}^2$ is defined as follows:
\begin{equation}
\label{eq:motiv_ch}
\varphi_{\vX}(\bt)=\exp \left( \ii(t_1,t_2)\cdot (\mu_1,\mu_2)^T -\sqrt{\frac{1}{2}(t_1,t_2)
\left(
\begin{array}{cc}
 \sigma_1^2 & 0     \\
 0 & \sigma_2^2   \\
 \end{array}
\right)(t_1, t_2)^T}
\right),
\end{equation}
It is not analytically separable, but it is possible to find a numerical rank-$k$ approximation. One can use the SVD algorithm or some heuristics:

\begin{equation}
\vphi_{\vX}(\bt)\approx \tilde{\vphi}_{\vX}(\bt)= \sum_{\nu=1}^R\vphi_{\nu,1}(t_1)
\cdot \vphi_{\nu,2}(t_2).
\end{equation}
%
% \begin{remark}
% A difficult task here is to find an 'optimal' (minimal) 
% rank $R$ and functions $\vphi_{\nu,1}(t_1)$,  $\vphi_{\nu,2}(t_2)$.
% \end{remark} 
%
% From the inversion theorem, the probability density of $\vX$ on $\D{R}^2$ 
% can be computed from $\vphi_{\vX}(\bt)$ as follows
% \begin{equation}  \label{eq:motiv_inv4}
% p_{\vX}(\by)=\frac{1}{(2\uppi)^2}
%   \int_{\D{R}^2} \exp(-\ii \ip{\by}{\bt})\vphi_{\vX}(\bt)\di\bt, 
%     \quad \by \in \D{R}^2.
% \end{equation}

% We can rewrite it as follows
% \begin{align}  \label{eq:motiv_inv5}
% p_{\vX}(\by)&=\frac{1}{(2\uppi)^2}\int_{\D{R}^2}\exp(-\ii\ip{\by}{\bt})\vphi_{\vX}(\bt)\di\bt \\
%  \nonumber &\approx \frac{1}{(2\uppi)^2} \int_{\D{R}^2} \exp(-\ii(y_1 t_1 + y_2 t_2))
% \sum_{\nu=1}^R \vphi_{\nu,1}(t_1)\cdot \vphi_{\nu,2}(t_2) \di t_1 \di t_2 \\ \nonumber
% &\approx \sum_{\nu=1}^R\frac{1}{(2\uppi)}\int_{\D{R}}\exp(-\ii y_1 t_1) \vphi_{\nu,1}(t_1)dt_1
%  \cdot  \frac{1}{(2\uppi)}\int_{\D{R}}\exp(-\ii y_2 t_2)\vphi_{\nu,2}(t_2) \di t_2 \\ \nonumber
% &\approx \sum_{\nu=1}^R p_{\nu,1}(y_1) \cdot p_{\nu,2}(y_2)
% \end{align}
% i.e.\ the probability density $p_{\vX}(\by)$ is numerically separable. 
%\end{example}
%\mbox{http://www.mathematik.uni-ulm.de/stochastik/lehre/ws02_03/statistik_2/skript/node25.html}
\end{example}
%




%  $Log: some_extra.tex,v $
%  Revision 1.3  2021/11/07 22:39:57  hgm
%  added header and footer
%
%  Revision 1.12  2021/11/07 22:19:10  hgm
%  added header and footer
%
%
%
%
%
%


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 





==> chaptersV2/tensor_CP.tex <==
% !TEX root = ../19_low-rank_tensor_prob_den_char.tex
% !TEX encoding = UTF-8 Unicode

% RCSID:       $Id: tensor_CP.tex,v 1.7 2021/11/13 10:28:05 hgm Exp $
% Authors:     Alexander Litvinenko, Youssef Marzouk, Hermann G. Matthies,
%              Marco Scavino, and Alessio Spantini
% Contact:     wire@tu-bs.de
% =================================

%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.7 $",
%%  DATE      = "$Date: 2021/11/13 10:28:05 $",
%%  FILENAME  = "$RCSfile: tensor_CP.tex,v $"}

%\section{Tensor representations} %\label{S:tensor-rep}
%



% Let $\Tp:=\Ten_{\mu=1}^d \R^{n_\mu}$ be the tensor space constructed
% from $(\R^{n_\mu}, \dotprod{}{}_{\R^{n_\mu}})$ ($d \geq 3$).
% Let the parameter space $P=\bigtimes_{\nu =1}^D P_\nu$
% ($d\leq D$) is the Cartesian product of tensor spaces $P_\nu$.
% %where
% %in general the order of every $P_\nu$ is (much) smaller then $d$.
% Further, $P_\nu$ depends on some representation rank parameter
% $r_\nu \in \N$. %From a
% %mathematical point of view, 
% A tensor representation $U$ is a
% multilinear map from a parameter space $P$ onto $\Tp$, i.e. $U : P
% \rightarrow \Tp$. A standard example of a tensor representation is the
% canonical tensor format.
% %
% \begin{definition}[r-Terms, Tensor Rank, Canonical Tensor Format, Elementary Tensor, Representation System]\label{def:CPFormat}
% The set $\Rp_r$ of tensors which can be represented in $\Tp$ with
% \emph{$r$-terms} is defined as
% %
% \begin{equation}\label{equ:Tr}
%     \Rp_r(\Tp):=\Rp_r := \left\{ \sum_{i=1}^r \Ten_{\mu=1}^d v_{i \mu} \in \Tp : v_{i \mu} \in
%     \R^{n_\mu}\right\}.
% \end{equation}
% %
% Let $v \in \Tp$. The \emph{tensor rank of $v$ in $\Tp$} is
% \begin{equation}\label{equ:tensorRang}
%     \rank(v):=\min \left\{ r \in \N_{0} : v \in \Rp_r \right \}.
% \end{equation}
% %
% The \emph{canonical tensor format in $\Tp$} for variable $r$ is
% defined by the mapping
% %
% \begin{eqnarray}\label{eqn:CanonicalFormat}
% U_{cp} : \bigtimes_{\mu = 1}^d \R^{n_\mu \times r} &\rightarrow& \Rp_{r},\\
%     \hat{v}:= (v_{i \mu}: 1\leq i \leq r, \mbox{ } 1 \leq \mu \leq d) &\mapsto& U_{cp}(\hat{v}) :=
%     \KtsS{i}{r}{d}{v}.\nonumber
% \end{eqnarray}
% %
% We call the sum of elementary tensors $v=\ktsS{i}{r}{d}{v} \in
% \Rp_r$ a tensor represented in the canonical tensor format with $r$
% terms, where an \emph{elementary tensor} is of the form
% $\Ten_{\mu=1}^d v_\mu \in \Rp_1$, $v_\mu \in V_\mu$. The system of
% vectors $\left(v_{i \mu} : 1\leq i \leq r, \mbox{ } 1\leq \mu \leq
% d\right)$ is a \emph{representation system} of $v$ with
% \emph{representation rank} $r$.
% \end{definition}
% %
% Note that the representation rank  refers to the representation
% system $(v_{i \mu}: 1\leq i \leq r, \mbox{ } 1 \leq \mu \leq d)$,
% not to the represented tensor. In our applications we work only with
% tensors represented in a tensor format. A tensor $u \in \Rp_r
% \subset \Tp$ with $\prod_{\mu=1}^d n_\mu$ entities is represented on
% a computer system with a representation system $\hat{u}= \left(u_{i
% \mu} \in \R^{n_\mu}: 1\leq i \leq r, \mbox{ } 1\leq \mu \leq
% d\right)$ and the use of $U_{cp}$, i.e. $u=U_{cp}(\hat{u})$. The
% memory requirement for the representation system $\hat{u}$ is only
% $r\sum_{\mu=1}^d n_{\mu}$. Later we will see that the efficient data
% representation in tensor formats has several benefits for the data
% analysis in high dimensions. For the data analysis we need
% operations described in Lemma \ref{lemma:operations}.
%

\newcommand{\CP}{\mrm{CP}}
\newcommand{\Tuck}{\mrm{T}}
\newcommand{\TT}{\mrm{TT}}

%



\section{Tensor formats}      \label{S:tensor-rep}
%
Our task is to approximate a high-dimensional function (e.g. a \pdf) in a low-rank tensor format. After discretisation of the high-dimensional function on a grid, we obtain a tensor, which is also a high-dimensional object. Now we need an appropriate \textit{tensor representation}, which will make efficient storage and efficient multi-linear algebra possible.
In this section, we give a short overview of known tensor representations (tensor formats) and review definitions and properties of the canonical polyadic (CP) tensor format.

Many tensor formats are used in quantum physics under the name \emph{tensor networks},
see \citep{VI03, Sachdev2010-a, EvenblyVidal2011-a, Orus2014-a, 
BridgemanChubb2017-a, BiamonteBergholm2017}. 
%We only look
%at the \emph{canonical polyadic} (CP), the \emph{Tucker}, and the \emph{Tensor Train}
%(TT) format.  
The CP \citep{Hitch:27} and \emph{Tucker} \citep{Tuck:66} formats 
have been well known for a long time and are therefore very
popular. For instance, CP and Tucker rank-structured tensor formats have been 
applied in chemometrics and in signal processing \citep{smilde-book-2004, Cichocki:2002}. 
The \emph{Tensor Train} format was originally developed in quantum physics and
chemistry as ``matrix product states'' (MPS), see \citep{VI03} and references therein, 
and rediscovered in \cite{oseledetsTyrt2010, oseledets2011} as tensor train.

A new class of tensor formats, which 
we do not consider here, is the hierarchical 
tensor (HT) format.  It was introduced in \citep{HackbuschKuhn2009}, and further 
considered in \citep{Grasedyck2010}.

We note that the sets of low-rank tensors 
of fixed rank in the CP format are not closed for $d>2$, whereas
in the Tucker, TT, or HT tensor formats these sets are closed. Linear algebra operations in the TT and HT formats
are based on the \emph{singular value decomposition} (SVD) \citep{OSTY09, Grasedyck2010}, 
and in the Tucker format on the  \emph{higher order SVD} (HOSVD) \citep{Tucker_trunk12}. 
In all tensor formats the tensor rank doubles for addition and squares for the
Hadamard product.  To avoid unnecessary and harmful rank growth,
the rank is usually truncated, e.g.\ by ALS-like or other optimisation algorithms 
\citep{EspigDiss, Espig2012VarCal}.

The idea of separation of variables lies behind of each tensor format. 
Separation of variables can be obtained by, e.g.\ applying the Taylor expansion,
 or decomposing in a Lagrange basis \citep{Winter}.

A tensor format is described by a
parameter vector space $\C{P}=\bigtimes_{\nu=1}^{d} \C{P}_\nu$,
where $\C{P}_\nu = \D{R}^{d_\nu}$, and a multilinear map 
$\tns{U}:\C{P} \rightarrow \C{T}$ into the tensor space 
$\C{T}:=\bigotimes_{\ell=1}^d \D{R}^{M_\ell}$.
For practical implementations of high dimensional problems we need
to distinguish between a tensor $\tnb{w} \in \C{T}$ and its tensor format
representation $\tnb{C} \in \C{P}$, where $\tnb{w}=\tns{U}(\tnb{C})$.  There are many
possibilities to define tensor formats.  Here, due to not so complicated notation, we
consider for the sake of simplicity only the
CP format and its properties \citep{HA12}. For the actual numerical tests we will use 
the tensor train (TT) data format. 
We also note that the reader can invent his or her own tensor format, which
fits especially well to the user's needs.


The CP format is cheap, it is simpler than the Tucker or TT format, but, 
compared to others, there are no reliable algorithms to compute CP decompositions 
for $d>2$ \citep{HA12, khorBook18}.
The Tucker format has stable algorithms \citep{Khoromskij_Low_Tacker}, 
but the storage and complexity costs are 
 $\C{O}(d\,r\,n +r^d)$, i.e.\ they grow exponentially with $d$. 
The TT format is a bit more complicated, but does not have this disadvantage.




% , assume that in the above example the data has
% been stored in the matrix $\vek{W}\in\D{R}^{M\times M}$, where $M=10^8=\sqrt{N}$,
% and consider its singular value decomposition (SVD)
% $\vek{W}=\vek{U}\vek{\Sigma}\vek{V}^\trpos = \sum_{m=1}^M \vsigma_m \vek{u}_m \vek{v}_m^\trpos$,
% where  $\vek{\Sigma}=\diag(\vsigma_1,\dots,\vsigma_M)$ is the diagonal matrix
% of singular values $\vsigma_m\ge 0$, assumed arranged by decreasing value,
% and $\vek{U}=[\vek{u}_1,\dots,\vek{u}_M]$,
% $\vek{V}=[\vek{v}_1,\dots,\vek{v}_M]$ collect the right and left singular vectors.
% Often there is a number $r\ll M$, such that for some small $\vepsilon>0$ one has
% $\vsigma_m \le \vepsilon$ for all $m>r$. Then one can formulate a compressed or
% truncated version 
% \[
% \vek{W}\approx\vek{W}_r =\vek{U}_r\vek{\Sigma}_r\vek{V}_r^\trpos
% =\sum_{m=1}^r \vsigma_m \vek{u}_m \vek{v}_m^\trpos
% =\sum_{m=1}^r  \vek{w}^{(1)}_m \otimes \vek{w}^{(2)}_m,
% \] 
% where $\vek{\Sigma}_r=\diag(\vsigma_1,\dots,\vsigma_r)$,
% $\vek{U}_r=[\vek{u}_1,\dots,\vek{u}_r]$, $\vek{V}_r=[\vek{v}_1,\dots,\vek{v}_r]$,
% and $\vek{w}^{(1)}_m = \sqrt{\vsigma_m} \vek{u}_m$, $\vek{w}^{(2)}_m = \sqrt{\vsigma_m} \vek{v}_m$.

%Another difference between tensors and matrices is that a
%matrix has only one rank, whereas a tensor may have many ranks. (obtained, for instance, 
%after the discretization 
%of a function $f(\bx,\by)=f(\vert \bx-\by\vert)$) separates a point $\bx=(x_1,...,x_d)\in \mathbb{R}^{d}$ from 
%a point $\by=(y_1,...,y_d)\in \mathbb{R}^{d}$, whereas the corresponding tensor (depending on tensor format) 
%separates $x_1-y_1$ from $x_2-y_2$... and $x_d-y_d$. This implies that tensors may have $d$ ranks $\br=(r_1,\ldots,r_d)$. In such case we speak about \textit{tensor rank}. 


\subsection{The canonical polyadic (CP) tensor format \AL{I rewrote it and shortened}}   \label{SS:CPFormat}
%
The CP representation of a multivariate function is one of the easiest tensor representations, it was developed in \citep{Hitch:27}. Schematically it is shown 
in 
Figure~\ref{fig:CP}, where a full tensor 
$\tnb{w}\in \D{R}^{n_1\times n_2\times n_3}$ (on the left) is represented as a sum of tensor products
(on the right). The lines on the right denote vectors
$ \vek{w}_{i,k} \in \mathbb{R}^{n_k}$, $i=1,\dots,r$, $k=1,2,3$.

%
\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{figs/CP1_point2.png}\quad\quad
\caption{Representation of a 3D tensor in the CP tensor format.}
\label{fig:CP}
\end{figure}
%

Tensor representation is a multi-linear mapping. There are many different representations, e.g., CP tensor representation maps tensor $\tnb{w}$ into the sum with $r$ terms $\sum_{i=1}^r \Ten_{\nu=1}^d \vek{w}_{i,\nu}$. The number $r$ is called the tensor rank.
The storage required to store a tensor in the CP tensor format is  $\C{O}(r\,d\,n)$ (assuming that $n=n_1=\ldots=n_d$).  To compute an element $(j_1,j_2,j_3)$, denoted by the red point on the left, we should compute the following sum
$\sum_{i=1}^r \vek{w}_{i,1}(j_1)\cdot \vek{w}_{i,2}(j_2)\cdot \vek{w}_{i,3}(j_3)$. The values $\vek{w}_{i,1}(j_1)$, $\vek{w}_{i,2}(j_2)$, and $\vek{w}_{i,3}(j_3)$ are denoted by the red points on the right hand side in Fig.~\ref{fig:CP}.
%


% \subsubsection{Basic operations with the canonical format \ALc{rewrite, it is copy/paste from previous}}  \label{SSS:CP-ops}
% \ALc{Delete or rewrite?}
%
%Let $\tnb{w}=U_{CT,r}(\tnb{p})=\sum_{j=1}^r \Ten_{\nu=1}^d \tns{w}_{j \nu}$ be
%represented in the canonical tensor format with $r$-terms and
%representation system $\tnb{w}\in P_{CT,r}$. The storage size for the parameter system is $\mathcal{O}(rdn)$.
%
%Numerical operations with tensors represented in the canonical
%format can be performed linear in $K$ \note{what is $K$?}. For instance, let
%$\tnb{w}=\sum_{i=1}^s \Ten_{\nu=1}^d \tns{w}_{i\nu} \in \Ten_{\nu=1}^d \R^{n
%\times n}$.

Let us denote the set of all rank-$r$ tensors by $\C{T}^r$. We note that if $\tnb{w}_1,\tnb{w}_2 \in \C{T}^r$, then $\tnb{w}_1+\tnb{w}_2 \notin  \C{T}^r $, and, therefore, $\C{T}^r$ is not a vector space \citep{Espig2012VarCal}. This sum belongs to $\C{T}^{2r}$.

%\paragraph{Matrix-vector product} $\tnb{W}\tnb{v}$ is given by
%\begin{equation*}
%    \tnb{W} \tnb{v} = \sum_{i=1}^s \sum_{j=1}^r \Ten_{\nu=1}^d \tns{W}_{i \nu} \tns{v}_{j\nu}.
%\end{equation*}
%The cost of computing $\tnb{W} \tnb{v}$ is $\C{O}\left( r \cdot s \cdot \sum_{\nu=1}^d
%n^2\right)$ arithmetic operations.

A complete description of fundamental operations in the canonical
tensor format and a their numerical cost can be found in
\citep{HA12}. For recent algorithms in the canonical tensor format we
refer to \citep{hackbusch2012tensor,  ModelReductionBook15, EspigDiss, EspigGrasedyckHackbusch2009, ESHA09_1}.
%
%Let
%$\tnb{u}=\sum_{j=1}^{k_u} \bigotimes_{\nu=1}^d \tns{u}_{j\nu}$, 
%$\tnb{u}\in \D{R}^{n^d}$,
%$\tns{u}_{j\nu} \in \RR^{n}$,
%and
%$\tnb{v}=\sum_{k=1}^{k_v} \bigotimes_{\mu=1}^d \tns{v}_{k\mu}$, 
%$\tnb{v}\in \D{R}^{n^d}$,
%$\tns{u}_{k\mu} \in \RR^{n}$.
We remind few properties \cite{Matthies2020} of the CP format. To multiply a tensor $\tnb{w}$ by a scalar $\alpha\in\D{R}$ costs $\C{O}(r\, n\, d)$:
\begin{equation}  
\label{eq:CP-scal-prod}
 \alpha\cdot \tnb{w} = \sum_{j=1}^{r} \alpha \bigotimes_{\nu=1}^d \vek{w}_{j,\nu}=
\sum_{j=1}^{r}  \bigotimes_{\nu=1}^d {\alpha_{\nu}}\vek{w}_{j,\nu},
\end{equation}
where $\alpha_{\nu} := \sqrt[d]{|\alpha|}$ for all $\nu > 1$,
and $\alpha_{1} := \sign(\alpha)\sqrt[d]{|\alpha|}$.

The sum of two tensors costs
only $\C{O}(1)$:
\begin{equation}  \label{eq:CP-add}
\tnb{w} = \tnb{u} + \tnb{v} =\left(\sum_{j=1}^{r_u} 
   \bigotimes_{\nu=1}^d \vek{u}_{j,\nu}\right) +
    \left(\sum_{k=1}^{r_v} \bigotimes_{\mu=1}^d \vek{v}_{k,\mu}\right)
  =
  \sum_{j=1}^{r_u+r_v} \bigotimes_{\nu=1}^d \vek{w}_{j,\nu} ,
\end{equation}
where $\vek{w}_{j,\nu}:=\vek{u}_{j,\nu}$ for $j\leq r_u$ and 
$\vek{w}_{j,\nu}:=\vek{v}_{j,\nu}$ for $r_u< j\leq r_u+r_v$. 
The sum $\tnb{w}$ generally has rank $r_u+r_v$.
The Hadamard product can be written as follows
\begin{equation}
\label{eq:CPHadamard}
\tnb{w}=\tnb{u} \odot \tnb{v} =
  \left(\sum_{j=1}^{r_u} \bigotimes_{\nu=1}^d \vek{u}_{j,\nu}\right) 
\odot 
  \left(\sum_{k=1}^{r_v} \bigotimes_{\nu=1}^d \vek{v}_{k,\nu}\right)
=
\sum_{j=1}^{r_u}\sum_{k=1}^{r_v} \bigotimes_{\nu=1}^d \left(\vek{u}_{j,\nu} \odot
\vek{v}_{k,\nu}\right).
\end{equation}
The new rank can increase till $r_ur_v$, and the computational cost is 
$\C{O}(r_u \,r_v n\, d)$.
The scalar product can be computed as follows:
\begin{equation}
\label{eq:CP_scalarProd}
    \bkt{\tnb{u}}{\tnb{v}}_{\C{T}} =\bkt{\sum_{j=1}^{r_u} \bigotimes_{\nu=1}^d \vek{u}_{j,\nu}}%
{\sum_{k=1}^{r_v} \bigotimes_{\nu=1}^d \vek{v}_{k,\nu}}_{\C{T}}
=
\sum_{j=1}^{r_u}\sum_{k=1}^{r_v} \prod_{\nu=1}^d 
\bkt{\vek{u}_{j,\nu}}{\vek{v}_{k,\nu}}_{\C{P}_\nu}.
\end{equation}
The computational cost is $\C{O}(r_u\,r_v\,n\,d)$. 
The tensor rank can be truncated via the ALS-method or Gauss-Newton-method \citep{EspigDiss, Espig2012VarCal}. The scalar product above helps to compute the Frobenius norm $\Vert \tnb{u} \Vert_2:=\sqrt{\bkt{\tnb{u}}{\tnb{v}}_{\C{T}}}$.




% In the following we will denote a solution
% of the approximation problem from Definition \ref{defn:appTask2}
% with $\mathfrak{App}_{\varepsilon}(v)$.
% %
% \begin{notation}\label{not:appSolution}
% Let $v \in \Rp_R$, $\varepsilon >0$ and $U_{cp}(\hat{x}^*)$ a
% solution of the approximation problem as analysed in \cite{EspigDiss,
% ESHA11_1}. 
% During the article, $U_{cp}(\hat{x}^*)$ is
% denote by
% %
% \begin{equation}\label{equ:app}
% \mathfrak{App}_{\varepsilon}(v):=U_{cp}(\hat{x}^*).
% \end{equation}
% %
% \end{notation}
%
%

\subsection{Tensor Train approximation of tensor $\tnb{w}$}
\label{sec:TT}

The tensor train format was introduced and developed in \cite{osel-tt-2011,oseledetsTyrt2010,BallaniGrasedyck2015,ds-alscross-2017pre}. The algorithms how to construct this tensor train decomposition in application to UQ problems are described in \cite{dolgov2015polynomial,DolgovLitvLiu19,dolgov2014computation}.
In our further numerical experiments we approximate $\tnb{w}$
in the Tensor Train (TT) data format \cite{osel-tt-2011}:
\begin{equation}   \label{eq:TTRep-comp-2}
  (\tns{w}_{i_1\dots i_d})= \prod_{\nu=1}^d \vek{W}^{(\nu)}_{i_\nu},
\quad 1\leq i_{\nu} \leq n_{\nu},
\end{equation}
which explains the original name \emph{matrix product state} (MPS) \citep{VI03}.
The matrices $\vek{W}^{(\nu)}_{i_\nu}$ of the size  $r_{\nu-1}\times r_\nu$ are also called ``carriages''
or ``waggons'' with ``wheels'' $i_\nu$ at the bottom, coupled to the next ``carriage''
or ``waggon'' via the matrix product.  This explains the \emph{tensor train} name. Observe that the first matrix $\vek{W}^{(0)}_{i_0}$
is always a row vector ($r_0=1$), and the last matrix  $\vek{W}^{(d)}_{i_d}$ is always a column vector ($r_d=1$).
The numbers $\{r_0,\ldots,r_d\}$ are called the \emph{TT ranks}.
For the efficiency of this representation, we assume that $\max\{r_0,\ldots,r_d\}\leq r$, where $r$ is a small integer, i.e. we assume a fast convergence of the approximation error $\varepsilon$ with the TT ranks.
Assuming $n_k \le n$, we can see that the TT format (see also \eqref{eq:tt}) contains at most $dnr^2$ elements, which is much smaller than the number of entries in the original tensor $n^d$.
\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{figs/TTTrain_1wheel.png}\quad\quad
\caption{A scheme of the TT format. Wagons represent TT blocks - tensors of order 3. The first and last wagons are second-order tensors. Connection between wagons represent an index by which two neighbour TT blocks (wagons) are contracted.
}
\label{fig:TT}
\end{figure}
%
\subsection{Reshaping of the vector}

A tensor is a multi-index 
array, where multi-indices are used instead of indices.  As an
example, consider a vector
$\vek{w}\in\D{R}^N$, $N=10^{12}$ data points.  We can \emph{reshape}
it into a matrix $\vek{W}\in\D{R}^{10^6 \times 10^6}\cong \D{R}^{10^6}\otimes\D{R}^{10^6}$, which is 
a tensor of 2nd order. To get a tensor of 3rd order, we reshape it in the following way
$\D{R}^{10^4 \times 10^4 \times 10^4}\cong \bigotimes_{k=1}^3 \D{R}^{10^4}$ and so on (see Section 1 in \cite{Matthies2020}).
%One way to obtain a tensor
%from a vector or matrix is to reshape it.  For example, 
%assume $\vek{v} \in \D{R}^{10^6}$ is a vector. After reshaping it
%we can obtain a matrix --- a tensor of 2nd order --- of size $10^3 \times 10^3$, 
%or a tensor of 3rd order of size $10^2\times 10^2\times 10^2$,
% or a tensor of 6th order of size $10\times ... \times 10$ (6 times). 
%Each element of such a six-dimensional hypercube is described by a multi-index 
%$\vek{m}=(m_1,\dots,m_6)$. 
The higher the order of the tensor, the more possibilities there are to find
a low-rank approximation \citep{HA12}.
The tensors  obtained in this way contain not only rows and columns, but also
\emph{slices} and \emph{fibres} \citep{Kolda:01, Kolda:07, DMV-SIAM2:00, HA12}. 
These slices and fibres can be analysed for linear dependencies, super symmetry,
or sparsity,  and may result in a strong data compression \cite{WhyLowRank19}.  
%!!!
%
%





%  $Log: tensor_CP.tex,v $
%  Revision 1.7  2021/11/13 10:28:05  hgm
%  adjusted refs
%
%  Revision 1.6  2021/11/13 10:00:01  hgm
%  adjusted refs
%
%  Revision 1.5  2021/08/03 08:25:20  hgm
%  small changes
%
%  Revision 1.3  2021/04/16 21:44:53  hgm
%  changes acc. to protocol of Apr 2021
%
%  Revision 1.2  2019/06/10 22:13:09  hgm
%  further down the road
%
%  Revision 1.1  2019/06/09 10:29:20  hgm
%  initial check-in
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../19_low-rank_tensor_prob_den_char"
%%% End: 





==> common/pdfsetup.tex <==
% RCSID:       $Id: pdfsetup.tex 36 2007-04-12 15:00:01Z opajonk $
% Author:      Oliver Pajonk
% Contact:     o.pajonk@tu-bs.de, oliver@oliverpajonk.de

% Setup PDF-Latex to fill in all relevant metadata into a PDF file
%
% Needs: - you have to declare \theauthor, \thetitle, \thesubject
%           \pdflinkcolor and  \thekeywords before including this file

% The following package defines \ifpdf properly even with MikTeX 2.5
\usepackage{ifpdf}

\ifpdf
  \usepackage[pdftex,
       colorlinks=true,		% use links with color instead of boxes
       bookmarksnumbered,	% bookmarks have numbers in front of topic
       bookmarksopen,		% opens the bookmarks when the PDF is opened
       pdfstartview=FitH,	% opens the PDF with 'fit width' view
       linkcolor=\pdflinkcolor,	% standard red
       citecolor=\pdflinkcolor,	% standard green
       urlcolor=\pdflinkcolor,	% standard cyan
       filecolor=\pdflinkcolor,	% ?
       hyperindex,		% ?
       plainpages=false,	% ?
       breaklinks=true,		% allow links to break across lines!
       pdfpagelabels, %?
       hypertexnames=true,
%        linktocpage=true  % if enabled the link in toc is placed on the number rather than on the text
     ]{hyperref}
     \pdfinfo{
        /Title (\thetitle)
        /Author (\theauthor)
        /Subject (\thesubject)
        /Keywords (\thekeywords)}
     \usepackage[dvipdf]{graphicx}
	 \usepackage[pdftex]{thumbpdf}
\else
  \usepackage[
    colorlinks=true,
    linkcolor=\pdflinkcolor,
    hyperindex,
    plainpages=false
  ]{hyperref}
  \usepackage[dvips]{graphicx}
\fi

\hypersetup{a5paper,
            colorlinks,
            linkcolor=\pdflinkcolor,
            citecolor=\pdflinkcolor,
            urlcolor=\pdflinkcolor,
            pdftitle={\thetitle},
            pdfauthor={\theauthor},
            pdfsubject={\thesubject},
            pdfkeywords={\thekeywords},
            pdfproducer={\theauthor~using \LaTeXe}}


==> svformula.tex <==
%  hgm's macros

\usepackage{amsmath}

\spnewtheorem{thm}{Theorem}{\bfseries}{\itshape}
%\spnewtheorem*{proof}{Proof}{\itshape}{\rmfamily}
\spnewtheorem{xmpl}[thm]{Example}{\itshape}{\rmfamily}
\spnewtheorem{prop}[thm]{Proposition}{\bfseries}{\itshape}
\spnewtheorem{rem}[thm]{Remark}{\itshape}{\rmfamily}
\spnewtheorem{coro}[thm]{Corollary}{\bfseries}{\itshape}
\spnewtheorem{schol}[thm]{Scholium}{\bfseries}{\itshape}
\spnewtheorem{defi}[thm]{Definition}{\bfseries}{\rmfamily}
\spnewtheorem{lem}[thm]{Lemma}{\bfseries}{\itshape}

\newcommand{\ignore}[1]{}

\newcommand{\Wo}{\mathring{\mrm{W}}}
\newcommand{\Ho}{\mathring{\mrm{H}}}
\newcommand{\Lp}{\mrm{L}}
\newcommand{\Wp}{\mrm{W}}
\newcommand{\Hp}{\mrm{H}}
\newcommand{\Ck}{\mrm{C}}


\def\r#1{{\accent'27 #1}}
\def\frks#1#2{{\raise0.8ex\hbox{{\leavevmode$\scriptstyle #1$}}}{\kern-0.4ex\hbox{/}}{\raise-0.2ex\hbox{\kern-0.4ex\hbox{{\leavevmode$\scriptstyle #2$}}}}}


\newcommand{\vrho}{\varrho}
\newcommand{\vepsilon}{\varepsilon}
\newcommand{\vsigma}{\varsigma}
\newcommand{\vtheta}{\vartheta}
\newcommand{\vphi}{\varphi}
\newcommand{\vpi}{\varpi}
\newcommand{\vkappa}{\varkappa}

%\newcommand{\vGamma}{\varGamma}
%\newcommand{\vDelta}{\varDelta}
%\newcommand{\vTheta}{\varTheta}
%\newcommand{\vLambda}{\varLambda}
%\newcommand{\vXi}{\varXi}
%\newcommand{\vPi}{\varPi}
%\newcommand{\vSigma}{\varSigma}
%\newcommand{\vUpsilon}{\varUpsilon}
%\newcommand{\vPhi}{\varPhi}
%\newcommand{\vPsi}{\varPsi}
%\newcommand{\vOmega}{\varOmega}

% math symbols

% slanted, bold, serifs (for vectors and matrices)
%\newcommand{\vek}[1]{\mathchoice{\displaystyle\mnb{#1}}{\textstyle\boldsymbol{#1}}{\scriptstyle\mnb{#1}}{\scriptscriptstyle\mnb{#1}}}
\newcommand{\vek}[1]{\mnb{#1}}

% upright, bold, serifs (usually not for variables), no lower case greek
\newcommand{\mat}[1]{\mathchoice{\displaystyle\mbf{#1}}{\textstyle\mathbf{#1}}{\scriptstyle\mbf{#1}}{\scriptscriptstyle\mbf{#1}}}

% upright, bold, sans-serif (usually not for variables), no lower case greek
\newcommand{\opb}[1]{\mnb{\msf{#1}}}

% upright, non-bold, sans-serif (usually not for variables), no lower case greek
\newcommand{\ops}[1]{\mathchoice{\displaystyle\msf{#1}}{\textstyle\msf{#1}}{\scriptstyle\msf{#1}}{\scriptscriptstyle\msf{#1}}}

% slanted, bold, sans-serif (for tensors)
\newcommand{\tnb}[1]{\mathchoice{\displaystyle\msb{#1}}{\textstyle\msb{#1}}{\scriptstyle\msb{#1}}{\scriptscriptstyle\mathboldsans{#1}}}

% slanted, non-bold, sans-serif (for tensor components)
\newcommand{\tns}[1]{\mathchoice{\displaystyle\msi{#1}}{\textstyle\msi{#1}}{\scriptstyle\msi{#1}}{\scriptscriptstyle\mathsans{#1}}}
 
\newcommand{\vcek}[1]{\vek{\check{#1}}}
\newcommand{\vbar}[1]{\vek{\bar{#1}}}
\newcommand{\vtil}[1]{\vek{\tilde{#1}}}
\newcommand{\vhat}[1]{\vek{\hat{#1}}}
 
\newcommand{\Mcek}[1]{\mat{\check{#1}}}
\newcommand{\Mbar}[1]{\mat{\bar{#1}}}
\newcommand{\Mtil}[1]{\mat{\tilde{#1}}}
\newcommand{\Mhat}[1]{\mat{\hat{#1}}}
 
\newcommand{\Tcek}[1]{\tnb{\check{#1}}}
\newcommand{\Tbar}[1]{\tnb{\bar{#1}}}
\newcommand{\Ttil}[1]{\tnb{\tilde{#1}}}
\newcommand{\That}[1]{\tnb{\hat{#1}}}
 
\newcommand{\Scek}[1]{\tns{\check{#1}}}
\newcommand{\Sbar}[1]{\tns{\bar{#1}}}
\newcommand{\Stil}[1]{\tns{\tilde{#1}}}
\newcommand{\Shat}[1]{\tns{\hat{#1}}}

\newcommand{\EXP}[1]{\D{E}\left(#1\right)}
 
\newcommand{\dlangle}{\langle\negthinspace\langle}
\newcommand{\drangle}{\rangle\negthinspace\rangle}

\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\divg}{div}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\gra}{gra}
% \ker is already defined
% \dim is already defined
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\inti}{int}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\acx}{acx}
\DeclareMathOperator{\co}{co}

\newcommand{\dd}{\mathop{}\!\partial}
\newcommand{\di}{\mathop{}\!\mathrm{d}}
\newcommand{\Di}{\mathop{}\!\mathrm{D}}
\newcommand{\ii}{\mathchoice{\displaystyle\mathrm i}
{\textstyle\mathrm i}{\scriptstyle\mathrm i}
{\scriptscriptstyle\mathrm i}}
\newcommand{\ee}{\mathchoice{\displaystyle\mathrm e}
{\textstyle\mathrm e}{\scriptstyle\mathrm e}
{\scriptscriptstyle\mathrm e}}


==> wiley_formula.tex <==
%  hgm's macros

\usepackage{amsmath}

\newtheorem{thm}{Theorem}
%\newtheorem{thm}{Theorem}[section]
\newtheorem{xmpl}[thm]{Example}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{rem}[thm]{Remark}
%\newtheorem{lemma}{Lemma}
\newtheorem{coro}[thm]{Corollary}
\newtheorem{schol}[thm]{Scholium}
\newtheorem{bei}[thm]{Beispiel}
\newtheorem{satz}[thm]{Satz}
\newtheorem{defi}[thm]{Definition}
\newtheorem{bem}[thm]{Bemerkung}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{koro}[thm]{Korollar}

\newcommand{\ignore}[1]{}

\newcommand{\Wo}{\mathring{\mrm{W}}}
\newcommand{\Ho}{\mathring{\mrm{H}}}
\newcommand{\Lp}{\mrm{L}}
\newcommand{\Wp}{\mrm{W}}
\newcommand{\Hp}{\mrm{H}}
\newcommand{\Ck}{\mrm{C}}

\def\r#1{{\accent'27 #1}}
\def\frks#1#2{{\raise0.8ex\hbox{{\leavevmode$\scriptstyle #1$}}}{\kern-0.4ex\hbox{/}}{\raise-0.2ex\hbox{\kern-0.4ex\hbox{{\leavevmode$\scriptstyle #2$}}}}}

\newcommand{\vrho}{\varrho}
\newcommand{\vepsilon}{\varepsilon}
\newcommand{\vsigma}{\varsigma}
\newcommand{\vtheta}{\vartheta}
\newcommand{\vphi}{\varphi}
\newcommand{\vpi}{\varpi}
\newcommand{\vkappa}{\varkappa}

% slanted capital Greek letters

%\newcommand{\vGamma}{\varGamma}
%\newcommand{\vDelta}{\varDelta}
%\newcommand{\vTheta}{\varTheta}
%\newcommand{\vLambda}{\varLambda}
%\newcommand{\vXi}{\varXi}
%\newcommand{\vPi}{\varPi}
%\newcommand{\vSigma}{\varSigma}
%\newcommand{\vUpsilon}{\varUpsilon}
%\newcommand{\vPhi}{\varPhi}
%\newcommand{\vPsi}{\varPsi}
%\newcommand{\vOmega}{\varOmega}

\DeclareMathSymbol{\Gamma}{\mathalpha}{letters}{"00}
\DeclareMathSymbol{\Delta}{\mathalpha}{letters}{"01}
\DeclareMathSymbol{\Theta}{\mathalpha}{letters}{"02}
\DeclareMathSymbol{\Lambda}{\mathalpha}{letters}{"03}
\DeclareMathSymbol{\Xi}{\mathalpha}{letters}{"04}
\DeclareMathSymbol{\Pi}{\mathalpha}{letters}{"05}
\DeclareMathSymbol{\Sigma}{\mathalpha}{letters}{"06}
\DeclareMathSymbol{\Upsilon}{\mathalpha}{letters}{"07}
\DeclareMathSymbol{\Phi}{\mathalpha}{letters}{"08}
\DeclareMathSymbol{\Psi}{\mathalpha}{letters}{"09}
\DeclareMathSymbol{\Omega}{\mathalpha}{letters}{"0A}


% math symbols
 
\newcommand{\vcek}[1]{\vek{\check{#1}}}
\newcommand{\vbar}[1]{\vek{\bar{#1}}}
\newcommand{\vtil}[1]{\vek{\tilde{#1}}}
\newcommand{\vhat}[1]{\vek{\hat{#1}}}
 
\newcommand{\Mcek}[1]{\mat{\check{#1}}}
\newcommand{\Mbar}[1]{\mat{\bar{#1}}}
\newcommand{\Mtil}[1]{\mat{\tilde{#1}}}
\newcommand{\Mhat}[1]{\mat{\hat{#1}}}
 
\newcommand{\Tcek}[1]{\tnb{\check{#1}}}
\newcommand{\Tbar}[1]{\tnb{\bar{#1}}}
\newcommand{\Ttil}[1]{\tnb{\tilde{#1}}}
\newcommand{\That}[1]{\tnb{\hat{#1}}}
 
\newcommand{\Scek}[1]{\tns{\check{#1}}}
\newcommand{\Sbar}[1]{\tns{\bar{#1}}}
\newcommand{\Stil}[1]{\tns{\tilde{#1}}}
\newcommand{\Shat}[1]{\tns{\hat{#1}}}

\newcommand{\EXP}[1]{\mathbb{E}\left(#1\right)}
 
\newcommand{\dlangle}{\langle\negthinspace\langle}
\newcommand{\drangle}{\rangle\negthinspace\rangle}

\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\divg}{div}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\gra}{gra}
% \ker is already defined
% \dim is already defined
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\inti}{int}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\acx}{acx}
\DeclareMathOperator{\co}{co}

\newcommand{\dd}{\mathop{}\!\partial}
\newcommand{\di}{\mathop{}\!\mathrm{d}}
\newcommand{\Di}{\mathop{}\!\mathrm{D}}
\newcommand{\ii}{\mathchoice{\displaystyle\mathrm i}
{\textstyle\mathrm i}{\scriptstyle\mathrm i}
{\scriptscriptstyle\mathrm i}}
\newcommand{\ee}{\mathchoice{\displaystyle\mathrm e}
{\textstyle\mathrm e}{\scriptstyle\mathrm e}
{\scriptscriptstyle\mathrm e}}

